Beyond Pinball Loss: Quantile Methods for Calibrated Uncertainty Quantification

Among the many ways of quantifying uncertainty in a regression setting, specifying the full quantile function is attractive, as quantiles are amenable to interpretation and evaluation. A model that predicts the true conditional quantiles for each input, at all quantile levels, presents a correct and efficient representation of the underlying uncertainty. To achieve this, many current quantile-based methods focus on optimizing the so-called pinball loss. However, this loss restricts the scope of applicable regression models, limits the ability to target many desirable properties (e.g. calibration, sharpness, centered intervals), and may produce poor conditional quantiles. In this work, we develop new quantile methods that address these shortcomings. In particular, we propose methods that can apply to any class of regression model, allow for selecting a trade-off between calibration and sharpness, optimize for calibration of centered intervals, and produce more accurate conditional quantiles. We provide a thorough experimental evaluation of our methods, which includes a high dimensional uncertainty quantification task in nuclear fusion.

==> NeurIPS2021/abstract.tex <==
\vspace{-3mm}
\begin{abstract}
\vspace{-1mm}

    Among the many ways of quantifying uncertainty in a regression setting, 
    specifying the full quantile function is attractive, 
    as quantiles are amenable to interpretation and evaluation. 
    A model that predicts the true conditional quantiles for each input, 
    at all quantile levels, presents a correct and efficient representation of the underlying uncertainty.
    To achieve this, many current quantile-based methods focus on optimizing the
    \textit{pinball loss}. However, this loss restricts the scope of applicable regression models,
    limits the ability to target many desirable properties (e.g. calibration, sharpness, centered intervals), 
    and may produce poor conditional quantiles.
    % This lack of flexibility limits a practitioner's ability to prioritize application-specific aspects of the model's output.
    In this work, we develop new quantile methods that address these shortcomings.
    In particular, we propose methods that can apply to any class of regression model, 
    % equip any class of regression model with quantile-based uncertainties,
    select an explicit balance between calibration and sharpness, 
    optimize for calibration of centered intervals, and produce more accurate conditional quantiles.
    We provide a thorough experimental evaluation of our methods,
    which includes a high dimensional uncertainty quantification task in nuclear fusion.






    % -------------- OLD ABSTRACT SCRAPS BELOW
    
    % % Quantiles provide an attractive form of uncertainty quantification for regression, as they are amenable to interpretation and evaluation. 
    % % Accordingly, a model that outputs the true conditional quantile for each input, for all probabilities, presents a correct and efficient representation of the underlying uncertainty.
    % % % While established methods exist in quantile regression, they may be restrictive in model class, in selecting a tradeoff between desirable properties (e.g. calibration, sharpness, centered intervals), and be insufficient in approaching the true conditional quantiles.
    % % While established methods exist for quantile regression (QR), they may be restricted to certain classes of models, limit the tradeoff between desirable properties (e.g. calibration, sharpness, centered intervals), and be insufficient in estimating the true conditional quantiles.
    % % In this work, we develop methods that add flexibility to, and extend the scope of, QR. 
    % % % We propose methods {that are applicable to non-differentiable models} {that allow QR in non-differentiable model}, allow selecting a pareto-optimal tradeoff between calibration and sharpness, optimize for calibration of centered intervals, and induce better convergence to the true conditional quantiles.
    % % We propose methods that allow for QR in any regression model, allow for selecting a pareto-optimal tradeoff between calibration and sharpness, optimize for calibration of centered intervals, and induce better convergence to the true conditional quantiles.
    
    
    % % Quantiles provide an attractive form of uncertainty quantification for regression, as they are amenable to interpretation and evaluation. 
    % % A model that outputs the true conditional quantiles for each input and for all probabilities, presents a correct and efficient representation of the underlying uncertainty.
    % % While established methods exist for quantile regression (QR), they may be restricted to certain classes of models, limit the tradeoff between desirable properties (e.g. calibration, sharpness, centered intervals), and may produce poor conditional quantiles.
    % % While most methods rely on the pinball loss to estimate quantiles from data, this may be 
    % % This lack of flexibility hurts practitioners since there may be application-specific aspects one may want to prioritize in the model's output.
    % % In this work, we develop methods that add flexibility to, and extend the scope of, QR. 
    % % In particular, we propose methods that allow for QR in any regression model, allow for selecting a Pareto-optimal tradeoff between calibration and sharpness, optimize for calibration of centered intervals, and produce more accurate conditional quantiles.
    
    % Among the many ways of quantifying uncertainty in a regression setting, 
    % specifying the full quantile function is attractive, 
    % as quantiles are amenable to interpretation and evaluation. 
    % A model that predicts the true conditional quantiles for each input, 
    % at all quantile levels, presents a correct and efficient representation of the underlying uncertainty.
    % To achieve this, many current quantile-based methods focus on optimizing the so-called
    % \textit{pinball loss}.
    % However, this loss 
    % % While current quantile-based methods focus on optimizing the pinball loss,  this
    % %
    % %  they are limited in scope to a relatively narrow set of applicable regression models, enforce
    % % a strict tradeoff between desirable properties (e.g. calibration, sharpness, centered intervals)
    % % 
    % restricts the scope of applicable regression models,
    % limits % the flexibility to choose % the ability to pursue % the flexibility to tradeoff between % the flexibility to achieve
    % the ability to target many
    % % the choice of
    % desirable properties (e.g. calibration, sharpness, centered intervals), 
    % and may produce poor conditional quantiles.
    % % This lack of flexibility limits a practitioner's ability to prioritize application-specific aspects of the model's output.
    % % This lack of flexibility hurts practitioners since there may be application-specific aspects one may want to prioritize in the model's output.
    % In this work, we develop new quantile methods that address these shortcomings.
    % In particular, we propose methods that
    % can apply to any class of regression model, 
    % % provide quantile-based uncertainties to any class of regression model,
    % % equip any class of regression model with quantile-based uncertainties,
    % allow for selecting a trade-off between calibration and sharpness, 
    % optimize for calibration of centered intervals, and produce more accurate conditional quantiles. We provide a thorough experimental evaluation of our methods,
    % which includes a high dimensional uncertainty quantification task in nuclear fusion.
    % % Code is available at\\
    % % \url{https://github.com/YoungseogChung/calibrated-quantile-uq}
    
    % % including on a high dimensional uncertainty quantification task in nuclear fusion.
    % % validate our methods experimentally on a variety of datasets and on a high dimensional uncertainty quantification task in nuclear fusion.
    
    
\end{abstract}

% \begin{keywords}
%     Uncertainty Quantification, Calibrated Regression, Quantile Regression, Aleatoric Uncertainty
% \end{keywords}

==> NeurIPS2021/app_ablation.tex <==
\section{Ablation Study}
\subsection{Ablation Study Details}
 \label{app:ablation_study_exp_setting}

The ablation study from Section~\ref{sec:ablation} (with full results in Appendix~\ref{app:full_ablation_results}) 
investigates the effect of group batching on two methods:
\textit{Cali} (combined calibration loss, one of our proposed methods)
and \textit{SQR} (a baseline method).

For each method, we applied group batching by tuning the group batching frequency hyperparameter 
with cross-validation according to the details in Appendix~\ref{app:uci_exp_details}.

When we did not apply group batching, each batch was a uniform draw from the training dataset,
which is the default setting in most batch optimization procedures. 


\subsection{Full Ablation Study Experiment Results} \label{app:full_ablation_results}
The full set of results from the ablation study presented in Section~\ref{sec:ablation}
is provided here. 
To re-iterate the purpose of this study: we show how group batching affects
UQ performance on two methods: \textit{Cali} (combined calibration loss, which is one 
of our proposed methods) and \textit{SQR} (a baseline method).

We present the effect of group batching via all of the evaluation metrics
(average calibration, sharpness, adversarial group calibration, check score, interval score,
and centered interval calibration).

\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c||c|c|}
 \hline & \multicolumn{2}{c|}{{\textit{Cali}}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}               \\\hline
Concrete & $6.6\pm0.9(17.6\pm2.3)$ & $\textbf{5.6}\pm0.8(\underline{17.3}\pm1.5)$ \\ \hline
Power    & $\textbf{1.7}\pm0.2(14.2\pm0.3)$ & $2.0\pm0.1(\underline{13.1}\pm0.1)$    \\ \hline
Wine     & $4.4\pm0.5(\underline{25.6}\pm0.8)$ & $\textbf{4.2}\pm0.4(26.0\pm0.8)$ \\ \hline
Yacht    & $11.1\pm1.8(\underline{1.8}\pm0.1)$ & $\textbf{8.3}\pm0.6(2.0\pm0.4)$     \\ \hline
Naval    & $2.8\pm0.2(\underline{12.1}\pm3.1)$ & $\textbf{2.4}\pm0.3(50.6\pm8.6)$    \\ \hline
Energy   & $9.2\pm0.3(\underline{2.8}\pm0.1)$ & $\textbf{5.8}\pm0.4(3.6\pm0.3)$  \\ \hline
Boston   & $9.7\pm1.3(\underline{10.2}\pm0.7)$ & $\textbf{8.5}\pm1.5(10.9\pm0.6)$ \\ \hline
Kin8nm   & $\textbf{3.4}\pm0.3(\underline{13.7}\pm0.4)$ & $3.5\pm0.3(\underline{13.7}\pm0.7)$ \\ \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |c||c|c|}
 \hline & \multicolumn{2}{c|}{{\textit{SQR}}} \\
 \hline
          & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Concrete  & $9.8\pm1.3(\underline{7.0}\pm0.6)$ & $\textbf{7.1}\pm0.9(8.5\pm0.6)$ \\ \hline
Power     & $\textbf{2.5}\pm0.3(14.0\pm0.5)$ & $2.9\pm0.5(\underline{13.6}\pm0.8)$ \\ \hline
Wine      & $4.5\pm0.4(29.7\pm0.5)$ & $\textbf{4.0}\pm0.4(\underline{28.5}\pm0.8)$ \\ \hline
Yacht     & $9.0\pm0.9(\underline{0.9}\pm0.1)$ & $\textbf{8.9}\pm0.9(2.3\pm0.2)$ \\ \hline
Naval     & $8.6\pm1.6(\underline{3.6}\pm0.1)$ & $\textbf{5.3}\pm0.8(6.0\pm0.5)$ \\ \hline
Energy    & $10.2\pm0.8(\underline{1.8}\pm0.1)$ & $\textbf{6.9}\pm1.1(2.4\pm0.2)$ \\ \hline
Boston    & $10.9\pm1.0(\underline{8.8}\pm1.1)$ & $\textbf{9.8}\pm1.2(9.5\pm0.9)$ \\ \hline
Kin8nm    & $4.7\pm0.3(\underline{11.1}\pm0.1)$ & $\textbf{3.9}\pm0.4(11.3\pm0.2)$ \\ \hline
\end{tabular}
\end{center}
\caption{\textbf{Group Batching Ablation: Average Calibration and Sharpness.}
    The table shows mean ECE and sharpness (in parentheses) and their standard error with and without group batching. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined for \textit{Cali} and \textit{SQR} separately. All values have been multiplied by 100 for readability.
    This is the same table as Figure~\ref{fig:group_batch_ablation_main} from Section~\ref{sec:ablation}, which is repeated here for completeness.
    \label{table:group_batch_ablation_app}}
% \end{center}
% \vspace{-5mm}
\end{figure*}


\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{ICML2021/figs/Cali_group_batching_cal_sharp.pdf}
    \caption{\textbf{Group Batching Ablation with \textit{Cali} Method: Average Calibration and Sharpness Plot.} 
    GB in legend refers to group batching. 
    Group batching tends to improve calibration and worsen sharpness for the \textit{Cali} method.}
    \label{fig:cali_ablation_cal_sharp}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{ICML2021/figs/Cali_group_batching_adv.pdf}
    \caption{\textbf{Group Batching Ablation with \textit{Cali} Method: Adversarial Group Calibration.} 
    GB in legend refers to group batching. 
    Group batching tends to improve adversarial group calibration for the \textit{Cali} method.}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{ICML2021/figs/SQR_group_batching_cal_sharp.pdf}
    \caption{\textbf{Group Batching Ablation with \textit{SQR} Method: Average Calibration and Sharpness Plot.} 
    GB in legend refers to group batching. 
    Group batching tends to improve calibration and worsen sharpness for \textit{SQR} method.}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    \includegraphics[width=\textwidth]{ICML2021/figs/SQR_group_batching_adv.pdf}
    % \includegraphics[width=\textwidth]{ICML2021/figs/SQR_group_batching_cal_sharp.pdf}
    \caption{\textbf{Group Batching Ablation with \textit{SQR} Method: Adversarial Group Calibration.}
    GB in legend refers to group batching. 
    Group batching tends to improve adversarial group calibration for \textit{SQR} method.}
    % \vspace{-4mm}
\end{figure*}


\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c||c|c || c|c|c|}
 \hline & \multicolumn{2}{c||}{\textit{Cali}} & \multicolumn{2}{c|}{\textit{SQR}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}            & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Concrete  & $ 0.120 \pm 0.007 $ & $ \mathbf{0.118 \pm 0.006} $   &   $ 0.083 \pm 0.006 $ & $ \mathbf{0.077 \pm 0.004} $ \\ \hline
Power     & $ \mathbf{0.063 \pm 0.002} $ & $ 0.064 \pm 0.001 $   &   $ \mathbf{0.056 \pm 0.001} $ & $ 0.057 \pm 0.001 $ \\ \hline
Wine      & $ \mathbf{0.209 \pm 0.007} $ & $ 0.210 \pm 0.008 $   &   $ \mathbf{0.206 \pm 0.008} $ & $ \mathbf{0.206 \pm 0.008} $ \\ \hline
Yacht     & $ \mathbf{0.018 \pm 0.002} $ & $ 0.019 \pm 0.004 $   &   $ \mathbf{0.011 \pm 0.002} $ & $ 0.013 \pm 0.002 $ \\ \hline
Naval     & $ \mathbf{0.042 \pm 0.009} $ & $ 0.159 \pm 0.029 $   &   $ \mathbf{0.007 \pm 0.000} $ & $ 0.014 \pm 0.001 $ \\ \hline
Energy    & $ \mathbf{0.016 \pm 0.000} $ & $ 0.017 \pm 0.002 $   &   $ \mathbf{0.013 \pm 0.000} $ & $ \mathbf{0.013 \pm 0.001} $ \\ \hline
Boston    & $ \mathbf{0.100 \pm 0.013} $ & $ 0.103 \pm 0.013 $   &   $ 0.091 \pm 0.007 $ & $ \mathbf{0.089 \pm 0.008} $ \\ \hline
Kin8nm    & $ \mathbf{0.094 \pm 0.002} $ & $ 0.096 \pm 0.005 $   &   $ 0.079 \pm 0.001 $ & $ \mathbf{0.077 \pm 0.000} $ \\ \hline
\end{tabular}
\caption{\textbf{Group Batching Ablation: Check Score.}
    This table shows mean test check score and their standard error with and without group batching
    for both \textit{Cali} and \textit{SQR}. The best mean for each dataset has been bolded for \textit{Cali} and \textit{SQR} separately. 
    While the general pattern is that group batching worsens the check score, 
    this is expected because group batching tends to worsen sharpness
    and the check score favors sharpness (Proposition 1 in main paper).
    Still, the change in the mean of the check score tends to be insignificant
    when considering the standard errors (except for Naval dataset).
    }\label{tab:group_batch_ablation_check}
\end{center}
\vspace{-5mm}
\end{figure*}

\begin{figure*}[h!]
\begin{center} %\label{fig:group_batch_ablation}
\begin{tabular}{ |c||c|c || c|c|c|}
 \hline & \multicolumn{2}{c||}{\textit{Cali}} & \multicolumn{2}{c|}{\textit{SQR}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}            & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Concrete & $ 1.498 \pm 0.083 $  &  $ \mathbf{1.465 \pm 0.086} $   &   $ 1.254 \pm 0.120 $  &  $ \mathbf{1.079 \pm 0.066} $ \\ \hline
Power    & $ \mathbf{0.667 \pm 0.025} $  &  $ 0.699 \pm 0.019 $   &   $ \mathbf{0.603 \pm 0.016} $  &  $ 0.615 \pm 0.014 $ \\ \hline
Wine     & $ \mathbf{2.495 \pm 0.130} $  &  $ 2.498 \pm 0.135 $   &   $ \mathbf{2.325 \pm 0.107} $  &  $ 2.362 \pm 0.117 $ \\ \hline
Yacht    & $ \mathbf{0.276 \pm 0.040} $  &  $ 0.298 \pm 0.063 $   &   $ 0.177 \pm 0.033 $  &  $ \mathbf{0.164 \pm 0.029} $ \\ \hline
Naval    & $ \mathbf{0.479 \pm 0.098} $  &  $ 1.560 \pm 0.268 $   &   $ \mathbf{0.069 \pm 0.003} $  &  $ 0.144 \pm 0.014 $ \\ \hline
Energy   & $ 0.218 \pm 0.009 $  &  $ \mathbf{0.204 \pm 0.018} $   &   $ 0.191 \pm 0.006 $  &  $ \mathbf{0.172 \pm 0.012} $ \\ \hline
Boston   & $ \mathbf{1.437 \pm 0.255} $  &  $ 1.449 \pm 0.259 $   &   $ 1.284 \pm 0.151 $  &  $ \mathbf{1.217 \pm 0.152} $ \\ \hline
Kin8nm   & $ \mathbf{1.102 \pm 0.031} $  &  $ 1.121 \pm 0.072 $   &   $ 0.914 \pm 0.016 $  &  $ \mathbf{0.871 \pm 0.011} $ \\ \hline
\end{tabular}
\caption{\textbf{Group Batching Ablation: Interval Score.}
    This table shows mean test interval score and their standard error with and without group batching
    for both \textit{Cali} and \textit{SQR}. The best mean for each dataset has been bolded for \textit{Cali} and \textit{SQR} separately. 
    The general pattern is that the interval score worsens for \textit{Cali} 
    and improves for \textit{SQR}.
    However, the change tends to be insignificant
    when considering the standard errors (except for Naval dataset).}
\end{center}
\vspace{-5mm}
\end{figure*}

\begin{figure*}[h!]
\begin{center} %\label{fig:group_batch_ablation}
\begin{tabular}{ |c||c|c || c|c|c|}
 \hline & \multicolumn{2}{c||}{\textit{Cali}} & \multicolumn{2}{c|}{\textit{SQR}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}            & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Concrete    & $ 0.102 \pm 0.014 $ & $ \mathbf{0.096 \pm 0.013} $   &   $ 0.188 \pm 0.029 $ & $ \mathbf{0.127 \pm 0.014} $ \\ \hline
Power       & $ \mathbf{0.033 \pm 0.003} $ & $ 0.037 \pm 0.002 $   &   $ \mathbf{0.040 \pm 0.008} $ & $ 0.047 \pm 0.006 $ \\ \hline
Wine        & $ 0.072 \pm 0.007 $ & $ \mathbf{0.065 \pm 0.007} $   &   $ 0.057 \pm 0.005 $ & $ \mathbf{0.055 \pm 0.005} $ \\ \hline
Yacht       & $ 0.139 \pm 0.018 $ & $ \mathbf{0.129 \pm 0.016} $   &   $ 0.128 \pm 0.027 $ & $ \mathbf{0.119 \pm 0.020} $ \\ \hline
Naval       & $ 0.048 \pm 0.006 $ & $ \mathbf{0.034 \pm 0.002} $   &   $ 0.114 \pm 0.032 $ & $ \mathbf{0.066 \pm 0.009} $ \\ \hline
Energy      & $ 0.146 \pm 0.013 $ & $ \mathbf{0.090 \pm 0.011} $   &   $ 0.171 \pm 0.018 $ & $ \mathbf{0.104 \pm 0.020} $ \\ \hline
Boston      & $ 0.142 \pm 0.032 $ & $ \mathbf{0.138 \pm 0.028} $   &   $ 0.195 \pm 0.021 $ & $ \mathbf{0.173 \pm 0.027} $ \\ \hline
Kin8nm      & $ \mathbf{0.061 \pm 0.004} $ & $ 0.067 \pm 0.005 $   &   $ 0.079 \pm 0.003 $ & $ \mathbf{0.069 \pm 0.009} $ \\ \hline

\end{tabular}
\caption{\textbf{Group Batching Ablation: Centered Interval Calibration.}
    This table shows mean test centered interval calibration (measured by ECE for centered intervals) score and their standard error with and without group batching
    for both \textit{Cali} and \textit{SQR}. The best mean for each dataset has been bolded for \textit{Cali} and \textit{SQR} separately. 
    The general pattern is that group batching improves centered interval calibration 
    for both \textit{Cali} and \textit{SQR}.
    While the change tends to be insignificant
    when considering the standard errors,
    the improvement is significant in numerous cases 
    (e.g. Naval and Energy for both methods, Concrete with \textit{SQR}).}
\end{center}
% \vspace{-5mm}
\end{figure*}



==> NeurIPS2021/app_add_discussion.tex <==
\section{Additional Discussions}


\paragraph{Potential negative social impacts}

This work proposes methods in uncertainty quantification (UQ), 
with a focus on the notion of calibration. 
UQ is a field that is becoming more and more important as many autonomous systems are being deployed in various real-life applications (self-driving cars, security devices, object recognition systems).
While we believe the development of robust and
accurate methods in UQ will accelerate deployment of autonomous systems and expand real-world 
use-cases, 
we also acknowledge the potential disruptive effects 
such change can have in the relevant industries.

Futher, calibration is a relevant notion in fairness \citep{kleinberg2016inherent}.
Though we propose methods to achieve better calibration
when making probabilistic forecasts, 
we note the potential for using such information with 
ill intent, e.g. to intentionally avoid calibrated (or fair) 
decisions.

\paragraph{Assets used in this work}
In implementing our work, we have referenced the implementation of 
one of the baseline methods (\textit{SQR}), which is publicly available under the Creative Commons Attribution-NonCommercial 4.0 International Public License.

We also state that no data from human subjects were used in this work and 
thus there is no personal identifying information.

==> NeurIPS2021/app_add_exp.tex <==
\section{Additional Experiments}
\subsection{Details of Synthetic Experiment (Figure~\ref{fig:synth_example})}
\label{app:synth_example}
\textbf{Dataset}: The synthetic dataset is based on the Boston
UCI dataset. 
A NN model, $\mu_\theta$, was trained on the train split of the Boston dataset to predict the mean by optimizing the MSE loss (same architecture and training details as described in Appendix~\ref{app:uci_exp_details}).
Afterwards, all points, $\{(x_i, y_i)\}_{i=1}^{N}$, in the full Boston dataset were re-labelled with the prediction of the mean model, $(x_i, \mu_\theta(x_i))$. 
Then, uniform noise, $\eps_i$ was added to these re-labelled mean values to create the observations, $\Tilde{y}_i$, i.e. $\Tilde{y}_i = \mu_\theta(x_i) + \eps_i$. 
The uniform noise was 0 mean, with width of the support equal to $5\%$ of the range of the mean values, i.e $\eps_i \sim$ Unif$[-0.025*(\max_i{y_i} - \min_i{y_i}), 0.025*(\max_i{y_i} - \min_i{y_i})]$.
Thus synthetic dataset is $\{(x_i, \Tilde{y_i})\}_{i=1}^{N}$.

\textbf{Procedure}: The training procedure follows exactly that of the main experiments, which is described in detail in Appendix~\ref{app:uci_exp_details}.
The only difference is that the models were trained for the full 1000 epochs, instead of halting training according to the validation loss. 



\subsection{Regularizing the Pinball Loss}
\label{app:regularization_pinball}
At first glance, regularization may appear to be the answer to what seems like 
an overfitting problem with the pinball loss, however, 
the problem is deeper and more specific to the loss function.
In this section, we empirically demonstrate the effect of applying regularization when minimizing the pinball loss.

With the \textit{SQR} method (which optimizes the pinball loss simultaneously for random batches of quantile levels),
we applied L1, L2, and dropout, 
by cross-validating the regularization coefficients 
in \{$2^{i}, i \in $ np.linspace$(-13, 1, 40)$\} for L1 and L2, % $2^{-13}$ and $2$ 
% in 40 increments on the log scale for L1 and L2,
and dropout probability $p$ 
in \{$2^{i}, i \in $ np.linspace$(-13, -1, 40)$\},
% between $2^{-13}$ and $2^{-1}$
% in 40 increments on the log scale for dropout, 
for the pinball loss criterion (i.e. cross-validate among 40 different regularization coefficients, between $2^{-13}$ and $2^{-1}$ on the log scale).  
We show the best calibrated regularization result, across all regularization methods and cross-validation (table in same format as Figure 2 in paper).
\begin{figure*}[h!]
\centering
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
          & \textit{SQR} & \textit{SQR w/Reg}      \\ \hline
concrete & $ \mathbf{9.3} \pm 1.5 (7.0 \pm 1.0)$ & $ 10.9 \pm 1.0 (\underline{6.9} \pm 0.6)$  \\ \hline
power    & $ 2.6 \pm 0.4 (\underline{13.4} \pm 0.2)$ & $ \mathbf{1.0} \pm 0.1 (14.8 \pm 0.1)$  \\ \hline
wine     & $ \mathbf{4.2} \pm 0.2 (29.5 \pm 0.4)$ & $ 5.1 \pm 0.8 (\underline{26.0} \pm 0.5)$  \\ \hline
yacht    & $ \mathbf{9.4} \pm 0.9 (\underline{1.0} \pm 0.1)$ & $ 12.3 \pm 2.6 (\underline{1.0} \pm 0.1)$   \\ \hline
naval    & $ \mathbf{9.7} \pm 1.6 (\underline{3.5} \pm 0.4) $ & $ 11.5 \pm 2.8 (\underline{3.5} \pm 0.3)$  \\ \hline
energy   & $ 9.8 \pm 0.8 (2.0 \pm 0.1) $ & $ \mathbf{9.4} \pm 1.3 (\underline{1.9} \pm 0.2)$   \\ \hline
boston   & $ \mathbf{9.0} \pm 0.8 (9.3 \pm 0.7) $ & $ 11.6 \pm 1.1 (\underline{8.6} \pm 0.8)$  \\ \hline
kin8nm   & $ 4.4 \pm 0.1 (11.4 \pm 0.2)$ & $ \mathbf{3.5} \pm 0.3 (\underline{11.2} \pm 0.2)$  \\ \hline
\end{tabular}
\caption{\textbf{Applying Regularization with SQR: Average Calibration and Sharpness.}
The table shows \textit{SQR}'s mean ECE and sharpness (in parentheses) and their standard error with and without regularization. Among the 3 regularization methods (L1, L2, dropout), the method resulting in the best calibration is shown, for each dataset. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined. All values have been multiplied by 100 for readability.}
\end{figure*}

Counter-intuitively, regularization tends to further the bias towards sharpness,
and upon reflection, this may not be surprising because the range of quantile
predictions shrink: given a quantile model $f: \mathcal{X} \times \mathcal{P} \rightarrow \mathcal{Y}$, where $\mathcal{P}$ is the space of quantile levels in $(0, 1)$, regularization affects the smoothness not only in $\mathcal{X}$, but also in $\mathcal{P}$, hence for any fixed $x\in\mathcal{X}$, the range in predictions for different quantile level inputs also shrinks.

\subsection{Comparison on 95\% Prediction Interval Task} \label{app:coverage_95}
In Section~\ref{sec:experiments}, we have presented an experiment that is targeted at evaluating the \textit{full predictive distribution} on the 8 UCI datasets.

In this section, we present an experiment that is targeted at constructing a \textit{$95\%$ centered prediction interval (PI)} on the same UCI datasets, for the purposes of comparing against other quantile-based algorithms that are designed to output only
a single quantile level.
This experiment setup is exactly the same as the prediction intervals experiments 
in Section 4.1 of the work by \citet{tagasovska2019single}, and we follow the exact same experiment procedure 
for a direct comparison against their reported results.

The comparison algorithms here are:
\begin{itemize}
    \item Dropout \citep{gal2016dropout}:
    a NN that uses a dropout layer during testing for multiple predictions
    \item QualityDriven \citep{pearce2018high}:
    a NN that optimizes a Binomial likelihood approximation as a surrogate loss for calibration and sharpness 
    \item GradientBoosting \citep{meinshausen2006quantile}:
    a decision tree based model that optimizes the pinball loss with gradient boosting
    \item QuantileForest \citep{meinshausen2006quantile}:
    a decision tree based model that predicts the quantiles based on the trained 
    output of a random forest
    \item ConditionalGaussian \citep{lakshminarayanan2017simple}: 
    a probabilistic NN that optimizes the Gaussian NLL to output the parameters 
    of a Gaussian distribution 
    % \item SQR (\cite{tagasovska2019single}):
    % a NN that simultaneoulsy optimizes the pinball loss for random draws of quantiles levels 
\end{itemize}

We show the performance of \textit{MAQR} to represent our proposed methods in this experiment, 
since \textit{MAQR} performs the best on the full predictive distribution evaluations in the UCI experiments of Section~\ref{sec:uci_fusion}.
We also omit the results of \textit{SQR} \citet{tagasovska2019single} in this experiment since we perform
a full evaluation comparison with \textit{SQR} in Section~\ref{sec:uci_fusion} and Appendix~\ref{app:all_uci_results},  \ref{app:all_fusion_results}, 
and the purpose here is to compare our proposed method against the additional baselines. 


In this experiment, since we only output two quantile levels ($0.025, 0.975$) to 
construct a single $95\%$ prediction interval, we do not assess calibration (which requires the predictions for all quantile levels)
and assess only the observed proportion of test points within the PI (also referred to as ``prediction interval coverage probability'' or ``PICP'') and sharpness 
represented by the width of the PI (also referred to as ``mean prediction interval width'' or ``MPIW'').
We refer the reader to \citet{tagasovska2019single} for exact details on the experiment setup and the hyperparameters tuned.
For \textit{MAQR}, we used the exact same NN architecture (1 layer of 64 hidden units, ReLU non-linearities) as the NN based baselines (\textit{Dropout, QualityDriven, ConditionalGaussian}) and the same training procedure as detailed in \citet{tagasovska2019single}.
The hyperparameters tuned for \textit{MAQR} are detailed in Appendix~\ref{app:uci_exp_details}.

\begin{figure*}[h!] 
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
            & \textit{Dropout}                        & \textit{QualityDriven}                  & \textit{GradientBoostingQR}                \\ \hline       
 concrete   & none                           & none                           & $0.93\pm0.00$ $(0.71\pm0.00)$     \\ \hline
 power      & $0.94\pm0.00$ $(0.37\pm0.00)$  & $0.93\pm0.02$ $(0.34\pm0.19)$  & none                              \\ \hline
 wine       & none                           & none                           & none                              \\ \hline
 yacht      & $0.97\pm0.03$ $(0.10\pm0.01)$  & $0.92\pm0.05$ $(0.04\pm0.01)$  & $0.95\pm0.02$ $(0.79\pm0.01)$     \\ \hline
 naval      & $0.96\pm0.01$ $(0.23\pm0.00)$  & $0.94\pm0.02$ $(0.21\pm0.11)$  & none                              \\ \hline
 energy     & $0.91\pm0.04$ $(0.17\pm0.01)$  & $0.91\pm0.04$ $(0.10\pm0.05)$  & none                              \\ \hline
 boston     & none                           & none                           & $0.89\pm0.00$ $(0.75\pm0.00)$     \\ \hline
 kin8nm     & none                           & $0.96\pm0.00$ $(0.84\pm0.00)$  & none                              \\ \hline    
\hline
            & \textit{QuantileForest}                 & \textit{ConditionalGaussian}            & \textbf{\textit{MAQR}}            \\ \hline
 concrete   & $0.96\pm0.01$ $(0.37\pm0.02)$  & $0.94\pm0.03$ $(0.32\pm0.09)$  & $0.93\pm0.01$ $(0.26\pm0.01)$     \\ \hline
 power      & $0.94\pm0.01$ $(0.18\pm0.00)$  & $0.94\pm0.01$ $(0.18\pm0.00)$  & $0.95\pm0.01$ $(0.28\pm0.03)$     \\ \hline
 wine       & none                           & $0.94\pm0.02$ $(0.49\pm0.03)$  & $0.95\pm0.02$ $(0.56\pm0.06)$     \\ \hline
 yacht      & $0.97\pm0.04$ $(0.28\pm0.11)$  & $0.93\pm0.06$ $(0.03\pm0.01)$  & $0.92\pm0.03$ $(0.03\pm0.01)$     \\ \hline
 naval      & $0.92\pm0.01$ $(0.22\pm0.00)$  & $0.96\pm0.01$ $(0.15\pm0.25)$  & $0.94\pm0.01$ $(0.03\pm0.00)$     \\ \hline
 energy     & $0.95\pm0.02$ $(0.15\pm0.01)$  & $0.94\pm0.03$ $(0.12\pm0.18)$  & $0.94\pm0.02$ $(0.05\pm0.01)$     \\ \hline
 boston     & $0.95\pm0.03$ $(0.37\pm0.02)$  & $0.94\pm0.03$ $(0.55\pm0.20)$  & $0.95\pm0.02$ $(0.34\pm0.09)$     \\ \hline
 kin8nm     & none                           & $0.93\pm0.01$ $(0.20\pm0.01)$  & $0.93\pm0.00$ $(0.20\pm0.01)$     \\ \hline
\hline

\end{tabular}
\caption{\textbf{95\% PI PICP and MPIW} The test average and standard deviation PICP of models with validation PICP in $[92.5\%, 97.5\%]$ is shown, and the test average and standard deviation MPIW is shown in parantheses. ``none'' indicates the method could not find a model with validation PICP in $[92.5\%, 97.5\%]$.}\label{tab:pi_95}
\end{center}
\end{figure*}

Summarizing the experimental result in Figure~\ref{tab:pi_95}:
\begin{itemize}
    \item 
    Our proposed method (\textit{MAQR}) is capable of consistently producing PIs
    that have the correct desired coverage ($0.95$),  
    even in cases when some of the baseline algorithms are not able to.
    \item
    Even when the baseline algorithms do produce PIs with correct desired coverage, 
    \textit{MAQR} is able to produce PI's that are much sharper (e.g. mean PI width for naval dataset
    is an order of magnitude sharper than all other baselines) 
\end{itemize}

On this limited output and evaluation setting, our proposed method is still competitive
in its performance.
However, it should be noted that this experiment tells \textit{only one facet} of overall UQ quality.
Inspecting and evaluating the full predictive uncertainty is necessary for a more thorough evaluation of UQ quality, as done in our main experiments in Section~\ref{sec:experiments}.


% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
%             & Dropout                        & QualityDriven                  & GradientBoostingQR                \\ \hline       
%  concrete   & none                           & none                           & $0.93\pm0.00$ $(0.71\pm0.00)$     \\ \hline
%  power      & $0.94\pm0.00$ $(0.37\pm0.00)$  & $0.93\pm0.02$ $(0.34\pm0.19)$  & none                              \\ \hline
%  wine       & none                           & none                           & none                              \\ \hline
%  yacht      & $0.97\pm0.03$ $(0.10\pm0.01)$  & $0.92\pm0.05$ $(0.04\pm0.01)$  & $0.95\pm0.02$ $(0.79\pm0.01)$     \\ \hline
%  naval      & $0.96\pm0.01$ $(0.23\pm0.00)$  & $0.94\pm0.02$ $(0.21\pm0.11)$  & none                              \\ \hline
%  energy     & $0.91\pm0.04$ $(0.17\pm0.01)$  & $0.91\pm0.04$ $(0.10\pm0.05)$  & none                              \\ \hline
%  boston     & none                           & none                           & $0.89\pm0.00$ $(0.75\pm0.00)$     \\ \hline
%  kin8nm     & none                           & $0.96\pm0.00$ $(0.84\pm0.00)$  & none                              \\ \hline    
% \hline
%             & QuantileForest                 & ConditionalGaussian            & SQR                               \\ \hline
%  concrete   & $0.96\pm0.01$ $(0.37\pm0.02)$  & $0.94\pm0.03$ $(0.32\pm0.09)$  & $0.94\pm0.03$ $(0.31\pm0.06)$     \\ \hline
%  power      & $0.94\pm0.01$ $(0.18\pm0.00)$  & $0.94\pm0.01$ $(0.18\pm0.00)$  & $0.93\pm0.01$ $(0.18\pm0.01)$     \\ \hline
%  wine       & none                           & $0.94\pm0.02$ $(0.49\pm0.03)$  & $0.93\pm0.03$ $(0.45\pm0.04)$     \\ \hline
%  yacht      & $0.97\pm0.04$ $(0.28\pm0.11)$  & $0.93\pm0.06$ $(0.03\pm0.01)$  & $0.93\pm0.06$ $(0.06\pm0.04)$     \\ \hline
%  naval      & $0.92\pm0.01$ $(0.22\pm0.00)$  & $0.96\pm0.01$ $(0.15\pm0.25)$  & $0.95\pm0.02$ $(0.12\pm0.09)$     \\ \hline
%  energy     & $0.95\pm0.02$ $(0.15\pm0.01)$  & $0.94\pm0.03$ $(0.12\pm0.18)$  & $0.94\pm0.03$ $(0.08\pm0.03)$     \\ \hline
%  boston     & $0.95\pm0.03$ $(0.37\pm0.02)$  & $0.94\pm0.03$ $(0.55\pm0.20)$  & $0.92\pm0.06$ $(0.36\pm0.09)$     \\ \hline
%  kin8nm     & none                           & $0.93\pm0.01$ $(0.20\pm0.01)$  & $0.93\pm0.01$ $(0.23\pm0.02)$     \\ \hline
% \hline
%           & \textbf{\textit{MAQR}}         & \\ \hline
% concrete   & $0.93\pm0.01$ $(0.26\pm0.01)$  & \\ \hline
% power      & $0.95\pm0.01$ $(0.28\pm0.03)$  & \\ \hline
% wine       & $0.95\pm0.02$ $(0.56\pm0.06)$  & \\ \hline
% yacht      & $0.92\pm0.03$ $(0.03\pm0.01)$  & \\ \hline
% naval      & $0.94\pm0.01$ $(0.03\pm0.00)$  & \\ \hline
% energy     & $0.94\pm0.02$ $(0.05\pm0.01)$  & \\ \hline
% boston     & $0.95\pm0.02$ $(0.34\pm0.09)$  & \\ \hline
% kin8nm     & $0.93\pm0.00$ $(0.20\pm0.01)$  & \\ \hline

% \end{tabular}
% \caption{Test Average and Standard Deviation PICP, MPIW on UCI Dataset}
% \end{center}

\subsection{Discussion on Recalibration \citep{kuleshov2018accurate}} \label{app:recal}
The recalibration algorithm by \citet{kuleshov2018accurate} utilizes isotonic regression with a validation set to fine-tune predictive uncertainties from a UQ model.
We have applied this recalibration as a post-processing step on the methods presented in Section~\ref{sec:experiments}, 
and the empirical results indicate that its effect on overall improvement in UQ quality is inconclusive.
Here, we show its effect on one of our methods, \textit{Interval}, because we observe the same pattern across all the methods, including the baseline algorithms.

Recalibration tends to improve average calibration.
This is expected, because recalibration specifically targets average calibration.
However, it does so at a cost in sharpness. This is evident in the recalibrated output moving 
upper left in the average calibration-sharpness plot in Figure~\ref{fig:uci_recal_cal_sharp}.

However, there is little to no improvement in adversarial group calibration (except for the Naval dataset) as shown in Figure~\ref{fig:uci_recal_gc}, which seems to indicate that the improvement in average calibration was not meaningful (i.e. the recalibrated result is not closer to individual calibration).
This is also the observation made by \citet{zhao2020individual}.

At the same time, the proper scoring rules improved on average (Figures~\ref{table:uci_recal_check}, \ref{table:uci_recal_int}), but interval calibration tended to worsen (Figure~\ref{table:uci_recal_int_cali}).

Based on these metrics, it is difficult to conclude on whether recalibration by \citet{kuleshov2018accurate} is 
a beneficial step or not for overall UQ quality.
If a practitioner is primarily concerned with average calibration,
the results indicate that recalibration \textit{is} a beneficial step, 
but if converging to the true conditional distribution is the primary objective, recalibration does not seem to be a robust remedy.

\begin{figure*}[h!] 
\begin{center} 
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
         & \textbf{\textit{Interval}}                   & \textbf{\textit{Interval Recalibrated}}     \\ \hline
concrete & $ 3.7 \pm 0.6	(\underline{18.1} \pm 0.6)$	& $\mathbf{3.1} \pm 0.4	(26.3 \pm 1.8)$ \\ \hline
power    & $ 2.2 \pm 0.4	(21.0 \pm 1.0)$	& $\mathbf{1.0} \pm 0.1	(\underline{20.6} \pm 0.5)$ \\ \hline
wine     & $ 5.0 \pm 0.8	(\underline{41.4} \pm 2.5)$	& $\mathbf{2.6} \pm 0.2	(50.5 \pm 1.8)$ \\ \hline
yacht    & $ 7.5 \pm 0.9	( \underline{4.5} \pm 1.0)$	& $\mathbf{4.7} \pm 0.5	( 5.6 \pm 1.1)$ \\ \hline
naval    & $ 4.7 \pm 1.4	(28.4 \pm 3.6)$	& $\mathbf{1.3} \pm 0.1	(\underline{21.9} \pm 3.3)$ \\ \hline
energy   & $ 4.3 \pm 0.6	( \underline{5.1} \pm 0.9)$	& $\mathbf{3.8} \pm 0.6	( 6.9 \pm 1.2)$ \\ \hline
boston   & $ 6.9 \pm 1.1	(\underline{20.3} \pm 0.5)$	& $\mathbf{5.4} \pm 0.9	(30.8 \pm 2.6)$ \\ \hline
kin8nm   & $ 2.9 \pm 0.4	(\underline{16.9} \pm 0.5)$	& $\mathbf{1.1} \pm 0.1	(20.6 \pm 0.3)$ \\ \hline
\end{tabular}
\caption{\textbf{UCI Average Calibration-Sharpness Table with Recalibration.} Recalibration
    tends to trade off sharpness for average calibration. 
    Better mean average calibration has been bolded, and better sharpness has been underlined.
    All values have been multiplied by 100 for readability.}
\label{table:uci_recal_cal_sharp_table}
\end{center}
\end{figure*}

\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    \includegraphics[width=\textwidth]{AISTATS2021/figs/recal_uci_cal_sharp.pdf}
    \caption{\textbf{UCI Average Calibration-Sharpness Plots with Recalibration.} Recalibration
    tends to trade off sharpness for average calibration. This is evident as the recalibrated
    predictions move \textit{upper left}.}
    \label{fig:uci_recal_cal_sharp}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    \includegraphics[width=\textwidth]{AISTATS2021/figs/recal_uci_group_cali.pdf}
    \caption{\textbf{UCI Adversarial Group Calibration with Recalibration.} Recalibration in general shows little improvement in adversarial group calibration.}
    \label{fig:uci_recal_gc}
    % \vspace{-4mm}
\end{figure*}


\begin{figure*}[h!] 
\begin{center} 
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
         & \textbf{\textit{Interval}}                   & \textbf{\textit{Interval Recalibrated}}     \\ \hline
concrete & $ 0.086 \pm 0.004 $           & $ \mathbf{0.077 \pm 0.004 }$  \\ \hline
power    & $ 0.062 \pm 0.001 $           & $ \mathbf{0.061 \pm 0.001 }$  \\ \hline
wine     & $ 0.214 \pm 0.006 $           & $ \mathbf{0.209 \pm 0.013 }$  \\ \hline
yacht    & $ \mathbf{0.018 \pm 0.003 }$  & $ \mathbf{0.018 \pm 0.004 }$  \\ \hline
naval    & $ 0.066 \pm 0.013 $           & $ \mathbf{0.062 \pm 0.012 }$  \\ \hline
energy   & $ 0.017 \pm 0.003 $           & $ \mathbf{0.016 \pm 0.003 }$  \\ \hline
boston   & $ 0.094 \pm 0.009 $           & $ \mathbf{0.076 \pm 0.014 }$  \\ \hline
kin8nm   & $ \mathbf{0.077 \pm 0.001 }$  & $ \mathbf{0.077 \pm 0.002 }$  \\ \hline
\end{tabular}
\caption{\textbf{UCI Check Score with Recalibration.} Recalibration tends to improve the check score.}
\label{table:uci_recal_check}
\end{center}
\end{figure*}

\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
          & \textbf{\textit{Interval}}                    & \textbf{\textit{Interval Recalibrated}}       \\ \hline
concrete & $ 0.943 \pm 0.053 $           & $ \mathbf{0.778 \pm 0.064}$   \\ \hline
power    & $ 0.620 \pm 0.010 $           & $ \mathbf{0.616 \pm 0.006}$   \\ \hline
wine     & $ 2.197 \pm 0.045 $           & $ \mathbf{1.921 \pm 0.024}$   \\ \hline
yacht    & $ 0.190 \pm 0.021 $           & $ \mathbf{0.158 \pm 0.025}$   \\ \hline
naval    & $ \mathbf{3.112 \pm 0.053} $  & $ 3.150 \pm 0.050$   \\ \hline
energy   & $ 0.182 \pm 0.026 $           & $ \mathbf{0.148 \pm 0.028}$   \\ \hline
boston   & $ 1.010 \pm 0.118 $           & $ \mathbf{0.931 \pm 0.107}$   \\ \hline
kin8nm   & $ 0.776 \pm 0.017 $           & $ \mathbf{0.754 \pm 0.023}$   \\ \hline
\end{tabular}
\caption{\textbf{UCI Interval Score with Recalibration.} Recalibration tends to improve the interval score.}
\label{table:uci_recal_int}
\end{center}
\end{figure*}

\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
          & \textbf{\textit{Interval}}                   & \textbf{\textit{Interval Recalibrated}}      \\ \hline
concrete & $ \mathbf{0.061 \pm 0.008 }$  & $ 0.068 \pm 0.015 $  \\ \hline
power    & $ \mathbf{0.023 \pm 0.003 }$  & $ 0.028 \pm 0.008 $  \\ \hline
wine     & $ \mathbf{0.079 \pm 0.014 }$  & $ \mathbf{0.079 \pm 0.019 }$  \\ \hline
yacht    & $ \mathbf{0.121 \pm 0.005 }$  & $ 0.136 \pm 0.025 $  \\ \hline
naval    & $ \mathbf{0.043 \pm 0.014 }$  & $ 0.105 \pm 0.016 $  \\ \hline
energy   & $ \mathbf{0.060 \pm 0.010 }$  & $ 0.066 \pm 0.005 $  \\ \hline
boston   & $ 0.079 \pm 0.015 $           & $ \mathbf{0.078 \pm 0.012 }$  \\ \hline
kin8nm   & $ \mathbf{0.048 \pm 0.006 }$  & $ 0.061 \pm 0.010 $  \\ \hline
\end{tabular}
\caption{\textbf{UCI Centered Interval Calibration with Recalibration.} Recalibration tends to worsen centered interval calibration.}
\label{table:uci_recal_int_cali}
\end{center}
\end{figure*}


==> NeurIPS2021/app_definition.tex <==
\section{Additional Definitions} \label{app:definition}

% \williex{Want an opening sentence before the bullets, such as:}\\
We give definitions for the two empirical quantities discussed in Section~\ref{sec:cali}.

The \textit{Empirical Calibration Objective}, $\mathcal{C}(D, \hQ_p, p)$,
is defined to be
\begin{align} \label{eq:emp_cal_obj}
    \begin{split}
        \mathcal{C}(D, \hQ, p) 
        & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ_p(x_i)) \mathbb{I}\{y_i > \hQ_p(x_i)\} \right] \\ 
        % &\mathcal{C}(D, \hQ, p) = \\
        % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ_p(x_i) - y_i) \mathbb{I}\{\hQ_p(x_i) > y_i\} \right].
    \end{split}
\end{align}

The \textit{Empirical Sharpness Objective}, $\mathcal{P}(D, \hQ_p, p)$, is defined to be
\begin{align} \label{eq:emp_sharp_obj}
    &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} 
        \begin{cases} 
            \hQ_{1-p}(x_i) - \hQ_p(x_i) \hspace{5pt} (p \leq 0.5)\\
            \hQ_p(x_i) - \hQ_{1-p}(x_i) \hspace{5pt} (p > 0.5).
        \end{cases}
\end{align}

% \begin{itemize}
% \item
% Empirical Calibration Objective, $\mathcal{C}(D, \hQ_p, p):$
% \begin{align} \label{eq:emp_cal_obj}
%     \begin{split}
%         \mathcal{C}(D, \hQ, p) 
%         & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         % &\mathcal{C}(D, \hQ, p) = \\
%         % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
%     \end{split}
% \end{align}

% \item
% Empirical Sharpness Objective, $\mathcal{P}(D, \hQ_p, p):$
% \begin{align} \label{eq:emp_sharp_obj}
%     &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} 
%         \begin{cases} 
%             \hQ(x_i, 1-p) - \hQ(x_i, p) \hspace{5pt} (p \leq 0.5)\\
%             \hQ(x_i, p) - \hQ(x_i, 1-p) \hspace{5pt} (p > 0.5)
%         \end{cases}
% \end{align}

% \end{itemize}

==> NeurIPS2021/app_epistemic.tex <==
\section{Considerations for Epistemic Uncertainty} \label{app:epistemic}

\subsection{Sources for Epistemic Uncertainty}
The primary focus of this paper is on learning a quantile model.
For any single setting of the parameters of the quantile model, the model outputs the 
current best estimate of the \textit{true underlying distribution} of the dataset.
Following the notation laid out in Section~\ref{sec:prelim}, the learned quantile model $\hQ$
is a best approximation to $\Q$, the quantile function of the true distribution.

Meanwhile, epistemic uncertainty refers to the uncertainty \textit{in making the distributional prediction, $\hQ$}.
\citet{pearce2018high} provides one method of decomposing the sources of epistemic uncertainty in a regression setting:
\begin{itemize}
        \item \emph{Model misspecification:} $\hQ$ may lack the flexibility to
        accurately model $
        \Q$, leading to systematic bias.
        
        \item  \emph{Data uncertainty:} $\hQ$ may not be estimated using a
        representative sample $\{ x_i, y_i \}$ from the assumed underlying distribution.
        
        \item \emph{Parameter uncertainty:} $\hQ$ may not be estimated using
        a large enough quantity of samples, leading to uncertainty about the estimated quantity.
\end{itemize}

\citet{pearce2018high} has argued that, 
given the rich class of function approximators 
at hand today (NN, deep trees, ensembles), model misspecification can be ignored, which we believe is reasonable. 
In modeling the remaining sources of uncertainties in $\hQ$, 
we can incorporate common standard methods to quantify epistemic uncertainty, 
including boostrapping the data, creating an ensemble of estimates for $\hQ$ with random parameter initializations, or fitting a residual process \citep{liu2019accurate}.  
Here, we describe one combination of these methods: 
an ensemble of estimates of the learned quantile function 
$\{\hQ^{(1)}, \hQ^{(2)},...\}$ each trained with random initialization (to address parameter uncertainty), on a bootstrapped sample of the training data 
(to address data uncertainty).
The uncertainty over this set of models is the epistemic uncertainty.

\subsection{Expressing and Utilizing Epistemic Uncertainty} \label{app:boot_ens}
Once we decide on methods to quantify the epistemic uncertainty, 
the next question is \textit{how to express the epistemic uncertainty}, 
especially when combining it with the current prediction of the aleatoric uncertainty.
This is still an open research question, especially in the regression setting, 
and methods of combining aleatoric with epistemic uncertainty will differ 
for how the uncertainty is represented (e.g. density estimates, quantiles, prediction intervals). 

One method of combination is to consider the utility of quantifying epistemic uncertainty.
Intuitively, for a given input, if we have high epistemic uncertainty, 
the combined uncertainty should be higher (i.e. less confident prediction), and vice versa.
If we consider a single quantile, it is unclear whether lower confidence
(due to epistemic uncertainty) would equate to a lower or higher quantile estimate.
However, if we consider constructing a centered prediction interval for total uncertainty,
it is straightforward to see that lower confidence should widen the interval, 
by raising the upper bound (quantile level above $0.5$) 
and lowering the lower bound (quantile level below $0.5$).
This conservative upper and lower bound can be constructed with 
the bootstrap distribution of each quantile according to each ensemble member prediction.
This is also the method utilized in \citet{pearce2018high}.

Suppose we have an ensemble of $M$ quantile models: 
$\{\hQ^{(1)}, \hQ^{(2)}, \dots, \hQ^{(M)}\}$.
For any test point $x^{*}$ and test coverage level $(1-\alpha^{*})$,
the total uncertainty represented by a centered prediction interval with upper bound $\hat{u}$ and lower bound $\hat{l}$ is constructed as:
\begin{align*}
    \hat{l} &= \bar{\mu}(x^{*}, \alpha^{*}/2) - z \frac{s(x^{*}, \alpha^{*}/2)}{\sqrt{M}} \\
    \hat{u} &= \bar{\mu}(x^{*}, 1 - \alpha^{*}/2) + z \frac{s(x^{*}, 1 - \alpha^{*}/2)}{\sqrt{M}} \\
    &\bar{\mu}(x^{*}, p^*) = \frac{1}{M}\sum_{i=1}^{M} \hQ^{(i)}(x^{*}, p^{*}) \\
    &s(x^{*}, p^*) = \sqrt{\frac{1}{M-1}\sum_{i=1}^{M} (\hQ^{(i)}(x^{*}, p^{*}) - \bar{\mu}(x^{*}, p^{*}))^{2}}
\end{align*}
and $z$ is the chosen critical value (e.g. $1.96$ for a conservative bound that takes the $95\%$ confidence interval of the bootstrap distribution).
In words, the construction of $\hat{u}, \hat{l}$ equates to constructing a
conservative prediction interval that depends on how dispersed or concentrated each ensemble member's predictions are.


\subsection{Metrics for Total Uncertainty Evaluation} \label{app:epist_metric}
After choosing a method to express epistemic uncertainty and combining it with 
aleatoric uncertainty for a prediction of total uncertainty, 
next comes the question of \textit{how to evaluate the combined uncertainty}.

The critical point here is that the calibration, sharpness and 
proper scoring rule metrics we have discussed thus far \textit{are not applicable here}. 
This is because these metric only judge how close the prediction is to the true
underlying distribution.
In fact, ECE (a measure of average calibration) can be shown to be identical to
the Wasserstein distance between distributions under the $L1$ distance metric \citep{zhao2020individual}.
In a hypothetical setting where we have very few datapoints and hence 
very high epistemic uncertainty throughout the whole data support, 
if one distributional prediction was extremely lucky and predicted a distribution that
adheres exactly to the true underlying distribution, the aforementioned metrics
will consider this prediction a perfect prediction -- 
however, a lucky guess is not at all a useful UQ, and to a practitioner,
a less confident prediction (by quantifying high epistemic uncertainty) is much more useful, 
rather than a very confident prediction that can be correct if it is lucky, 
but confidently very incorrect otherwise.

We also emphasize here that, while standard evaluation experiments and metrics exist for the
\textit{classification} setting (e.g. by training an image classifier on the MNIST dataset
and testing on the Non-MNIST dataset to assess the entropy of the predicted class probabilities or 
the output of a trained out-of-distribution detector), 
there does not exists standard experiments and metrics to evaluate epistemic uncertainty in the  \textit{regression setting}.

Therefore, we propose one evaluation metric to assess combined total uncertainty, which is \textit{sharpness subject to sufficient coverage} and we will refer to this metric as ``epistemic coverage''.
Epistemic coverage measures average calibration of a centered prediction interval, but the difference in observed probabilities from expected probabilities is penalized only when the observed probability is less than
the expected probability (i.e. do not penalize the prediction if the observed probability is
higher than the expected probability), and if this sufficient coverage condition is 
met, then we evaluate sharpness. 

By this metric, only over-confidence is penalized and under-confidence 
is considered acceptable. However, since infinitely wide prediction intervals 
are also not useful, we also consider sharpness after sufficient coverage is met.

\subsection{Demonstrating Effect of Bootstrap Ensembling and the Epistemic Coverage Metric}
We design an ``epistemic experiment'' to show the effect of incorporating epistemic uncertainty via 
bootstrapped ensembles.
In this experiment, we swap the train and test sets, such that the training set is much smaller than the test set (roughly $\frac{1}{7}$ of test set size), hence, the model should have very high epistemic uncertainty in making predictions on the test set.
It is expected that by not incorporating epistemic uncertainty in such a setting, 
the model will produce \textit{overconfident} predictions that are \textit{too sharp}.
This overconfidence will be penalized heavily by the epistemic coverage metric we described above in Appendix~\ref{app:epist_metric}, and sharpness should also indicate that the predictions are 
too tight.
Producing conservative distributional predictions via the bootstrapped ensembling technique described above 
in Appendix~\ref{app:boot_ens} is expected to mitigate these overconfidence issues
by incorporating epistemic uncertainty.

We show the effect on one of our methods, \textit{Interval}, because the same effect can be observed for any of the quantile methods, including the baseline algorithms.
The results are shown in Figure~\ref{fig:epist_uci_cal_sharp}.

When a conservative PI is constructed with the bootstrapped ensemble (labelled \textit{Interval Boot-Ens}), the epistemic coverage error decreases significantly to or near zero, which is expected given that the conservative bounds only work to widen the PI, and the epistemic coverage error only penalizes PI that are not wide enough.
The increase in width is also evident in the increase in sharpness with bootstrap ensembling.

Therefore, the ensembling technique does work to incorporate epistemic uncertainty
from a practical standpoint by imbuing more underconfidence into the distributional predictions.
Still, quantifying and evaluating epistemic uncertainty in a regression setting is an 
open problem, and we leave for future work developing alternative methods of quantifying 
epistemic uncertainty in regression.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{AISTATS2021/figs/epist_uci_cal_sharp.pdf}
    \caption{\textbf{Epistemic Experiments on UCI Datasets.} We evaluate epistemic coverage in
    the epistemic experiment setting where the train set is much smaller than the test set. Epistemic coverage only penalizes overconfidence. Sharpness is the average width of the 95\% PI.}
    \label{fig:epist_uci_cal_sharp}
    % \vspace{-4mm}
\end{figure*}


==> NeurIPS2021/app_exp_details.tex <==
\section{Details on Datasets and Setup of Main Experiments} \label{app:data_exp_details}

\subsection{UCI Experiment Details} \label{app:uci_exp_details}
Here, we provide details on the setup of the UCI experiments presented in Section~\ref{sec:uci_fusion}.

For each of the 8 UCI datasets, we split $10\%$ of the data into the test set, and we further split $20\%$ of the remaining $90\%$ of the data for the validation, resulting in a train/validation/test split of proportions $72\%, 18\%, 10\%$.
For all tasks and all 8 datasets, the data was preprocessed by centering to zero mean and scaling to unit variance. 

We used the same NN architecture across all methods: 2 layers of 64 hidden units with ReLU non-linearities.
We used the same learning rate, $1e^{-3}$, and the same batch size, 64, for all methods. 
For all methods, training was stopped early if the validation loss did not decrease for more than $200$ epochs, until a maximum of $10000$ epochs.
If training was stopped early, the final model was backtracked to the model with lowest validation loss.

\textit{IndvCal} (individual calibration) has one hyperparameter, $\alpha$, which balances
the NLL loss and the individual calibration loss in the loss function.
We 5-fold cross-validated $\alpha$ in [0.0, 1.0] in 20 equi-spaced intervals based on  
Pareto optimality in test set NLL and adversarial group calibration.
If there were multiple $\alpha$ values that were Pareto optimal, we chose the value
that had the best test set adversarial group calibration.

\textit{Cali} (penalized calibration loss) has one hyperparameter, $\lambda$, which balances the calibration loss and sharpness penalty in the loss function.
We tuned $\lambda$ according to the same grid as above for $\alpha$, based on the criterion of adversarial group calibration.
Note that adversarial group calibration will not always favor lower values of $\lambda$
as $\lambda=0$ will only target average calibration, which, in the degenerate case, may converge
to the marginal distribution of $\F_{\bold{Y}}$. This state will achieve very poor adversarial group calibration. 

Group batching was applied to \textit{Interval} (interval score) and \textit{Cali} according to the implementation detailed in Appendix~\ref{app:group_batching}.
During training, we alternated between ``group batching epochs'' and ``regular batching epochs'' (where batches are drawn uniformly from the training set), 
and the frequency of group batching epochs was a hyperparameter we tuned with cross-validation in [1, 2, 3, 5, 10, 30, 100], based on the criterion of 
adversarial group calibration.

\textit{MAQR} has a two-step training process: we first learn a mean model, then construct a quantile dataset $D$, then regress onto this dataset with the quantile model. 
Both the mean model and the quantile model had the same NN architecture as mentioned above.
The mean model was trained with the MSE loss according to the same, aforementioned training procedure. 
For each UCI dataset, we learned one mean model from the first seed, and re-used this mean model for all other seeds.
Using this mean model, we then populated the quantile dataset according to the method outlined in Algorithm~\ref{alg:maqr_main}.
Algorithm~\ref{alg:maqr_main} requires one hyperparameter: the distance threshold in $\mathcal{X}$ space ($d_N$ in Line 2 of Algorithm~\ref{alg:CondQuantEst}). 
We tuned this hyperparameter by setting the minimum distance required to include $k$ number of points, on average, in constructing an empirical CDF at each training point. 
We tuned this parameter with cross-validation using the grid $k \in [10, 20, 30, 40, 50]$.
The quantile model was trained according to the same training procedure but with one difference: the batch size was set to 1024 because the quantile dataset $D$ could become very large due to many conditional quantile estimates at each training point.

All methods, for all datasets were repeated with 5 seeds: [0, 1, 2, 3, 4].

\subsection{Fusion Experiment Details} \label{app:fusion_exp_details}
We first describe the fusion dataset from Section~\ref{sec:uci_fusion}, then
the details of the fusion experiment set up.

The fusion dataset was recorded from the DIII-D tokamak in San Diego, CA, USA, and describes the dynamics of plasma during a nuclear fusion reaction within the tokamak.
Consent and access to use this dataset was obtained via
collaborations with the Princeton Plasma Physics Lab.

While the dataset in its raw format is a time-series of the state variables and action variables, for the purposes of a supervised learning problem to learn the dynamics of plasma, it has been re-structrued into a \textit{(state, action, next state)} format. 
Therefore, the modeling task at hand is to learn the mapping \textit{(state, action)} to \textit{(next state)}, and the UQ task is then to learn the distribution 
over the next state given the current state and action.

There are 10 plasma state variables that we use both as the input state variables and the target variables. For the action variables, we use the power level of 8 neutral beams, which are a primary means of controlling plasma in a tokamak. These variables are described in Figure~\ref{tab:fusion_variables}.


\begin{figure*} 
\begin{center}
\begin{tabular}{ |c|c| }
 \hline
            & \textbf{State Variables} \\\hline
 aminor     &  Minor Radius   \\ \hline
 dssdenest  &  Line Averaged Electron Density   \\ \hline
 efsbetan   &  Normalized Beta   \\ \hline
 efsli      &  Internal Inductance   \\ \hline
 efsvolume  &  Plasma Volume   \\ \hline
 ip         &  Plasma Curent   \\ \hline
 kappa      &  Elongation   \\ \hline
 R0         &  Major Radius   \\ \hline
 tribot     &  Bottom Triangularity   \\ \hline
 tritop     &  Top Triangularity   \\ \hline
\end{tabular}
\vspace{2mm}

\begin{tabular}{ |c|c| } 
\hline
            & \textbf{Action Variables} \\\hline
 pinj\_15l   &  Co-current Beam 1 Power   \\ \hline
 pinj\_15r   &  Co-current Beam 2 Power   \\ \hline
 pinj\_21l   &  Counter-current Beam 1 Power   \\ \hline
 pinj\_21r   &  Counter-current Beam 2 Power   \\ \hline
 pinj\_30l   &  Co-current Beam 3 Power   \\ \hline
 pinj\_30r   &  Co-current Beam 4 Power   \\ \hline
 pinj\_33l   &  Co-current Beam 5 Power   \\ \hline
 pinj\_33r   &  Co-current Beam 6 Power   \\ \hline
\end{tabular}  
\caption{\textbf{State and Action Variables for Fusion Dataset.} 10 variables describe the current state of plasma, and the action space is 8 dimensional.}
 \label{tab:fusion_variables}
\end{center}
\end{figure*}



% \begin{figure*}[h!]
% \begin{center} \label{table:uci_int_cali}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & Interval                   & Interval Recalibrated      \\ \hline
%  concrete & $ \mathbf{0.061 (0.008)}$  & $ 0.068 (0.015)$  \\ \hline
%  power    & $ \mathbf{0.023 (0.003)}$  & $ 0.028 (0.008)$  \\ \hline
%  wine     & $ \mathbf{0.079 (0.014)}$  & $ \mathbf{0.079 (0.019)}$  \\ \hline
%  yacht    & $ \mathbf{0.121 (0.005)}$  & $ 0.136 (0.025)$  \\ \hline
%  naval    & $ \mathbf{0.043 (0.014)}$  & $ 0.105 (0.016)$  \\ \hline
%  energy   & $ \mathbf{0.060 (0.010)}$  & $ 0.066 (0.005)$  \\ \hline
%  boston   & $ 0.079 (0.015)$           & $ \mathbf{0.078 (0.012)}$  \\ \hline
%  kin8nm   & $ \mathbf{0.048 (0.006)}$  & $ 0.061 (0.010)$  \\ \hline
% \end{tabular}
% \caption{\textbf{UCI Interval Calibration} Caption}
% \end{center}
% \end{figure*}



As input to the dynamics model, we model the current state as a 200 millisecond (ms) history window of the 10 state variables and 8 action variables, 
and we model the current action as a 200ms window into the future of the 8 action variables. 
The target variables are modeled as the change (or delta) of the state variables 200ms in the future. 
The state and action features are engineered according to the method used by~\citet{fu2020machine}. 
Each 200ms window is taken as one ``frame'', the 200ms window is further divided into 2 ``frames'' of equal length (100ms each), as well as thirds. 
Then we calculate the mean, variance, and slope of each state and action variable for each of these frames, and collect these statistics as the features. 
Hence, each 200ms window for 1 variable is summarized into 18 features (3 statistics per frame, and 6 frames per 200ms window).
Since there are 10 state variables and 8 action variables, and since the state window is 200ms long and the action window is 200ms long, the input is a 468 dimensional array (10 state variables + 8 previous action variables + 8 current action variables for a total of 26 input variables, and 18 features per variable). 
Once these features are created, we centered and scaled the inputs and targets to zero mean and unit variance. 

There were a total of $100$K training data points, and $10$K validation and $10$K test data points.

The training and hyperparameter tuning procedures were exactly the same as 
the UCI experiments (detailed above in Appendix~\ref{app:uci_exp_details}), except for two differences: 1) we have increased the NN capacity to 3 hidden layers of 100 hidden units and 2) the batch size was set to 500.

The fusion experiment was likewise repeated 5 times with the seeds [0, 1, 2, 3, 4].

\subsection{Group Batching Implementation Details} \label{app:group_batching}
Group batching, as introduced in Section~\ref{sec:group_batch}, 
is a general procedure in which deliberate subsets of the training data
are constructed and batched from during train time. 
There is no ``correct'' method to form these subsets, because the main
point is to simply \textit{not draw batches from $\F_{\bold{X}}$}.
One could consider thresholding the values of each dimension of the domain
and discretizing the subsets according to the thresholds, 
and also taking unions of these discretizations to form new subsets as well.

This implementation can be computationally demanding, 
because for each threshold setting, one has to make sure
to choose a subset with sufficiently many points, and iteratively
increase or decrease the dimension thresholds if no subset with
sufficiently many points can be found.
This computational cost increases significantly with dimension.

Our implementation of group batching for all our experiments were as follows: we sort the datapoints according to a single dimension, 
then take consecutive sets of size equal to the batch size, and use these 
sets as the batches to take gradient steps over during an epoch.
We repeat the above process by cycling through each dimension for sorting.
While this process is very simple and inexpensive and only considers 
a single dimension in constructing the subsets, 
this group batching scheme has shown to be very effective in our 
experiments.
% Group batching in right plot of Figure~\ref{fig:demo} has also been performed in this exact same way.

\subsection{Calculation of Evaluation Metrics} \label{app:measuring_metrics}

To measure the calibration metrics (average, adversarial group, centered interval),
we discretized the expected probabilities from $0.01$ to $0.99$ in $0.01$ increments
(i.e. $0.01$, $0.02$, $\dots$, $0.97$, $0.98$, $0.99$)
and calculated ECE according to this finite discretization.

To measure centered interval calibration, for each expected probability $p$, 
we predict centered $100 \times p \%$ PIs, and calculate $\hat{p}^{\text{obs}}_{avg}$ 
as the proportion of test points falling within the PI, 
i.e. $\hat{p}^{\text{obs}}_{avg}(p)$ here would be calculated as 
\begin{align*}
    \hat{p}^{\text{obs}}_{avg}(p) \text{   for centered intervals   } = \frac{1}{N}\sum_{i=1}^{N} \mathbb{I}\{ \hQ(x_i, 0.5-p/2) \leq y_i \leq \hQ(x_i, 0.5 + p/2)\}.
\end{align*}



The procedure in which we measure adversarial group calibration is the following.
For a given test set, we scale group size between $1\%$ and $100\%$ of the full test set size, in 10 equi-spaced intervals, and for each group size, we draw 20 random groups from the test set and record the worst calibration incurred across these 20 random groups. This is also the method used by \citet{zhao2020individual} to measure adversarial group calibration.

Sharpness was measured as the mean width of the $95\%$ centered PI (i.e. between  $p=0.025$ and $0.975$). 

The proper scoring rules (check score, interval score) were measured as the average of the score on the test set.

\subsection{Discussion of Compute and Resources}
\label{app:compute}
All experiments were run on a single NVIDIA GeForce GTX 1080Ti GPU, with a Intel(R) Xeon(R) Silver 4110 CPU.
The fusion datasets were the largest (100K training) and highest dimensional (468 dimensional) and took the longest to run: training one model to convergence took roughly $\sim1$ hour.




==> NeurIPS2021/app_exp_results.tex <==
\section{Full Experimental Results}
\label{app:all_experiments}

In this section, we provide all of the experimental results from 
Section~\ref{sec:experiments}, for all metrics:
1) average calibration - sharpness, 2) adversarial group calibration, 3) check score, 4) interval score, and 5) centered interval calibration

For average calibration and sharpness, we present the numeric tables
again, along with a visualization which plots calibration and sharpness
along the $x$ and $y$ axes. 


\subsection{Full UCI Experiment Results}
\label{app:all_uci_results}


\begin{figure*}[ht!]
    \centering
    
    \includegraphics[width=\textwidth]{arXiv/figs/full_calibration_table_uci.pdf}
    
    \caption{\textbf{UCI Average Calibration-Sharpness Table.}
    The table shows mean average calibration (measured by ECE) and sharpness in parentheses, along with $\pm 1$ standard error. 
    The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined. 
    All values have been multiplied by 100 for readability (same table as Figure~\ref{fig:uci_table_figure} (Top), repeated here for completeness).
    }
    \label{fig:uci_ece_sharp_table_full_app}
    \vspace{-1mm}
    % \vspace{-4mm}
\end{figure*}

\begin{figure}[H]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/uci_cal_sharp.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/uci_cal_sharp_all_8.pdf}
    \caption{\textbf{UCI Average Calibration-Sharpness Plot.} Visualization of average calibration-sharpness from UCI experiments in Section~\ref{sec:uci_fusion}}
    \label{fig:full_uci_cal_sharp}
    % \vspace{-4mm}
\end{figure}
% \vspace{-4mm}

\begin{figure}[H]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/uci_group_cali.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/uci_group_cali_all_8.pdf}
    \caption{
    \textbf{UCI Adversarial Group Caibration.}
    The plot displays the worst calibration error incurred for any group of any given size. The mean is plotted along with $\pm1$ standard error in shades. Group size here refers to the proportion of the test dataset size
    (full results for Figure~\ref{fig:uci_table_figure} (Bottom)).
    }
    \label{fig:full_uci_gc}
    % \vspace{-4mm}
\end{figure}

\begin{figure*}[h!]
\begin{center} \label{table:full_uci_check}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
% & \textit{SQR}                 & \textit{IndvCal}            & \textbf{\textit{Interval}}      & \textbf{\textit{Cali}}     & \textbf{\textit{MAQR}}        \\\hline
% concrete & $0.085 (0.006)$   & $0.085 (0.005)$    & $ 0.086 (0.004)$  & $ 0.118 (0.006)$  & $\textbf{ 0.059 (0.008)}$    \\ \hline
% power    & $\mathbf{0.057 (0.001)}$   & $ 0.070 (0.001) $  & $ 0.062 (0.001)$  & $ 0.064 (0.001)$  & $0.058 (0.001)$    \\ \hline
% wine     & $0.205 (0.008)$   & $ 0.219 (0.004) $  & $ 0.214 (0.006)$  & $ 0.210 (0.008)$  & $\textbf{ 0.191 (0.003)}$    \\ \hline
% yacht    & $0.012 (0.002)$   & $ 0.015 (0.002) $  & $ 0.018 (0.003)$  & $ 0.019 (0.004)$  & $\textbf{ 0.007 (0.001)}$    \\ \hline
% naval    & $0.070 (0.001)$   & $ 0.276 (0.004) $  & $ 0.066 (0.013)$  & $ 0.159 (0.029)$  & $\textbf{ 0.004 (0.000)}$    \\ \hline
% energy   & $0.014 (0.000)$   & $ 0.015 (0.001) $  & $ 0.017 (0.003)$  & $ 0.017 (0.002)$  & $\textbf{ 0.010 (0.001)}$    \\ \hline
% boston   & $0.088 (0.008)$   & $ 0.095 (0.008) $  & $ 0.094 (0.009)$  & $ 0.103 (0.013)$  & $\textbf{ 0.063 (0.016)}$    \\ \hline
% kin8nm   & $0.078 (0.001)$   & $ 0.104 (0.003) $  & $ 0.077 (0.001)$  & $ 0.096 (0.005)$  & $\textbf{ 0.070 (0.001)}$    \\ \hline
         & \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}      & \textbf{\textit{Cali}}     & \textbf{\textit{MAQR}}        \\\hline
concrete & $0.085 (0.006)$              & $ 0.085 \pm 0.005 $    & $ 0.086 \pm 0.004 $  & $ 0.118 \pm 0.006$  & $\mathbf{ 0.059 \pm 0.008 }$    \\ \hline
power    & $\mathbf{0.057 \pm 0.001 }$  & $ 0.070 \pm 0.001 $    & $ 0.062 \pm 0.001 $  & $ 0.064 \pm 0.001$  & $0.058 \pm 0.001 $              \\ \hline
wine     & $0.205 \pm 0.008 $           & $ 0.219 \pm 0.004 $    & $ 0.214 \pm 0.006 $  & $ 0.210 \pm 0.008$  & $\mathbf{ 0.191 \pm 0.003}$    \\ \hline
yacht    & $0.012 \pm 0.002 $           & $ 0.015 \pm 0.002 $    & $ 0.018 \pm 0.003 $  & $ 0.019 \pm 0.004$  & $\mathbf{ 0.007 \pm 0.001}$    \\ \hline
naval    & $0.070 \pm 0.001 $           & $ 0.276 \pm 0.004 $    & $ 0.066 \pm 0.013 $  & $ 0.159 \pm 0.029$  & $\mathbf{ 0.004 \pm 0.000}$    \\ \hline
energy   & $0.014 \pm 0.000 $           & $ 0.015 \pm 0.001 $    & $ 0.017 \pm 0.003 $  & $ 0.017 \pm 0.002$  & $\mathbf{ 0.010 \pm 0.001}$    \\ \hline
boston   & $0.088 \pm 0.008 $           & $ 0.095 \pm 0.008 $    & $ 0.094 \pm 0.009 $  & $ 0.103 \pm 0.013$  & $\mathbf{ 0.063 \pm 0.016}$    \\ \hline
kin8nm   & $0.078 \pm 0.001 $           & $ 0.104 \pm 0.003 $    & $ 0.077 \pm 0.001 $  & $ 0.096 \pm 0.005$  & $\mathbf{ 0.070 \pm 0.001}$    \\ \hline
\end{tabular}
\caption{\textbf{UCI Check Score.} Full check score results of UCI experiments from Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{MAQR} tends to achieve the best check score, 
    which is surprising given that \textit{SQR} utilizes the
    same model class to optimize the check score directly.}
\end{center}
% \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
\begin{center} \label{table:full_uci_int}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
%           & \textit{SQR}                 & \textit{IndvCal}            & \textbf{\textit{Interval}}      & \textbf{\textit{Cali}}     & \textbf{\textit{MAQR}}        \\\hline
%  concrete & $ 2.038 (0.225) $   & $ 1.157 (0.069) $  & $ 0.943 (0.053)$  & $ 1.465 (0.086)$  & $ \textbf{ 0.672 (0.118})$    \\ \hline
%  power    & $ 0.834 (0.022) $   & $ 0.917 (0.021) $  & $ 0.620 (0.010)$  & $ 0.699 (0.019)$  & $ \textbf{0.592 (0.009)}$    \\ \hline
%  wine     & $ 3.242 (0.166) $   & $ 3.168 (0.019) $  & $ 2.197 (0.045)$  & $ 2.498 (0.135)$  & $ \textbf{2.052 (0.052)}$    \\ \hline
%  yacht    & $ 0.314 (0.061) $   & $ 0.197 (0.036) $  & $ 0.190 (0.021)$  & $ 0.298 (0.063)$  & $ \textbf{0.086 (0.016)}$    \\ \hline
%  naval    & $ 0.097 (0.011) $   & $ 3.112 (0.053) $  & $ 0.620 (0.114)$  & $ 1.560 (0.268)$  & $ \textbf{0.044 (0.001)}$    \\ \hline
%  energy   & $ 0.290 (0.016) $   & $ 0.223 (0.017) $  & $ 0.182 (0.026)$  & $ 0.204 (0.018)$  & $ \textbf{0.101 (0.006)}$    \\ \hline
%  boston   & $ 1.833 (0.299) $   & $ 1.395 (0.176) $  & $ 1.010 (0.118)$  & $ 1.449 (0.259)$  & $ \textbf{0.864 (0.287)}$    \\ \hline
%  kin8nm   & $ 1.241 (0.041) $   & $ 1.347 (0.031) $  & $ 0.776 (0.017)$  & $ 1.121 (0.072)$  & $ \textbf{0.691 (0.015)}$    \\ \hline
& \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}      & \textbf{\textit{Cali}}     & \textbf{\textit{MAQR}}        \\\hline
concrete & $ 2.038 \pm 0.225 $   & $ 1.157 \pm 0.069 $  & $ 0.943 \pm 0.053 $  & $ 1.465 \pm 0.086 $  & $ \mathbf{ 0.672 \pm 0.118 }$    \\ \hline
power    & $ 0.834 \pm 0.022 $   & $ 0.917 \pm 0.021 $  & $ 0.620 \pm 0.010 $  & $ 0.699 \pm 0.019 $  & $ \mathbf{0.592 \pm 0.009 }$    \\ \hline
wine     & $ 3.242 \pm 0.166 $   & $ 3.168 \pm 0.019 $  & $ 2.197 \pm 0.045 $  & $ 2.498 \pm 0.135 $  & $ \mathbf{2.052 \pm 0.052 }$    \\ \hline
yacht    & $ 0.314 \pm 0.061 $   & $ 0.197 \pm 0.036 $  & $ 0.190 \pm 0.021 $  & $ 0.298 \pm 0.063 $  & $ \mathbf{0.086 \pm 0.016 }$    \\ \hline
naval    & $ 0.097 \pm 0.011 $   & $ 3.112 \pm 0.053 $  & $ 0.620 \pm 0.114 $  & $ 1.560 \pm 0.268 $  & $ \mathbf{0.044 \pm 0.001 }$    \\ \hline
energy   & $ 0.290 \pm 0.016 $   & $ 0.223 \pm 0.017 $  & $ 0.182 \pm 0.026 $  & $ 0.204 \pm 0.018 $  & $ \mathbf{0.101 \pm 0.006 }$    \\ \hline
boston   & $ 1.833 \pm 0.299 $   & $ 1.395 \pm 0.176 $  & $ 1.010 \pm 0.118 $  & $ 1.449 \pm 0.259 $  & $ \mathbf{0.864 \pm 0.287 }$    \\ \hline
kin8nm   & $ 1.241 \pm 0.041 $   & $ 1.347 \pm 0.031 $  & $ 0.776 \pm 0.017 $  & $ 1.121 \pm 0.072 $  & $ \mathbf{0.691 \pm 0.015 }$    \\ \hline
\end{tabular}
\caption{\textbf{UCI Interval Score} Full interval score results 
of UCI experiments from Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{MAQR} tends to achieve the best interval score, 
    which is surprising given that \textit{Interval} utilizes the
    same model class to optimize the interval score directly.}
\end{center}
% \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
\begin{center} \label{table:uci_int_cali}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
& \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}      & \textbf{\textit{Cali}}     & \textbf{\textit{MAQR}}        \\\hline
concrete & $ 0.186 \pm 0.031 $   & $ 0.089 \pm 0.005 $  & $ 0.061 \pm 0.008 $  & $ 0.096 \pm 0.013 $  & $ \mathbf{0.059 \pm 0.020 }$    \\ \hline
power    & $ 0.045 \pm 0.004 $   & $ 0.068 \pm 0.008 $  & $ 0.023 \pm 0.003 $  & $ 0.037 \pm 0.002 $  & $ \mathbf{0.010 \pm 0.002 }$    \\ \hline
wine     & $ 0.053 \pm 0.006 $   & $ 0.169 \pm 0.008 $  & $ 0.079 \pm 0.014 $  & $ 0.065 \pm 0.007 $  & $ \mathbf{0.045 \pm 0.005 }$    \\ \hline
yacht    & $ 0.135 \pm 0.009 $   & $ 0.100 \pm 0.020 $  & $ 0.121 \pm 0.005 $  & $ 0.129 \pm 0.016 $  & $ \mathbf{0.085 \pm 0.024 }$    \\ \hline
naval    & $ 0.128 \pm 0.031 $   & $ 0.039 \pm 0.003 $  & $ 0.043 \pm 0.014 $  & $ 0.110 \pm 0.013 $  & $ \mathbf{0.012 \pm 0.002 }$    \\ \hline
energy   & $ 0.174 \pm 0.011 $   & $ 0.163 \pm 0.009 $  & $ 0.060 \pm 0.010 $  & $ 0.090 \pm 0.011 $  & $ \mathbf{0.052 \pm 0.018 }$    \\ \hline
boston   & $ 0.163 \pm 0.020 $   & $ \mathbf{0.050 \pm 0.007 } $  & $ 0.079 \pm 0.015 $  & $ 0.138 \pm 0.028 $  & $ 0.092 \pm 0.041 $    \\ \hline
kin8nm   & $ 0.070 \pm 0.005 $   & $ 0.080 \pm 0.002 $  & $ 0.048 \pm 0.006 $  & $ 0.067 \pm 0.005 $  & $ \mathbf{0.019 \pm 0.008 }$    \\ \hline
\end{tabular}
\caption{\textbf{UCI Centered Interval Calibration} Full centered interval calibration results 
of UCI experiments from Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{MAQR} tends to achieve the best centered interval calibration. \label{table:app_uci_centered_interval}}
\end{center}
\end{figure*}

% Interval Calibration
% \begin{figure*}[ht!]
% \begin{center} \label{table:int_cali}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & SQR                 & IndvCal            & \textbf{Int}      & \textbf{Cali}     & \textbf{MAQR}        \\\hline
%  concrete & $ 0.18 (0.03) $   & $ 0.08 (0.00) $  & $ 0.06 (0.00)$  & $ 0.09 (0.01)$  & $ 0.05 (0.02)$    \\ \hline
%  power    & $ 0.04 (0.00) $   & $ 0.06 (0.00) $  & $ 0.02 (0.00)$  & $ 0.03 (0.00)$  & $ 0.01 (0.00)$    \\ \hline
%  wine     & $ 0.05 (0.00) $   & $ 0.16 (0.00) $  & $ 0.07 (0.01)$  & $ 0.06 (0.00)$  & $ 0.04 (0.00)$    \\ \hline
%  yacht    & $ 0.13 (0.00) $   & $ 0.10 (0.02) $  & $ 0.12 (0.00)$  & $ 0.12 (0.01)$  & $ 0.08 (0.02)$    \\ \hline
%  naval    & $ 0.12 (0.03) $   & $ 0.03 (0.00) $  & $ 0.04 (0.01)$  & $ 0.11 (0.01)$  & $ 0.01 (0.00)$    \\ \hline
%  energy   & $ 0.17 (0.01) $   & $ 0.16 (0.00) $  & $ 0.06 (0.01)$  & $ 0.09 (0.01)$  & $ 0.05 (0.01)$    \\ \hline
%  boston   & $ 0.16 (0.02) $   & $ 0.05 (0.00) $  & $ 0.07 (0.01)$  & $ 0.13 (0.02)$  & $ 0.09 (0.04)$    \\ \hline
%  kin8nm   & $ 0.07 (0.00) $   & $ 0.08 (0.00) $  & $ 0.04 (0.00)$  & $ 0.06 (0.00)$  & $ 0.01 (0.00)$    \\ \hline
% \end{tabular}
% \end{center}
% \end{figure*}


% \begin{center} \label{table:int}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & SQR                 & IndvCal            & Int               & Cali              & MAQR        \\\hline
%  concrete & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  power    & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  wine     & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  yacht    & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  naval    & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  energy   & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  boston   & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
%  kin8nm   & $  () $   & $  () $  & $  ()$  & $  ()$  & $  ()$    \\ \hline
% \end{tabular}
% \end{center}


\clearpage
\subsection{Full Fusion Experiment Results} \label{app:all_fusion_results}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{arXiv/figs/full_calibration_table_fusion.pdf}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali.pdf}
    \caption{\textbf{Fusion Average Calibration-Sharpness Table.} The table shows mean average calibration (measured by ECE) and sharpness in parentheses, along with $\pm 1$ standard error. 
    The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined. 
    All values have been multiplied by 100 for readability.
    \textit{Cali} tends to achieve the best average calibration,
    while \textit{SQR} achieves the sharpest predictions (same table as Figure~\ref{fig:fusion_table_figure} (Top), repeated here for completeness)
    }
    \label{fig:fusion_ece_sharp_table_full}
    % \vspace{-4mm}
\end{figure*}


\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/fusion_cal_sharp_all_8.pdf}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali.pdf}
    \caption{\textbf{Fusion Average Calibration-Sharpness Plot.} Visualization of average calibration-sharpness from fusion experiments from Section~\ref{sec:uci_fusion}}.
    \label{fig:full_fusion_cal_sharp}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/fusion_group_cali_all_8.pdf}
    \caption{\textbf{Fusion Adversarial Group Calibration}  Full fusion results of Figure~\ref{fig:fusion_table_figure} (Bottom).
    \textit{Cali} and \textit{Interval} tend to achieve the best
    calibration for any group of any size in the test set.}
    \label{fig:full_fusion_gc}
    % \vspace{-4mm}
\end{figure*}


\begin{figure*}[h!]
\begin{center} \label{table:full_fusion_check}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 & \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}               & \textbf{\textit{Cali}}                      \\\hline
aminor     & $ \mathbf{0.087 \pm 0.000 } $   & $ 0.182 \pm 0.000 $  & $ 0.097 \pm 0.002 $  & $ 0.092 \pm 0.002 $ \\ \hline
dssdenest  & $ \mathbf{0.179 \pm 0.003 } $   & $ 0.273 \pm 0.003 $  & $ 0.180 \pm 0.001 $  & $ 0.184 \pm 0.002 $ \\ \hline
betan      & $ \mathbf{0.146 \pm 0.001 } $   & $ 0.253 \pm 0.005 $  & $ 0.153 \pm 0.002 $  & $ 0.150 \pm 0.001 $ \\ \hline
li         & $ \mathbf{0.097 \pm 0.001 } $   & $ 0.166 \pm 0.003 $  & $ 0.102 \pm 0.001 $  & $ 0.104 \pm 0.001 $ \\ \hline
volume     & $ \mathbf{0.051 \pm 0.001 } $   & $ 0.107 \pm 0.007 $  & $ 0.053 \pm 0.001 $  & $ 0.052 \pm 0.001 $ \\ \hline
ip         & $ \mathbf{0.068 \pm 0.000 } $   & $ 0.199 \pm 0.011 $  & $ 0.077 \pm 0.002 $  & $ 0.076 \pm 0.001 $ \\ \hline
kappa      & $ \mathbf{0.072 \pm 0.001 } $   & $ 0.150 \pm 0.004 $  & $ 0.079 \pm 0.002 $  & $ 0.078 \pm 0.001 $ \\ \hline
R0         & $ \mathbf{0.120 \pm 0.001 } $   & $ 0.208 \pm 0.002 $  & $ 0.126 \pm 0.002 $  & $ 0.130 \pm 0.005 $ \\ \hline
tribot     & $ \mathbf{0.084 \pm 0.001 } $   & $ 0.184 \pm 0.020 $  & $ 0.092 \pm 0.001 $  & $ 0.096 \pm 0.005 $ \\ \hline
tritop     & $ \mathbf{0.102 \pm 0.001 } $   & $ 0.200 \pm 0.018 $  & $ 0.107 \pm 0.004 $  & $ 0.107 \pm 0.002 $ \\ \hline
\end{tabular}
\caption{\textbf{Fusion Check Score} Check score results from fusion experiments in Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{SQR} achieves the best check score.}
\end{center}
\end{figure*}


\begin{figure*}[h!]
\begin{center} \label{table:fusion_int}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
& \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}               & \textbf{\textit{Cali}}                      \\\hline
aminor     & $ 1.181 \pm 0.007 $   & $ 3.225 \pm 0.000 $  & $ \mathbf{1.090 \pm 0.017 }$  & $ 1.207 \pm 0.035$ \\ \hline
dssdenest  & $ 2.387 \pm 0.060 $   & $ 4.352 \pm 0.109 $  & $ \mathbf{1.995 \pm 0.011 }$  & $ 2.369 \pm 0.054$ \\ \hline
betan      & $ 1.970 \pm 0.013 $   & $ 4.301 \pm 0.124 $  & $ \mathbf{1.725 \pm 0.021 }$  & $ 2.002 \pm 0.046$ \\ \hline
li         & $ 1.354 \pm 0.018 $   & $ 2.923 \pm 0.088 $  & $ \mathbf{1.146 \pm 0.010 }$  & $ 1.410 \pm 0.015$ \\ \hline
volume     & $ 0.711 \pm 0.023 $   & $ 2.036 \pm 0.154 $  & $ \mathbf{0.602 \pm 0.012 }$  & $ 0.697 \pm 0.026$ \\ \hline
ip         & $ 0.906 \pm 0.005 $   & $ 3.203 \pm 0.295 $  & $ \mathbf{0.845 \pm 0.017 }$  & $ 0.978 \pm 0.026$ \\ \hline
kappa      & $ 1.010 \pm 0.010 $   & $ 2.639 \pm 0.101 $  & $ \mathbf{0.891 \pm 0.015 }$  & $ 1.066 \pm 0.020$ \\ \hline
R0         & $ 1.599 \pm 0.011 $   & $ 3.310 \pm 0.064 $  & $ \mathbf{1.414 \pm 0.012 }$  & $ 1.709 \pm 0.057$ \\ \hline
tribot     & $ 1.211 \pm 0.009 $   & $ 3.185 \pm 0.242 $  & $ \mathbf{1.074 \pm 0.012 }$  & $ 1.421 \pm 0.115$ \\ \hline
tritop     & $ 1.481 \pm 0.022 $   & $ 3.564 \pm 0.351 $  & $ \mathbf{1.232 \pm 0.034 }$  & $ 1.444 \pm 0.031$ \\ \hline
\end{tabular}
\caption{\textbf{Fusion Interval Score} 
    Interval score results from fusion experiments in  Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{Interval} achieves the best interval score.}
\end{center}
\end{figure*}

\begin{figure*}[h!]
\begin{center} \label{table:fusion_int_cali}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
& \textit{SQR}                 & \textit{mPAIC}            & \textbf{\textit{Interval}}               & \textbf{\textit{Cali}}                      \\\hline
aminor     & $ 0.081 \pm 0.006 $   & $ 0.268 \pm 0.000 $  & $\mathbf{ 0.055 \pm 0.007 } $ & $ 0.058 \pm 0.004 $ \\ \hline
dssdenest  & $ 0.072 \pm 0.003 $   & $ 0.162 \pm 0.003 $  & $\mathbf{ 0.054 \pm 0.006 } $ & $ 0.071 \pm 0.008 $ \\ \hline
betan      & $\mathbf{0.051 \pm 0.001 }$   & $ 0.160 \pm 0.012  $  & $ 0.087 \pm 0.009 $  & $ 0.056 \pm 0.007 $ \\ \hline
li         & $ 0.071 \pm 0.011 $   & $ 0.214 \pm 0.017 $  & $ 0.069 \pm 0.013 $  & $\mathbf{ 0.043 \pm 0.003 } $\\ \hline
volume     & $ 0.073 \pm 0.007 $   & $ 0.315 \pm 0.022 $  & $ 0.063 \pm 0.007 $  & $\mathbf{ 0.056 \pm 0.002 } $\\ \hline
ip         & $ 0.051 \pm 0.003 $   & $ 0.227 \pm 0.020 $  & $ 0.077 \pm 0.015 $  & $\mathbf{ 0.036 \pm 0.003 } $\\ \hline
kappa      & $ 0.069 \pm 0.008 $   & $ 0.254 \pm 0.014 $  & $ 0.078 \pm 0.011 $  & $\mathbf{ 0.053 \pm 0.004 } $\\ \hline
R0         & $ 0.068 \pm 0.007 $   & $ 0.168 \pm 0.009 $  & $\mathbf{ 0.058 \pm 0.007 } $ & $ 0.066 \pm 0.004 $ \\ \hline
tribot     & $ 0.087 \pm 0.006 $   & $ 0.227 \pm 0.016 $  & $\mathbf{ 0.074 \pm 0.008 } $ & $ 0.080 \pm 0.007 $ \\ \hline
tritop     & $ 0.077 \pm 0.006 $   & $ 0.231 \pm 0.017 $  & $ 0.058 \pm 0.015 $  & $ \mathbf{0.037 \pm 0.004 }$ \\ \hline
\end{tabular}
\caption{\textbf{Fusion Centered Interval Calibration}
     Full centered interval calibration results from fusion experiments in Section~\ref{sec:uci_fusion}.
    Mean score across 5 trials is given, along with $\pm 1$ standard error. 
    The best mean has been bolded.
    \textit{Cali} and \textit{Interval} achieves the best centered
    interval calibration in 9 out of 10 datasets.}
\end{center}
\end{figure*}


==> NeurIPS2021/app_maqr.tex <==
\section{Model Agnostic Quantile Regression} \label{app:maqr}
\subsection{General Algorithm for Model Agnostic Quantile Regression} 
As stated in Section~\ref{sec:maqr}, Algorithm~\ref{alg:maqr_main} is one implementation of a general 
model-agnostic quantile regression procedure, in which we take direct estimates of the target density
and regress onto these estimates. 
This general framework is state in Algorithm~\ref{alg:general_mauq}

\begin{algorithm}[h ]
  \caption{General Algorithm for Model Agnostic Quantile Regression} 
\begin{algorithmic}[1]\label{alg:general_mauq}
%   \STATE {\bfseries Input:} capital $T$, initial capital $t_{init}$, mean functions $\mu^{(x)}$, kernel functions $\sigma^{(x)}$.
    \STATE {\bfseries Input:} Train data $\{x_i, y_i\}_{i=1}^{N}$
    % an untrained regression model $\hat{g}$ of designated model type,
    % optionally
    % \STATE If $f$ is not given, fit a regression model $f(x)$ with $\{x_i, y_i\}_{i=1}^{N}$\ 
    % \STATE Calculate the residuals $\epsilon_i = y_i - f(x_i)$, \hspace{2mm}$i=1,\ldots,N$
    % \STATE Calculate the residuals $\epsilon_i = y_i - \hat{f}(x_i)$, \hspace{2mm}$i\in[N]$
    \STATE Initialize $D \leftarrow \varnothing$
    \FOR{$i=1$ {\bfseries to} $N$}
    \STATE Select a set of quantile levels $\{p_k\}_{k=1}^{m}$, \hspace{1mm}$p_k \in [0,1]$
    \STATE $\hat{q}_{i, p_k} \leftarrow$ KDE estimate of $\Q(x_i, p_k)$, $k=1,\ldots,m$
    % \STATE $E_{i,d} \leftarrow \{\eps_j: \textrm{dist}(x_i, x_j) \leq d, 1 \leq j \leq N \}$
    % Find $\{(x_j, \epsilon_j) : \textrm{dist}(x_i, x_j) \leq d, 1 \leq j \leq N \}$, 
    % Determine which $x_j \in \{x_k\}_{k=1}^{N}$ are "close to" {\unsure (muy malo)} $x_i$ and create the set of nearby points $\{x_j, \epsilon_j\}$ 
    % \STATE Construct an empirical CDF with $E_{i,d}$ to produce $\hF_{\by|x_i}: e \mapsto p\in[0,1]$
    % $\{e_j\}$
    % \STATE Find the inverse values of $\hat{G}$ of $\{p_k\}_{k=1}^{m}$, denote this set $\{\epsilon_k\}_{k=1}^{m}$
    % using $\hat{G}_i^{-1}: p\in[0,1] \rightarrow \epsilon$
    \STATE $D \leftarrow D \cup \{x_i, p_k, \hat{q}_{i, p_k}\}_{k=1}^{m}$
    \ENDFOR 
    % \STATE Fit a regression model $\hat{g}$ with $D$: tuple $(x, p)$ as input and $\epsilon$ as target
    % \STATE Use $D$ to fit a regression model $g_p: x \mapsto \eps$, for $p \in \{p_k\}_{k=1}^{m}$
    \STATE Use $D$ to fit a regression model $\hQ$ \\
    \hspace{10pt} $\hQ: (x_i, p_k) \mapsto \hat{q}_{i, p_k}$, \hspace{2mm}$k=1,\ldots,m$ 
    % : tuple $(x, p)$ as input and $\epsilon$ as target
%   \STATE Draw $\widetilde{f}(x, \cdot) \sim GP(\mu^{(x)}, \sigma^{(x)}) | D_{t - 1}$ for all $x \in \X$.
%   \STATE {\bfseries Output:} $f + g_p$, for $p \in \{p_k\}_{k=1}^{m}$
  \STATE {\bfseries Output:} $\hat{g}$, \hspace{2mm}$k=1,\ldots,m$
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:maqr_main} implements the KDE step of Algorithm~\ref{alg:general_mauq} (Line 5 of Algorithm~\ref{alg:general_mauq})
by using a uniform kernel over $\cx$ (Line 2 of Algorithm~\ref{alg:CondQuantEst}) and $\cy$ (Lines 3,5,6 of Algorithm~\ref{alg:CondQuantEst}).
% In this case, the quantile estimates $\{p_k, \hat{q}_{i, p_k}\}$ is exactly the estimator $\{m_n(\hat{q}_{i, p_k}|x_i), \hat{q}_{i, p_k}\}$
% from \cite{stute1986almost}, and under mild assumptions on the bandwidth of the kernel over $\cx$, by Theorem 1 of \cite{stute1986almost}, 
% the quantile dataset $D$ in line 9 of Algorithm~\ref{alg:maqr} is consistent for almost all $x \in \cx$, 
% i.e. for almost all $x \in \cx$, the conditional quantile estimates approach the true conditional quantiles almost surely 
% as the number of datapoints $N \rightarrow \infty$.
% We refer the reader to \cite{stute1986almost} for details on the proof. 
% What this signifies is that in the limit of datapoints, 
% the regression targets for the quantile model will be the true conditional quantiles, and hence, the labels we attribute to each quantile and quantile level are in fact the true underlying values.

It should also be noted that many other conditional KDE methods can be used to construct the dataset $D$.
We refer the reader to \citet{holmes2012fast, hyndman1996estimating} for a more thorough treatment of methods in conditional KDE.

Lastly, this algorithm is model agnostic because \textit{any} regression model
can be used for $\hat{g}$ in Algorithm~\ref{alg:general_mauq}, and for $\hat{f}$ and $\hat{g}$ in Algorithm~\ref{alg:maqr_main}.
In our specific implementation of Algorithm~\ref{alg:maqr_main}, we used a neural network 
for $\hat{g}$ to fit the quantile dataset $D$, but we can also use other models, 
such as a random forest or gradient-boosted trees. 
In particular, we have replaced $\hat{g}$ in Algorithm~\ref{alg:maqr_main} with
a gradient-boosted tree model and observed very similar UQ performance on the UCI datasets
as reported in Section~\ref{sec:uci_fusion} (we omit numerical values because they are very similar 
and otherwise uninformative).


\subsection{Algorithm Complexity} \label{app:alg_complexity_analysis}
% Algorithm~\ref{alg:maqr_main} has two stages, depending on whether the mean function 
% $\hat{f}$ is provided or not. 
% In the case this function is not provided, 
% the first stage constitutes learning this function with a standard regression algorithm
% (usually a regression model with MSE loss). 
% We do not analyze this step.

Lines 2 and 3 of Algorithm~\ref{alg:CondQuantEst} requires calculating the distance between $x_k$ and all other $x_i, 1\leq i \leq N$, 
and ordering these distances to construct the empirical CDF. 
Let the distance calculation between a pair of points take constant $C$ time. 
Ordering the distance requires sorting the $N$ distances. 
Hence, Lines 5 and 6 takes $\mathcal{O}(N\log N)$ time.

If $K$ points are in the set $E_{k,d_{N}}$, 
Lines 5, 6, 7 of Algorithm~\ref{alg:CondQuantEst} are done for each of the $K$ points.
% the CDF construction in Line 6 also requires an ordering on these $K$ points, 
% which is $\mathcal{O}(K\log K)$. 
We consider the worst case when each set $E_{k,d_{N}}$ contains all $N$ points, 
which costs $\mathcal{O}(N)$.

The above two procedures are done for all $N$ points (Line 4 of Algorithm~\ref{alg:maqr_main}), 
therefore the for loop from Lines 4 to 7 in Algorithm~\ref{alg:maqr_main} requires $\mathcal{O}(N^2 \log N)$ time. 
This loop takes into account creating the dataset $D$ for the quantile model. 
The rest of the algorithm constitutes fitting a regression model with this dataset $D$, which we do not analyze here.

We now discuss the space complexity. 
In Lines 5, 6, 7 of Algorithm~\ref{alg:CondQuantEst}, we only draw the quantiles at which a discontinuous step occurs in the constructed empirical CDF. 
For example, if we constructed an empirical CDF with three equally weighted points, we will only draw the quantiles $[1/3, 2/3, 1]$.
Following this procedure, in the worst case, for each of the $N$ points, we will construct a CDF with all $N$ points, and hence draw $N$ quantiles to append to the quantile model dataset $D$. 
If we consider the space complexity of the mean function and the quantile model to be constant, 
the algorithm requires $O(N^2)$ space in total. 



% \subsubsection{One Version of the Algorithm}

% \begin{algorithm}[h!]
%   \caption{Model Agnostic Quantile Regression} 
% \begin{algorithmic}[1]\label{alg:mauq}
% %   \STATE {\bfseries Input:} capital $T$, initial capital $t_{init}$, mean functions $\mu^{(x)}$, kernel functions $\sigma^{(x)}$.
%     \STATE {\bfseries Input:} Train data $\{x_i, y_i\}_{i=1}^{N}$,
%     % an untrained regression model $\hat{g}$ of designated model type,
%     % optionally
%     trained regression model $\hat{f}(x)$
%     % \STATE If $f$ is not given, fit a regression model $f(x)$ with $\{x_i, y_i\}_{i=1}^{N}$\ 
%     % \STATE Calculate the residuals $\epsilon_i = y_i - f(x_i)$, \hspace{2mm}$i=1,\ldots,N$
%     \STATE Calculate the residuals $\epsilon_i = y_i - \hat{f}(x_i)$, \hspace{2mm}$i\in[N]$
%     \STATE Initialize $D \leftarrow \varnothing$
%     \FOR{$i=1$ {\bfseries to} $N$}
%     \STATE $E_{i,d} \leftarrow \{\eps_j: \textrm{dist}(x_i, x_j) \leq d, 1 \leq j \leq N \}$
%     % Find $\{(x_j, \epsilon_j) : \textrm{dist}(x_i, x_j) \leq d, 1 \leq j \leq N \}$, 
%     % Determine which $x_j \in \{x_k\}_{k=1}^{N}$ are "close to" {\unsure (muy malo)} $x_i$ and create the set of nearby points $\{x_j, \epsilon_j\}$ 
%     \STATE Construct an empirical CDF with $E_{i,d}$ to produce $\hF_{\by|x_i}: e \mapsto p\in[0,1]$
%     % $\{e_j\}$
%     \STATE Select a set of quantile levels $\{p_k\}_{k=1}^{m}$, \hspace{1mm}$p_k \in [0,1]$
%     \STATE $\hat{q}_{i, p_k} \leftarrow \inf \{e: p_k \leq \hF_{\by|x_i}(e)\}$, \hspace{2mm}$k=1,\ldots,m$
%     % \STATE Find the inverse values of $\hat{G}$ of $\{p_k\}_{k=1}^{m}$, denote this set $\{\epsilon_k\}_{k=1}^{m}$
%     % using $\hat{G}_i^{-1}: p\in[0,1] \rightarrow \epsilon$
%     \STATE $D \leftarrow D \cup \{x_i, p_k, \hat{q}_{i, p_k}\}_{k=1}^{m}$
%     \ENDFOR 
%     % \STATE Fit a regression model $\hat{g}$ with $D$: tuple $(x, p)$ as input and $\epsilon$ as target
%     % \STATE Use $D$ to fit a regression model $g_p: x \mapsto \eps$, for $p \in \{p_k\}_{k=1}^{m}$
%     \STATE Use $D$ to fit a regression model $\hat{g}$ \\
%     \hspace{10pt} $\hat{g}: (x_i, p_k) \mapsto \hat{q}_{i, p_k}$, \hspace{2mm}$k=1,\ldots,m$ 
%     % : tuple $(x, p)$ as input and $\epsilon$ as target
% %   \STATE Draw $\widetilde{f}(x, \cdot) \sim GP(\mu^{(x)}, \sigma^{(x)}) | D_{t - 1}$ for all $x \in \X$.
% %   \STATE {\bfseries Output:} $f + g_p$, for $p \in \{p_k\}_{k=1}^{m}$
%   \STATE {\bfseries Output:} $\hat{f} + \hat{g}$, \hspace{2mm}$k=1,\ldots,m$
% \end{algorithmic}
% \end{algorithm}




==> NeurIPS2021/app_theory.tex <==
\section{Theoretical Results}
\subsection{Proof of Proposition 1} \label{app:prop_1}


{\bf Proposition 1}. \label{prop:pinball}
{\it Consider a finite dataset $D$, the pinball loss $\rho_\tau$ (Eq.~\ref{eq:pinball_loss}) and a quantile model
$f: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$ that is average calibrated on $D$, i.e. $\text{ECE}(D, f) = 0$.
Then there always exists another quantile model $g: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$, such that, for any quantile level $\tau \in (0, 1)$, 
$g$ has lower pinball loss than $f$ on $D$, i.e. 
$\sum_{i=1}^{N}\rho_\tau(y_i, g_\tau(x_i)) < \sum_{i=1}^{N}\rho_\tau(y_i, f_\tau(x_i))$,
but worse average calibration than $f$, i.e. $\text{ECE}(D, g) > \text{ECE}(D, f)$.} 

\textbf{Proof:}
% Denote $\pobs(D, \tau)$ as the average observed probability of $f$ for the quantile level $\tau$.

%%% BEGIN: original
% Since $f$ is average calibrated on $D$,  
% for any given quantile level $\tau \in (0, 1)$, $\pobs(D, \tau) = \tau$,
%%% END: original 
Denote $\{p_j\}_{j=1}^{m}$ 
as the set of quantiles used to compute $ECE(D,f)$.
Since $f$ is average calibrated on $D$,
for any $\tau \in \{p_j\}_{j=1}^{m}$, $\pobs(D, \tau)$ of $f$ is equal to $\tau$, i.e.
% $\pobs(D, \tau)$ of $f = \tau$, 
\begin{itemize}
    \item $|\{(x_i, y_i) \mid y_i \leq f_{\tau}(x_i)\}| = \tau*N$, 
    \item $|\{(x_i, y_i) \mid y_i > f_{\tau}(x_i)\}| = (1-\tau)*N$.
\end{itemize}

Denote $\{(x_i, y_i) \mid y_i \leq f_{\tau}(x_i)\}$ as $S^{\text{under}}_{f}$
and $\{(x_i, y_i) \mid y_i > f_{\tau}(x_i)\}$ as $S^{\text{over}}_{f}$.

Let $\rho_\tau(D, f_{\tau})$ be the pinball loss of $f_\tau$ on $D$, i.e. $\rho_{\tau}(D, f_{\tau}) = \sum_{i=1}^N \rho_\tau(y_i, f_\tau(x_i))$.

Then, 
% The pinball loss of $f_{\tau}$ on $D$ is equal to:
\begin{align*}
\begin{aligned}
\rho_\tau(D, f_{\tau})
= \sum_{i=1}^{N}\rho_\tau(y_i, f_\tau(x_i))
&= \sum_{(x_i,y_i) \in S^{\text{under}}_{f}} (f_\tau(x_i) - y_i)(1-\tau) \\
&+ \sum_{(x_i,y_i) \in S^{\text{over}}_{f}} (f_\tau(x_i) - y_i)(-\tau).
\end{aligned}
\end{align*}

We can construct another quantile model $g$, 
s.t. its prediction for $\tau$, $g_\tau$, is as follows:
% For this $\tau$, we can construct a new prediction $g_{\tau}$, as follows: 
% take any point $(x_k, y_k) \in S_{\text{under}}$
% and set $g_\tau(x_k)$ 
% $= y_k - \frac{1-\tau}{2\tau}(f_{\tau}(x_k) - y_k)$. 
% For all other points, $(x_i, y_i)_{i\neq k}\in D$, set $g_{\tau}(x_i) = f_{\tau}(x_i)$.
take any point $(x_k, y_k) \in S^{\text{over}}_{f}$
and set $g_\tau(x_k)$ 
$= y_k - \frac{\tau}{2(1-\tau)}(f_{\tau}(x_k) - y_k)$. 
For all other points, $(x_i, y_i)_{i\neq k}\in D$, set $g_{\tau}(x_i) = f_{\tau}(x_i)$.

% $=\frac{1}{2\tau}[(1+\tau)y_k - (1-\tau)f_{\tau}(x_k)]$.


Since $y_k - g_{\tau}(x_k) = \frac{\tau}{2(1-\tau)}(f_{\tau}(x_k) - y_k) < 0$,
we have that $y_k < g_{\tau}(x_k)$.

Therefore, 
$|\{(x_i, y_i) \mid y_i \leq g_{\tau}(x_i)\}| = (\tau*N) + 1$ and 
$|\{(x_i, y_i) \mid y_i > g_{\tau}(x_i)\}| = ((1-\tau)*N) - 1$.

Therefore, $|\pobs(D, \tau)$ of $g$ $-$ $\tau |$ $>$ $|\pobs(D, \tau)$ of $f$ $-$ $\tau |$, which implies that according to $\{p_j\}_{j=1}^{m}$, 
$ECE(D, g) > ECE(D, f)$.

We further consider the pinball loss of $g_{\tau}$ on $D$, $\rho_\tau(D, g_\tau)$.

$\rho_\tau(D, g_\tau) = \sum_{i=1}^{N}\rho_\tau(y_i, g_\tau(x_i)) =  \rho_\tau(y_k, g_\tau(x_k)) + \sum_{i\in[N], i\neq k}\rho_\tau(y_i, f_\tau(x_i))$.

Note that the term, $\rho_\tau(y_k, g_\tau(x_k))$ satisfies:
% \begin{align*}
%     \rho_\tau(y_k, g_\tau(x_k)) 
%     &= (g_\tau(x_k) - y_k)(-\tau) \\
%     &= (y_k - g_\tau(x_k))(\tau) \\
%     &= \frac{1-\tau}{2\tau}(f_{\tau}(x_k) - y_k) (\tau) \\
%     &= \frac{1}{2}(f_{\tau}(x_k) - y_k)(1-\tau) \\
%     &< (f_{\tau}(x_k) - y_k)(1-\tau) \\
%     &= \rho_\tau(y_k, f_\tau(x_k))   
% \end{align*}
\begin{align*}
    \rho_\tau(y_k, g_\tau(x_k)) 
    &= (g_\tau(x_k) - y_k)(1-\tau) \\
    &= \frac{\tau}{2(1-\tau)}(y_k - f_{\tau}(x_k)) (1-\tau) \\
    &= \frac{\tau}{2}(y_k - f_{\tau}(x_k)) \\
    &< \tau(y_k - f_{\tau}(x_k)) \\
    &= (-\tau)(f_{\tau}(x_k) - y_k) \\
    &= \rho_\tau(y_k, f_\tau(x_k))   
\end{align*}

Therefore, $\rho_\tau(D, g_\tau) < \rho_\tau(D, f_\tau)$,
i.e. the pinball loss of $g_{\tau}$ on $D$ is less than the pinball loss of $f_{\tau}$ on $D$.

Note that for any $\tau \not\in \{p_j\}_{j=1}^{m}$, 
we can follow the same steps to construct $g_\tau$ 
s.t. $|\pobs(D, \tau)$ of $g$ $-$ $\tau |$ $>$ $|\pobs(D, \tau)$ of $f$ $-$ $\tau |$, i.e. $g_\tau$ is more miscalibrated than $f_\tau$.
Therefore, for any quantile level $\tau \in (0, 1)$, $\sum_{i=1}^{N}\rho_\tau(y_i, g_\tau(x_i)) < \sum_{i=1}^{N}\rho_\tau(y_i, f_\tau(x_i))$, but
$\text{ECE}(D, g) > \text{ECE}(D, f)$. 

\hfill $\qedsymbol$

\subsection{Proof of Proposition 2} \label{app:prop_2}

{\bf Proposition 2}. \label{prop:cal_obj}
{\it For any quantile level $p \in (0, 1)$, 
the true quantile function $\mathbb{Q}_p$ minimizes the calibration objective, 
$\mathcal{C}(\hat{\mathbb{Q}}_p, p)$.
Further, on a finite dataset $D$, the empirical calibration objective, $\mathcal{C}(D, \hat{\mathbb{Q}}_p, p)$,
is minimized by an average calibrated solution on $D$, i.e. when $\pobs(D, p) = p$.}

\textbf{Proof:}\\
Recall the calibration objective for a quantile level $p\in(0,1)$,
\begin{align*}
    \mathcal{C}(\hQ_p, p) 
    &= \mathbb{I}\{\hat{p}_p < p\} * \E[Y-\hQ_p | Y > \hQ_p] * P(Y > \hQ_p) \\ 
    & \hspace{5pt} + \mathbb{I}\{\hat{p}_p > p\} * \E[\hQ_p - Y | \hQ_p > Y] * P(\hQ_p > Y), 
    \text{where} \hspace{5pt} \hp_p = P(Y \leq \hQ_p). \nonumber
\end{align*}

For the true quantile function $\Q_p$, $P(Y\leq \Q_p) = p$, thus achieves the minimum value of $0$ for $\mathcal{C}(\hQ_p, p)$, as
the two non-negative terms of $\mathcal{C}(\hQ_p, p) $ are $0$.


Further, recall the empirical calibration objective,
\begin{align*}
    \begin{split}
        \mathcal{C}(D, \hQ, p) 
        & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        % &\mathcal{C}(D, \hQ, p) = \\
        % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
    \end{split}
\end{align*}

An average calibrated solution on the dataset $D$ satisfies $\hp^{\text{obs}}_{avg} = p$, thus achieves the minimum value of $0$ for $\mathcal{C}(D, \hQ, p)$, as
the two non-negative terms of $\mathcal{C}(D, \hQ, p) $ are $0$. 

\hfill $\qedsymbol$

\subsection{Derivation of Gradients of Calibration Objective} \label{app:note_3}
Denote the CDF and PDF of the random variable $Y$ as $\mathbb{F}_{Y}$ and
$f_{Y}$.
\begin{itemize}
    \item When $\hp_p = P(Y \leq \hQ_p) < p$:\\
    \begin{align*}
        \mathcal{C}(\hQ_p, p) 
        &= \E[Y-\hQ_p | Y > \hQ_p] * P(Y > \hQ_p)\\
        &= \left(\E[Y | Y > \hQ_p]-\hQ_p\right) * P(Y > \hQ_p)\\
        &= \left(\frac{\int_{\hQ_p}^{\infty} y f_Y(y) dy}{P(Y > \hQ_p)} -\hQ_p\right) * P(Y > \hQ_p)\\
        &= \left(\int_{\hQ_p}^{\infty} y f_Y(y) dy \right)
        - \left(\hQ_p * P(Y > \hQ_p)\right) \\
        &= \left(\int_{\hQ_p}^{\infty} y f_Y(y) dy \right)
        - \left(\hQ_p * (1 - F_Y(\hQ_p))\right) \\
    \end{align*}
    
    Note that,
    \begin{align*}
        \frac{\partial \left(\int_{\hQ_p}^{\infty} y f_Y(y) dy \right)}{\partial \hQ_p} 
        &= -\hQ_p * f_Y(\hQ_p) \\ 
        \frac{\partial  \left(\hQ_p * (1 - F_Y(\hQ_p)\right) }{\partial \hQ_p}
        &= (1 - F_Y(\hQ_p) + \hQ_P * (-f_y(\hQ_p))
    \end{align*}
    
    Therefore,
    \begin{align*}
        \frac{\partial \mathcal{C}(\hQ_p, p)}{\partial \hQ_p} 
        &= \frac{\partial \left(\int_{\hQ_p}^{\infty} y f_Y(y) dy \right)}{\partial \hQ_p} - \frac{\partial  \left(\hQ_p * (1 - F_Y(\hQ_p)\right) }{\partial \hQ_p} \\ 
        &= -\hQ_p * f_Y(\hQ_p) - (1 - F_Y(\hQ_p) + \hQ_P * f_y(\hQ_p) \\ 
        &= - (1 - F_Y(\hQ_p)\\
        &= -P(Y>\hQ_p)
    \end{align*}
    
    
    \item When $\hp_p = P(Y \leq \hQ_p) > p$:\\
    \begin{align*}
        \mathcal{C}(\hQ_p, p) 
        &= \E[\hQ_p - Y | \hQ_p > Y] * P(\hQ_p > Y)\\
        &= \left(\hQ_p - \E[Y | \hQ_p > Y]\right) * P(\hQ_p > Y)\\
        &= \left(\hQ_p - \frac{\int^{\hQ_p}_{-\infty} y f_Y(y) dy}{P( \hQ_p > Y)}\right) * P(\hQ_p > Y)\\
        &= \left(\hQ_p *P(\hQ_p > Y)\right)  - \left(\int^{\hQ_p}_{-\infty} y f_Y(y) dy \right)\\
        &= \left(\hQ_p * F_Y(\hQ_p)\right) - \left(\int^{\hQ_p}_{-\infty} y f_Y(y) dy \right)\\
    \end{align*}
    Note that,
    \begin{align*}
        \frac{\partial \left(\hQ_p * F_Y(\hQ_p)\right)}{\partial \hQ_p}
        &= F_Y(\hQ_p) + \hQ_P * f_Y(\hQ_p)\\
        \frac{\partial \left(\int^{\hQ_p}_{-\infty} y f_Y(y) dy \right)}{\partial \hQ_p} 
        &= \hQ_p * f_Y(\hQ_p)
    \end{align*}
    
    Therefore,
    \begin{align*}
        \frac{\partial \mathcal{C}(\hQ_p, p)}{\partial \hQ_p} 
        &= \frac{\partial  \left(\hQ_p * F_Y(\hQ_p\right) }{\partial \hQ_p} - 
        \frac{\partial \left(\int^{\hQ_p}_{-\infty} y f_Y(y) dy \right)}{\partial \hQ_p}\\ 
        &= F_Y(\hQ_p) + \hQ_P * f_Y(\hQ_p) - \hQ_p * f_Y(\hQ_p)\\
        &= F_Y(\hQ_p)\\
        &= P(Y<\hQ_p).
    \end{align*}
\end{itemize}
\hfill $\square$


\subsection{Optimum of Interval Score} \label{app:int_score}
Following notation from Section~\ref{sec:int}, we denote $\hat{l} = \hQ(x, \frac{\alpha}{2})$ and $\hat{u} = \hQ(x, 1-\frac{\alpha}{2})$, 
and we omit conditioning on $x$ for clarity.

Assume $\hat{l} \leq \hat{u}$. Then,
\begin{align*}
    &\mathbb{E}\left[ S_{\alpha}(\hat{l}, \hat{u}; y) \right]\\
    &= \int_{-\infty}^{\hat{l}} S_{\alpha}(\hat{l}, \hat{u}; y) d\F(y) 
    + \int_{\hat{l}}^{\hat{u}} S_{\alpha}(\hat{l}, \hat{u}; y) d\F(y) 
    + \int_{\hat{u}}^{\infty} S_{\alpha}(\hat{l}, \hat{u}; y) d\F(y)\\
    &= (\hat{u} - \hat{l})
    + \frac{2}{\alpha} \int_{-\infty}^{\hat{l}} (\hat{l} - y) d\F(y) 
    + \frac{2}{\alpha} \int_{\hat{u}}^{\infty} (y - \hat{u})  d\F(y)\\
    &\frac{\partial \mathbb{E}\left[ S_{\alpha}(\hat{l}, \hat{u}; y) \right]}{\partial \hat{l}} 
    = -1 + \frac{2}{\alpha}\int_{-\infty}^{\hat{l}} d\F(y) = -1 + \frac{2}{\alpha} \F(\hat{l})\\
    &\frac{\partial \mathbb{E}\left[ S_{\alpha}(\hat{l}, \hat{u}; y) \right]}{\partial \hat{u}} 
    = 1 - \frac{2}{\alpha}\int_{\hat{u}}^{\infty} d\F(y) = 1 - \frac{2}{\alpha}(1- \F(\hat{u})).
\end{align*}
Setting $\frac{\partial \mathbb{E}\left[ S_{\alpha}(\hat{l}, \hat{u}; y) \right]}{\partial \hat{l}}$ and $\frac{\partial \mathbb{E}\left[ S_{\alpha}(\hat{l}, \hat{u}; y) \right]}{\partial \hat{u}}$ to zero reveals the interval loss minima at the respective true quantiles,
\begin{align*}
    \F(\hat{l}) &= \frac{\alpha}{2} \text{  and  } \F(\hat{u}) = 1 - \frac{\alpha}{2}\\
    \text{i.e.  } \hat{l} &= \Q(\cdot, \frac{\alpha}{2}) \text{  and  } \hat{u} = \Q(\cdot, 1 - \frac{\alpha}{2})
\end{align*}
% $\F(\hat{l}) = \frac{\alpha}{2}$, $\F(\hat{u}) = 1 - \frac{\alpha}{2}$, i.e. $\hat{l} = \Q(\cdot, \frac{\alpha}{2})$, $\hat{u} = \Q(\cdot, 1 - \frac{\alpha}{2})$. 
\hfill $\square$


==> NeurIPS2021/checklist.tex <==
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See summary of contributions in the introduction (Section~\ref{sec:introduction}).}
  \item Did you describe the limitations of your work?
    \answerYes{See first paragraph in Section~\ref{sec:cali}, see last paragraph in Section~\ref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss potential negative impacts of our work in the Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have made sure our work conforms to the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All Theorem and Proposition statements (Sections~\ref{sec:metrics}, ~\ref{sec:maqr}, ~\ref{sec:cali}) state the full set of assumptions.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Appendix has proofs for all theoretical statements.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code and its instructions are included in supplemental materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Full details of experimental setup are included in Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments have been repeated with 5 random seeds, and all error bars are reported in Section~\ref{sec:experiments} and the Appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We discuss experimental setup and compute resources in the Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the source of the nuclear fusion dataset in Section~\ref{sec:uci_fusion}, we cite code used in the Appendix.}
  \item Did you mention the license of the assets?
    \answerYes{We mention license of assets in the Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{No new assets are included in the supplemental materials or as a URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We mention data usage consent in the Appendix.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We discuss in the Appendix how the data contains no PII.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> NeurIPS2021/conclusion.tex <==
\vspace{-2mm}
\section{Discussion}
\label{sec:discussion}
\vspace{-3mm}
In this paper, we have proposed four methods to improve quantile estimates 
for calibrated uncertainty quantification in regression.
We assert that the pinball loss may not be an adequate objective
to optimize in order to achieve calibration,
and that our proposed methods provide better means of learning 
calibrated conditional quantiles.
We have also extended the scope of regression models on which quantile-based UQ 
can be applied by developing a model-agnostic method.
This can be of practical interest 
to users that have specific training infrastructure or preexisting regression procedures 
since these procedures can be leveraged to quantify uncertainty without additional overhead.
% for
% which they want to quantify uncertainty without additional overhead.

By providing an extensive evaluation with a suite of metrics,
we also aim to show
% the value of providing a holistic review and comparison
% of many existing metrics
that there is not one single metric that captures full information about 
the performance of a UQ procedure. Rather, a holistic review of multiple types of metrics
sheds light on different aspects of performance.
% This point motivated us to additionally develop and make publicly available \href{https://github.com/uncertainty-toolbox/uncertainty-toolbox}{Uncertainty Toolbox}, a Python library for evaluation, visualization and recalibration of predictive uncertainty, which includes the full suite of metrics discussed in this work.

In certain applications, users may also be concerned with modeling epistemic uncertainty.
This is somewhat orthogonal to the goals of this paper;  nevertheless, we provide a
discussion on how bootstrapped ensembles of our methods can incorporate epistemic
uncertainty in Appendix~\ref{app:epistemic}.
% There are a few future directions that we hope to pursue ... ???


% In this paper, we have advocated expressing distributional prediction with quantiles 
% and have proposed four methods to improve quantile estimates of predictive uncertainty.
% We have also emphasized the key goal that UQ in regression should strive for (i.e. individual calibration), 
% and have described the relevant metrics that can be used to give some perspective on how well this goal has been achieved,
% as well as the metrics' limitations. 
% This is further demonstrated in our experiments, where we have tried to give a holistic picture
% of UQ performance assessment, and it's shown that no single metric will give the 
% best summary, and rather considering the set of metrics together is beneficial.
% One may argue that a UQ method must also be able to incorporate epistemic uncertainty.
% While this would be an orthogonal direction from our stated goals and metrics 
% (i.e. for converging to the true underlying distribution),
% we provide a discussion of how we can choose to incorporate epistemic uncertainty into quantile models
% and produce combined uncertainty estimates in Appendix~\ref{app:epistemic}.



% One future direction is incorporating adversarial group calibration into a recalibration algorithm, 
% as recalibration methods only consider average calibration.
% Another direction is devising a better optimization method for average calibration.

% \ianx{\textbf{Ian Attempt:} In this paper we introduced four new methods for improving quantile estimates. We assert that pinball loss does not directly target key quantities practitioners are concerned with (e.g. calibration and sharpness), and that our proposed methods are more suited for these quantities. We hope that this disentangles quantile regression from pinball loss and makes practitioners and researchers more carefully consider whether pinball loss is appropriate for their application.}

% \ianx{\textbf{Ian Attempt Epistemic (but I kind of think could be good to be in section 3)} Often one is also concerned about epistemic uncertainty. This is somewhat orthogonal to the goals of this paper; nevertheless, we provide discussion on how bootstrapped ensembled versions of methods can incorporate epistemic uncertainty in Appendix(APPENDIX).}

==> NeurIPS2021/depr_experiments.tex <==
% \vspace{-1mm}
\section{Experiments}
\label{sec:experiments}
% \vspace{-1mm}
% \begin{figure*}[t]
% % \begin{table}[ht!]
% % \begin{adjustbox}{width=8.5cm, height=1.5cm}
% % \begin{adjustbox}{width=1.1\columnwidth,center}
% % \begin{center} \label{table:uci_check}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & SQR                 & IndvCal            & \textbf{Int}      & \textbf{Cali}     & \textbf{MAQR}        \\\hline
% concrete & $\textit{ 0.085 (0.006) }$   & $\textbf{\textit{ 0.085 (0.005) }}$  & $ 0.086 (0.004)$  & $ 0.118 (0.006)$  & $\textbf{ 0.059 (0.008)}$    \\ \hline
% power    & $\textbf{ 0.057 (0.001) }$   & $ 0.070 (0.001) $  & $ 0.062 (0.001)$  & $ 0.064 (0.001)$  & $\textbf{\textit{ 0.058 (0.001)}}$    \\ \hline
% wine     & $\textbf{\textit{ 0.205 (0.008) }}$   & $ 0.219 (0.004) $  & $ 0.214 (0.006)$  & $ 0.210 (0.008)$  & $\textbf{ 0.191 (0.003)}$    \\ \hline
% yacht    & $\textbf{\textit{ 0.012 (0.002) }}$   & $ 0.015 (0.002) $  & $ 0.018 (0.003)$  & $ 0.019 (0.004)$  & $\textbf{ 0.007 (0.001)}$    \\ \hline
% naval    & $ 0.070 (0.001) $   & $\textbf{\textit{ 0.276 (0.004) }}$  & $ 0.066 (0.013)$  & $ 0.159 (0.029)$  & $\textbf{ 0.004 (0.000)}$    \\ \hline
% energy   & $\textbf{\textit{ 0.014 (0.000) }}$   & $ 0.015 (0.001) $  & $ 0.017 (0.003)$  & $ 0.017 (0.002)$  & $\textbf{ 0.010 (0.001)}$    \\ \hline
% boston   & $\textbf{\textit{ 0.088 (0.008) }}$   & $ 0.095 (0.008) $  & $ 0.094 (0.009)$  & $ 0.103 (0.013)$  & $\textbf{ 0.063 (0.016)}$    \\ \hline
% kin8nm   & $ 0.078 (0.001) $   & $ 0.104 (0.003) $  & $\textbf{\textit{ 0.077 (0.001)}}$  & $ 0.096 (0.005)$  & $\textbf{ 0.070 (0.001)}$    \\ \hline
% \end{tabular}
% % \caption{\textbf{UCI Check Score} Caption}
% % \end{center}
% % \end{adjustbox}
% % \end{table}
% \end{figure*}
% \vspace{-2mm}

We demonstrate our proposed methods' performance on the standard 8 UCI datasets \citep{asuncion2007uci}, 
and on a real-world problem in nuclear fusion.
To assess the predictions, we use all metrics from Section~\ref{sec:metrics} that can be estimated with a finite test dataset: 1) average calibration vs sharpness, 2) adversarial group calibration, 
3) interval calibration, 4) check score (note, this is identical to pinball loss), 
and 5) interval score.

To measure the calibration metrics (average, interval, adversarial group),
we discretized the expected probabilities from 0.01 to 0.99 in 0.01 increments
(i.e. 0.01, 0.02, \dots, 0.97, 0.98, 0.99)
% we scaled the expected probabilities from $0.01$ to $0.99$ in $0.01$ increments 
and estimated ECE (Eq.~\ref{eq:ece}) according to this finite discretization.
For interval calibration, for each expected probability $p$, 
we predict centered $p$ PIs, and calculate $\hat{p}^{\text{obs}}_{avg}$ 
as the proportion of test points falling within the PI.
Appendix~\ref{app:data_exp_details} details how we estimated adversarial group calibration.
Sharpness was measured as the mean width of the $95\%$ centered PI (i.e. between quantile levels $p=0.025$ and $0.975$). 
The proper scoring rules (check, interval) were measured as the average of the score on the test set.
% \begin{enumerate}
%     \item Average calibration vs sharpness: We measure the error in average calibration on the test set according to Equation~\ref{eq:ece}.
%     and $p$ is discretized in $0.01$ increments ($0.01,\dots, 0.99)$. Sharpness is measured with the mean of the width of a centered 95\% interval (width between $p=0.025$ and $0.975$). 
%     \item Adversarial group calibration: we draw random subsets from the test set, and scale the size of the subset from 1\% to 100\% of the full test dataset size. For each subset size, we record the \textit{worst} calibration measured across random draws of the subset.
%     \item Interval calibration: we predict centered $(1-\alpha)$ prediction intervals, for all $\alpha=0.01, 0.02,\dots 0.99$ and measure miscalibration according to \ref{eq:ece} with $p^{\text{obs}}_{avg}$ calculated as the proportion of test points falling within the predicted interval.
%     \item Check score: measured as average of check score (pinball loss) on the test set
%     \item Interval score: measured as average of interval score on the test set 
% \end{enumerate}


We provide a comparison against current state-of-the-art UQ methods 
for which computing the above metrics is tractable. 
\textit{SQR} \citep{tagasovska2019single} is an NN model that optimizes the pinball loss
for a batch of random quantile levels $p\sim U(0,1)$.
\textit{mPAIC} \citep{zhao2020individual} is a randomized extension of 
probabilistic neural networks \citep{lakshminarayanan2017simple, nix1994estimating}
that optimizes a combination of the standard Gaussian NLL and 
a loss that is designed to induce individual calibration.

While more quantile and PI based UQ methods exist, 
they are mostly designed to output a single quantile level or interval coverage level,
which makes measuring calibration extremely expensive (training up to 100 models separately).
For these methods, we provide a comparison on a simplified task of predicting $95\%$ PI in Appendix~\ref{app:coverage_95}.
Lastly, one method that can additionally be considered is the recalibration algorithm by \citet{kuleshov2018accurate}.
This algorithm is not a standalone UQ method, but a refinement step that can be applied on top of other methods. 
We find that applying this recalibration may improve the average calibration of a prediction, 
but does so at a significant cost in sharpness, hence is not a robust remedy.
We discuss recalibration results in Appendix~\ref{app:recal}.

All experimental results report the mean and standard error across 5 trials: error bars and shades in plots indicate $\pm 1$ standard error; in numeric tables, the mean is presented with 1 standard error in parentheses.  
% \subsection{Toy} \label{sec:toy}
% Show that pinball loss doesn't go to correct true quantiles. Show that all of our methods do. 




% \vspace{-2mm}
\subsection{Benchmark UCI Datasets} \label{sec:uci}
% \vspace{-2mm}


\begin{figure*}[ht!]
    \centering
    
    \includegraphics[width=\textwidth]{arXiv/figs/full_calibration_table_uci.pdf}
    
    \caption{\textbf{UCI Average Calibration-Sharpness Table.}
    The table shows mean average calibration (measured by ECE) and sharpness in parentheses, along with $\pm 1$ standard error. 
    The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined. 
    All values have been multiplied by 100 for readability.
    }
    \label{fig:uci_ece_sharp_table_full}
    % \vspace{-1mm}
    % \vspace{-4mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.6\textwidth]{figs/fusion_gc.png}
    % \includegraphics[width=1.0\textwidth]{AISTATS2021/figs/fusion_gc.png}
    %
    % \includegraphics[width=8.5cm, height=4cm]{AISTATS2021/figs/uci_cal_sharp.pdf}
    % \includegraphics[width=8.5cm, height=4cm]{AISTATS2021/figs/uci_group_cali.pdf}
    %
    \hspace{3mm}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/uci_group_cali.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/uci_group_cali_all_8.pdf}
    % \includegraphics[width=0.97\textwidth]{AISTATS2021/figs/fusion_cal_sharp_onerow.pdf}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali_onerow.pdf}
    \caption{
    \textbf{UCI Adversarial Group Caibration.}
    The plot displays the worst calibration error incurred for any group of any given size. The mean is plotted along with $\pm1$ standard error in shades. Group size here refers to the proportion of the test dataset size.}
    % \williex{fusion plots a placeholder for now, will replace with UCI plots} 
    % \williex{TODO: write that all plots are in the appendix}}
    \label{fig:uci_plots}
    % \vspace{-4mm}
\end{figure*}

\begin{figure*}[t] 
% \begin{table}[ht!]
% \begin{adjustbox}{width=8.5cm, height=1.5cm}
% \begin{adjustbox}{width=1.1\columnwidth,center}
\setlength\doublerulesep{3pt}
\begin{center} 
\begin{tabular}{ |c|  |c|c|c|c|c|c| } 
 \hline
         & \textit{SQR}                         & \textit{\textbf{MAQR}}             \\ \Xhline{3\arrayrulewidth} %\hhline{|=||=|=|}
concrete & $8.5 (0.6)$               & $\mathbf{  5.9 \pm  0.8 }$    \\ \hline
power    & $\mathbf{5.7 \pm 0.1 }$   & $ 5.8 \pm  0.1 $              \\ \hline
wine     & $20.5 \pm 0.8 $           & $\mathbf{ 19.1 \pm 0.3}$    \\ \hline
yacht    & $1.2 \pm  0.2 $           & $\mathbf{ 0.7 \pm  0.1}$    \\ \hline
naval    & $7.0 \pm  0.1 $           & $\mathbf{ 0.4 \pm  0.0}$    \\ \hline
energy   & $1.4 \pm  0.0 $           & $\mathbf{ 1.0 \pm  0.1}$    \\ \hline
boston   & $8.8 \pm  0.8 $           & $\mathbf{ 6.3 \pm  1.6}$    \\ \hline
kin8nm   & $7.8 \pm  0.1 $           & $\mathbf{ 7.0 \pm  0.1}$    \\ \hline
% Boston   & $ 8.8 (0.8) $           & $\mathbf{ 6.3 (1.6)}$ \\ \hline
% Concrete & $ 8.5 (0.6) $           & $\mathbf{ 5.9 (0.8)}$ \\ \hline
% Energy   & $ 1.4 (0.0) $           & $\mathbf{ 1.0 (0.1)}$ \\ \hline
% Kin8nm   & $ 7.8 (0.1) $           & $\mathbf{ 7.0 (0.1)}$ \\ \hline
% Naval    & $ 7.0 (0.1) $           & $\mathbf{ 0.4 (0.0)}$ \\ \hline
% power    & $\mathbf{ 0.057 (0.001) }$  & $ 0.058 (0.001) $         \\ \hline
% wine     & $ 0.205 (0.008) $           & $\mathbf{ 0.191 (0.003)}$ \\ \hline
% yacht    & $ 0.012 (0.002) $           & $\mathbf{ 0.007 (0.001)}$ \\ \hline
\end{tabular}
\hspace{0.3pt}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 \textit{\textbf{Interval}}  & \textit{\textbf{MAQR}}              \\ \Xhline{3\arrayrulewidth} %\hhline{|=|=|}
$ 94.3 (5.3)$     & $ \mathbf{67.2 (11.8)}$  \\ \hline
$ 62.0 (1.0)$   & $ \mathbf{59.2 (0.9)}$  \\ \hline
$ 219.7 (4.5)$   & $ \mathbf{205.2 (5.2)}$  \\ \hline
$ 19.0 (2.1)$   & $ \mathbf{8.6 (1.6)}$  \\ \hline
$ 62.0 (11.4)$    & $ \mathbf{4.4 (0.1)}$  \\ \hline
$ 18.2 (2.6)$     & $ \mathbf{10.1 (0.6)}$  \\ \hline
$ 101.0 (11.8)$   & $ \mathbf{86.4 (28.7)}$  \\ \hline
$ 77.6 (1.7)$     & $ \mathbf{69.1 (1.5)}$  \\ \hline
\end{tabular}
\hspace{0.3pt}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 \textit{\textbf{Interval}}  & \textit{\textbf{MAQR}}     \\ \Xhline{3\arrayrulewidth} %\hhline{|=|=|}
$ 6.1 (0.8)$   & $ \mathbf{5.9 (2.0)}$  \\ \hline
$ 2.3 (0.3)$   & $ \mathbf{1.0 (0.2)}$  \\ \hline
$ 7.9 (1.4)$   & $ \mathbf{4.5 (0.5)}$  \\ \hline
$ 12.1 (0.5)$   & $ \mathbf{8.5 (2.4)}$  \\ \hline
$ 4.3 (1.4)$   & $ \mathbf{1.2 (0.2)}$  \\ \hline
$ 6.0 (1.0)$   & $ \mathbf{5.2 (1.8)}$  \\ \hline
$ \mathbf{7.9 (1.5)}$   & $ 9.2 (4.1)$  \\ \hline
$ 4.8 (0.6)$   & $ \mathbf{1.9 (0.8)}$  \\ \hline
  
%  $ \mathbf{7.9 (1.5)}$   & $ 9.2 (4.1)$  \\ \hline
%  $ 6.1 (0.8)$   & $ \mathbf{5.9 (2.0)}$  \\ \hline
%  $ 6.0 (1.0)$   & $ \mathbf{5.2 (1.8)}$  \\ \hline
%  $ 4.8 (0.6)$   & $ \mathbf{1.9 (0.8)}$  \\ \hline
%  $ 4.3 (1.4)$   & $ \mathbf{1.2 (0.2)}$  \\ \hline
%  $ 0.023 (0.003)$   & $ \mathbf{0.010 (0.002)}$  \\ \hline
%  $ 0.079 (0.014)$   & $ \mathbf{0.045 (0.005)}$  \\ \hline
%  $ 0.121 (0.005)$   & $ \mathbf{0.085 (0.024)}$  \\ \hline
\end{tabular}
\caption{\textbf{UCI Experiments.} \textbf{Left}: Check  score. \textbf{Middle}: Interval score. 
\textbf{Right}: Interval Calibration. Each table shows the top two methods only, in
terms of average performance. Full set of results (additional methods and datsets) are
in Appendix~\ref{app:all_uci_results}. The highest scoring results for each
dataset are shown in \textbf{bold}.
\label{fig:uci_numbers}}
\end{center}
\end{figure*}


We evaluate 5 methods on the 8 UCI datasets: three proposed algorithms---\textit{MAQR}, \textit{Cali} (penalized calibration loss), and \textit{Interval} (interval score)---and 2 alternative algorithms---\textit{SQR} and \textit{mPAIC}.
% Results from the first 5 datasets in alphabetical order are presented, 
% and the full set of results are in Appendix~\ref{app:all_uci_results}.
We use the the same NN architecture, learning rate, and training details
for all methods.
% , and we follow
% the same training procedure by halting training based on validation loss.
Appendix~\ref{app:uci_exp_details} includes more details on the experiment setup and hyperparameters.

The average calibration-sharpness metrics are presented in table form in Figure~\ref{fig:uci_ece_sharp_table_full}.
\textit{MAQR} seems to be best at producing calibrated models and achieves the best calibration on 7 out of 8 datasets. 
% and sometimes dominates other methods in \textit{both} calibration and sharpness. 
Adversarial group calibration in Figure~\ref{fig:uci_plots} also indicates that 
\textit{MAQR} generally tends to achieve lowest calibration error across \textit{any} random group of \textit{any} size with more than one point (6 out of 8 datasets).
The check and interval scores in the tables in Figure~\ref{fig:uci_numbers} also rank 
\textit{MAQR}'s prediction as best, which is surprising given that 
\textit{SQR} is a NN of the same capacity that was explicitly trained to optimize the check score, 
and likewise for \textit{Interval} with the interval score.
This indicates the distribution predicted by \textit{MAQR} is fundamentally different 
as it utilizes direct estimates of the conditional distribution,
while the other methods all optimize a specific loss function.

\textbf{Excluding \textit{MAQR}}: Figure~\ref{fig:uci_ece_sharp_table_full} shows \textit{SQR}, \textit{Interval} and \textit{Cali} all producing competitive calibration-sharpness results (i.e. there is no other method that is dominant in \textit{both} calibration and sharpness), with \textit{mPAIC} performing the poorest.
Notably, \textit{SQR} tends to produce the sharpest predictions,
which is not surprising following Proposition 1.
Adversarial group calibration in Figure~\ref{fig:uci_plots}, however, suggests that \textit{SQR}'s predictions have not approached the true conditional quantiles well:
e.g. on the Energy dataset, \textit{SQR} reports better average calibration on the full test set than \textit{mPAIC},
but \textit{mPAIC} is better adversarially calibrated than \textit{SQR}.
Centered interval calibration in Figure~\ref{table:app_uci_centered_interval}, Appendix~\ref{app:all_uci_results} suggests that
\textit{Interval} produces better calibrated centered intervals, 
even when average calibration was worse (e.g. Power dataset, Figure~\ref{table:app_uci_centered_interval}).


% \vspace{-2mm}
\subsection{Modeling Uncertainty in Nuclear Fusion} \label{sec:fusion}
% \vspace{-2mm}

We further demonstrate the performance of our algorithms on a 
high-dimensional task from nuclear fusion: quantifying uncertainty in plasma dynamics. 
The plasma data was recorded from the DIII-D tokamak, a nuclear fusion device operated by General Atomics \citep{luxon2002design}. 
Plasma dynamics during fusion reactions are highly stochastic and running live fusion experiments is costly. 
Hence, practitioners use this dataset to learn a dynamics model of the system, 
for various purposes such as learning a controller to optimize reaction efficiency and stability \citep{fu2020machine, boyer2019feedback, boyer2019real}.
There are 10 scalar target signals to model in this dataset (full list in Appendix~\ref{app:fusion_exp_details}), 
each describing a particular aspect of the current state of plasma.
For each signal, the input features are 468 dimensional.
We do not apply \textit{MAQR} on this dataset because of the high computational costs and statistical challenge associated with nonparametric density estimation in high dimensions.
% We do not apply MAQR on this dataset because estimating localities in the domain space for conditional density estimation 
% is intractable in such high dimensions.
Appendix~\ref{app:fusion_exp_details} provides more details on the data and experiment setup. 

Results on the first 5 signals (alphabetical order) are presented here, 
and the full set of results are in Appendix~\ref{app:all_fusion_results}.
Average calibration and sharpness are shown in a 2-dimensional scatter-plot
in the top row of Figure~\ref{fig:fusion_plots}, where a similar pattern can be observed across the signals:
\textit{SQR} produces the sharpest predictions, \textit{Cali} and \textit{Interval} are most calibrated 
with \textit{Cali} sharper than \textit{Interval}, 
and \textit{mPAIC} performs the poorest with least calibrated and sharp predictions.
It is generally known that plasma dynamics display complex stochasticity
\citep{fu2020machine, kowal2020kelvin}, and hence we suspect \textit{mPAIC}'s
performance degrades significantly because 
it assumes a Gaussian output and is trained according to the Gaussian likelihood.

\begin{figure*}[ht]
    \centering
    % \includegraphics[width=8.5cm, height=3.5cm]{figs/fusion_cal_sharp.pdf}
    % \includegraphics[width=8.5cm, height=3.5cm]{figs/fusion_group_cali.pdf}
    % \caption{\textbf{Fusion Calibration-Sharpness} Caption}
    %
    % \includegraphics[width=\textwidth]{figs/fusion_first_five.pdf}
    \includegraphics[width=\textwidth]{arXiv/figs/fusion_first_five_all_8.pdf}
    %
    % \hspace{3mm}
    % \includegraphics[width=0.97\textwidth]{figs/fusion_cal_sharp_onerow.pdf}
    % \includegraphics[width=\textwidth]{figs/fusion_group_cali_onerow.pdf}
    \caption{\textbf{Nuclear Fusion Experiments.} \textbf{Top row:} Average calibration and sharpness. \textbf{Bottom row:} Adversarial group calibration (group size refers to proportion of dataset size). Full set of results
    (additional signals) are in Appendix~\ref{app:all_fusion_results}.}
    \label{fig:fusion_plots}
\end{figure*}

\begin{figure*}[ht!]
\begin{center} 
\setlength\doublerulesep{3pt}
\begin{tabular}{ |c| |c|c|c|c|c|c| } 
 \hline
            & \textit{SQR}       & \textit{mPAIC}            & \textit{\textbf{Interval}}           & \textit{\textbf{Cali}}                      \\ \Xhline{3\arrayrulewidth} %\hhline{|=||=|=|=|=|}
 aminor        & $ 8.1 (0.6) $   & $ 26.8 (0.0) $  & $\textbf{ 5.5 (0.7)} $ & $ 5.8 (0.4)$ \\ \hline
dssdenest     & $ 7.2 (0.3) $   & $ 16.2 (0.3) $  & $\textbf{ 5.4 (0.6)} $ & $ 7.1 (0.8)$ \\ \hline
efsbetan      & $\textbf{5.1 (0.1)}$   & $ 16.0 (1.2) $  & $ 8.7 (0.9)$  & $ 5.6 (0.7)$ \\ \hline
efsli         & $ 7.1 (1.1) $   & $ 21.4 (1.7) $  & $ 6.9 (1.3)$  & $\textbf{ 4.3 (0.3)} $\\ \hline
efsvolume     & $ 7.3 (0.7) $   & $ 31.5 (2.2) $  & $ 6.3 (0.7)$  & $\textbf{ 5.6 (0.2)} $\\ \hline
%  ip         & $ 0.051 (0.003) $   & $ 0.227 (0.020) $  & $ 0.077 (0.015)$  & $\textbf{ 0.036 (0.003)} $\\ \hline
%  kappa      & $ 0.069 (0.008) $   & $ 0.254 (0.014) $  & $ 0.078 (0.011)$  & $\textbf{ 0.053 (0.004)} $\\ \hline
%  R0         & $ 0.068 (0.007) $   & $ 0.168 (0.009) $  & $\textbf{ 0.058 (0.007)} $ & $ 0.066 (0.004)$ \\ \hline
%  tribot     & $ 0.087 (0.006) $   & $ 0.227 (0.016) $  & $\textbf{ 0.074 (0.008)} $ & $ 0.080 (0.007)$ \\ \hline
%  tritop     & $ 0.077 (0.006) $   & $ 0.231 (0.017) $  & $ 0.058 (0.015)$  & $ \textbf{0.037 (0.004)}$ \\ \hline
\end{tabular}
\caption{\textbf{Interval Calibration on Nuclear Fusion Experiments.} 
The highest scoring results for each signal are shown in \textbf{bold}.
Full set of results (additional signals and metrics) are in the Appendix~\ref{app:all_fusion_results}. \label{table:fusion_numbers}}
\end{center}
\end{figure*}

Adversarial group calibration in bottom row of Figure~\ref{fig:fusion_plots} suggests that 
\textit{SQR} has significantly traded off calibration for sharpness when compared to
\textit{Cali} and \textit{Interval}. 
Comparing \textit{Cali} and \textit{Interval}, we see that \textit{Cali} oftentimes
dominates \textit{Interval} in both average calibration and sharpness, and also
achieves better adversarial group calibration. 

Interval calibration in 
the table in Figure~\ref{table:fusion_numbers} also shows that \textit{Cali} produces
competitive centered intervals, suggesting that \textit{Cali} has better
estimated the conditional quantiles, in general.


\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c||c|c|}
 \hline & \multicolumn{2}{c|}{\textbf{\textit{Cali}}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}               \\\hline
Concrete & $6.6\pm0.9(17.6\pm2.3)$ & $\textbf{5.6}\pm0.8(\underline{17.3}\pm1.5)$ \\ \hline
Power    & $\textbf{1.7}\pm0.2(14.2\pm0.3)$ & $2.0\pm0.1(\underline{13.1}\pm0.1)$    \\ \hline
Wine     & $4.4\pm0.5(\underline{25.6}\pm0.8)$ & $\textbf{4.2}\pm0.4(26.0\pm0.8)$ \\ \hline
Yacht    & $11.1\pm1.8(\underline{1.8}\pm0.1)$ & $\textbf{8.3}\pm0.6(2.0\pm0.4)$     \\ \hline
Naval    & $2.8\pm0.2(\underline{12.1}\pm3.1)$ & $\textbf{2.4}\pm0.3(50.6\pm8.6)$    \\ \hline
Energy   & $9.2\pm0.3(\underline{2.8}\pm0.1)$ & $\textbf{5.8}\pm0.4(3.6\pm0.3)$  \\ \hline
Boston   & $9.7\pm1.3(\underline{10.2}\pm0.7)$ & $\textbf{8.5}\pm1.5(10.9\pm0.6)$ \\ \hline
Kin8nm   & $\textbf{3.4}\pm0.3(\underline{13.7}\pm0.4)$ & $3.5\pm0.3(\underline{13.7}\pm0.7)$ \\ \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |c||c|c|}
 \hline & \multicolumn{2}{c|}{\textbf{\textit{SQR}}} \\
 \hline
          & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Concrete  & $9.8\pm1.3(\underline{7.0}\pm0.6)$ & $\textbf{7.1}\pm0.9(8.5\pm0.6)$ \\ \hline
Power     & $\textbf{2.5}\pm0.3(14.0\pm0.5)$ & $2.9\pm0.5(\underline{13.6}\pm0.8)$ \\ \hline
Wine      & $4.5\pm0.4(29.7\pm0.5)$ & $\textbf{4.0}\pm0.4(\underline{28.5}\pm0.8)$ \\ \hline
Yacht     & $9.0\pm0.9(\underline{0.9}\pm0.1)$ & $\textbf{8.9}\pm0.9(2.3\pm0.2)$ \\ \hline
Naval     & $8.6\pm1.6(\underline{3.6}\pm0.1)$ & $\textbf{5.3}\pm0.8(6.0\pm0.5)$ \\ \hline
Energy    & $10.2\pm0.8(\underline{1.8}\pm0.1)$ & $\textbf{6.9}\pm1.1(2.4\pm0.2)$ \\ \hline
Boston    & $10.9\pm1.0(\underline{8.8}\pm1.1)$ & $\textbf{9.8}\pm1.2(9.5\pm0.9)$ \\ \hline
Kin8nm    & $4.7\pm0.3(\underline{11.1}\pm0.1)$ & $\textbf{3.9}\pm0.4(11.3\pm0.2)$ \\ \hline
\end{tabular}
\end{center}
\caption{\textbf{Group Batching Ablation: Average Calibration and Sharpness.}
    The table shows mean ECE and sharpness (in parentheses) and their standard error with and without group batching. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined for \textit{Cali} and \textit{SQR} separately. All values have been multiplied by 100 for readability.\label{table:group_batch_ablation}}

% \end{center}
% \vspace{-5mm}
\end{figure*}


% \begin{figure*}[h!]
% \begin{center} 
% \begin{tabular}{ |c||c|c || c|c|c|}
%  \hline & \multicolumn{2}{c||}{\textit{Cali}} & \multicolumn{2}{c|}{\textit{SQR}} \\
%  \hline
%           & \textit{Random Batch}                 & \textit{Group Batch}            & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
% Boston & $9.7\pm1.3(\underline{10.2}\pm0.7)$ & $\textbf{8.5}\pm1.5(10.9\pm0.6)$ & $10.9\pm1.0(\underline{8.8}\pm1.1)$ & $\textbf{9.8}\pm1.2(9.5\pm0.9)$ \\ \hline
% Concrete & $6.6\pm0.9(17.6\pm2.3)$ & $\textbf{5.6}\pm0.8(\underline{17.3}\pm1.5)$ & $9.8\pm1.3(\underline{7.0}\pm0.6)$ & $\textbf{7.1}\pm0.9(8.5\pm0.6)$ \\ \hline
% Energy & $9.2\pm0.3(\underline{2.8}\pm0.1)$ & $\textbf{5.8}\pm0.4(3.6\pm0.3)$ & $10.2\pm0.8(\underline{1.8}\pm0.1)$ & $\textbf{6.9}\pm1.1(2.4\pm0.2)$ \\ \hline
% Kin8nm & $\textbf{3.4}\pm0.3(\underline{13.7}\pm0.4)$ & $3.5\pm0.3(\underline{13.7}\pm0.7)$ & $4.7\pm0.3(\underline{11.1}\pm0.1)$ & $\textbf{3.9}\pm0.4(11.3\pm0.2)$ \\ \hline
% Wine & $4.4\pm0.5(\underline{25.6}\pm0.8)$ & $\textbf{4.2}\pm0.4(26.0\pm0.8)$ & $4.5\pm0.4(29.7\pm0.5)$ & $\textbf{4.0}\pm0.4(\underline{28.5}\pm0.8)$ \\ \hline
% Yacht & $11.1\pm1.8(\underline{1.8}\pm0.1)$ & $\textbf{8.3}\pm0.6(2.0\pm0.4)$ & $9.0\pm0.9(\underline{0.9}\pm0.1)$ & $\textbf{8.9}\pm0.9(2.3\pm0.2)$ \\ \hline
% Power & $\textbf{1.7}\pm0.2(14.2\pm0.3)$ & $2.0\pm0.1(\underline{13.1}\pm0.1)$ & $\textbf{2.5}\pm0.3(14.0\pm0.5)$ & $2.9\pm0.5(\underline{13.6}\pm0.8)$ \\ \hline
% Naval & $2.8\pm0.2(\underline{12.1}\pm3.1)$ & $\textbf{2.4}\pm0.3(50.6\pm8.6)$ & $8.6\pm1.6(\underline{3.6}\pm0.1)$ & $\textbf{5.3}\pm0.8(6.0\pm0.5)$ \\ \hline
% \end{tabular}
% \caption{\textbf{Group Batching Ablation: Average Calibration and Sharpness.}
%     The table shows mean ECE and sharpness (in parentheses) and their standard error with and without group batching. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined for \textit{Cali} and \textit{SQR} separately. All values have been multiplied by 100 for readability.} \label{fig:group_batch_ablation}
% \end{center}
% \vspace{-5mm}
% \end{figure*}

\subsection{Ablation Study: Effect of Group Batching} \label{sec:ablation}
% \vspace{-2mm}
Lastly, we provide an ablation study on the effect of group batching (experiment details in Appendix~\ref{app:ablation_study_exp_setting}).
Figure~\ref{table:group_batch_ablation} displays how group batching 
affects average calibration-sharpness of
one proposed method (\textit{Cali}) and one baseline method (\textit{SQR}) on all 8 UCI datasets.
Average calibration improved on 6 out of 8 datasets for \textit{Cali},
and on 7 out of 8 datasets on \textit{SQR}.
While sharpness tends to worsen (increase) with group batching, 
we note that higher sharpness \textit{is} desirable 
if there actually exists high noise in the true data distribution.
In Appendix~\ref{app:full_ablation_results}, we show that group batching also improves adversarial group calibration, suggesting that the underlying data distribution truly does have high noise.
This study indicates that deliberately taking batches during training that do not follow $\F_{\mathbf{X}}$ can help to improve UQ performance.



% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/fusion_cal_sharp.pdf}
%     \caption{\textbf{Fusion Calibration-Sharpness} Caption}
%     \label{fig:fusion_cal_sharp}
%     \vspace{-4mm}
% \end{figure*}

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/fusion_group_cali.pdf}
%     \caption{\textbf{Fusion Adversarial Group Calibration} Caption}
%     \label{fig:fusion_gc}
%     \vspace{-4mm}
% \end{figure*}


==> NeurIPS2021/experiments.tex <==
\vspace{-2mm}
\section{Experiments}
% \label{sec:experiments_with_ablation}
\label{sec:experiments}
\vspace{-1mm}

% \begin{figure*}[t]
% % \begin{table}[ht!]
% % \begin{adjustbox}{width=8.5cm, height=1.5cm}
% % \begin{adjustbox}{width=1.1\columnwidth,center}
% % \begin{center} \label{table:uci_check}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & SQR                 & IndvCal            & \textbf{Int}      & \textbf{Cali}     & \textbf{MAQR}        \\\hline
% concrete & $\textit{ 0.085 (0.006) }$   & $\textbf{\textit{ 0.085 (0.005) }}$  & $ 0.086 (0.004)$  & $ 0.118 (0.006)$  & $\textbf{ 0.059 (0.008)}$    \\ \hline
% power    & $\textbf{ 0.057 (0.001) }$   & $ 0.070 (0.001) $  & $ 0.062 (0.001)$  & $ 0.064 (0.001)$  & $\textbf{\textit{ 0.058 (0.001)}}$    \\ \hline
% wine     & $\textbf{\textit{ 0.205 (0.008) }}$   & $ 0.219 (0.004) $  & $ 0.214 (0.006)$  & $ 0.210 (0.008)$  & $\textbf{ 0.191 (0.003)}$    \\ \hline
% yacht    & $\textbf{\textit{ 0.012 (0.002) }}$   & $ 0.015 (0.002) $  & $ 0.018 (0.003)$  & $ 0.019 (0.004)$  & $\textbf{ 0.007 (0.001)}$    \\ \hline
% naval    & $ 0.070 (0.001) $   & $\textbf{\textit{ 0.276 (0.004) }}$  & $ 0.066 (0.013)$  & $ 0.159 (0.029)$  & $\textbf{ 0.004 (0.000)}$    \\ \hline
% energy   & $\textbf{\textit{ 0.014 (0.000) }}$   & $ 0.015 (0.001) $  & $ 0.017 (0.003)$  & $ 0.017 (0.002)$  & $\textbf{ 0.010 (0.001)}$    \\ \hline
% boston   & $\textbf{\textit{ 0.088 (0.008) }}$   & $ 0.095 (0.008) $  & $ 0.094 (0.009)$  & $ 0.103 (0.013)$  & $\textbf{ 0.063 (0.016)}$    \\ \hline
% kin8nm   & $ 0.078 (0.001) $   & $ 0.104 (0.003) $  & $\textbf{\textit{ 0.077 (0.001)}}$  & $ 0.096 (0.005)$  & $\textbf{ 0.070 (0.001)}$    \\ \hline
% \end{tabular}
% % \caption{\textbf{UCI Check Score} Caption}
% % \end{center}
% % \end{adjustbox}
% % \end{table}
% \end{figure*}
\vspace{-2mm}

%%%%% \
%%%%% BEGIN: UCI Figures
%%%%% /
\begin{figure*}[t!]
    \centering
    
    \includegraphics[width=\textwidth]{NeurIPS2021/figures/full_uci_cal_sharp_table.pdf}
    \includegraphics[width=\textwidth]{NeurIPS2021/figures/uci_group_cali_first_5.pdf}
    
    \caption{\textbf{UCI Experiments.}  
    \textbf{(Top Table):} Average calibration (measured by ECE) and sharpness in parentheses. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined (all values multiplied by 100 for readability).
    \textbf{(Bottom Figure):} Adversarial group calibration for the first 5 UCI datasets (full set of results in Appendix~\ref{app:all_uci_results}). Group size refers to proportion of test dataset size. 
    % Because of limited space, only the first four fusion datasets are shown here, but the full table can be found in Appendix~\ref{app:all_experiments}.
    }
    \label{fig:uci_table_figure}
    \vspace{-3mm}
\end{figure*}
%%%%% \
%%%%% END: UCI Figures
%%%%% /



%%%%% \
%%%%% BEGIN: FUSION Figures
%%%%% /
\begin{figure*}[t!]
    \centering
    
    \includegraphics[width=0.95\textwidth]{NeurIPS2021/figures/full_fusion_cal_sharp_table.pdf}
    \includegraphics[width=\textwidth]{NeurIPS2021/figures/fusion_group_cali_first_5.pdf}
    
    \caption{\textbf{Fusion Experiments.}  
    \textbf{(Top Table):} Average calibration (measured by ECE) and sharpness in parentheses. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined (all values multiplied by 100 for readability).
    \textbf{(Bottom Figure):} Adversarial group calibration for the first 5 fusion datasets (full set of results in Appendix~\ref{app:all_fusion_results}). Group size refers to proportion of test dataset size. 
    % Because of limited space, only the first four fusion datasets are shown here, but the full table can be found in Appendix~\ref{app:all_experiments}.
    }
    \label{fig:fusion_table_figure}
    \vspace{-4mm}
\end{figure*}
%%%%% \
%%%%% END: FUSION Figures
%%%%% /





We demonstrate the performances of our proposed methods on the standard 8 UCI datasets \cite{asuncion2007uci}, 
and on a real-world problem in nuclear fusion. 
To assess the predictions, we use all metrics from Section~\ref{sec:metrics} that can be estimated with a finite test dataset: 1) average calibration vs sharpness, 2) adversarial group calibration, 
3) centered interval calibration, 4) check score, and 5) interval score.
The results for the first two of these metrics are displayed in the main body of the paper, and the results for the other three metrics are shown in Appendix~\ref{app:all_experiments} due to space restrictions.
% Since average calibration must always be inspected together
% with sharpness (Section~\ref{sec:metrics}), they are plotted together during evaluation (e.g. Figure~\ref{fig:uci_plots}, top row).
We describe how each of these evaluation metrics are calculated in
Appendix~\ref{app:measuring_metrics}.



% To measure the calibration metrics (average, centered interval, adversarial group),
% we discretized the expected probabilities 
% from $0.01$ to $0.99$ in $0.01$ increments 
% and estimated ECE (\ref{eq:ece}) according to this finite discretization.
% For centered interval calibration, for each expected probability $p$, 
% we predict centered $p$ PIs, and calculate $\hat{p}^{\text{obs}}_{avg}$ 
% as the proportion of test points falling within the PI. 
% The full equation for centered interval calibration is in Appendix~\ref{app:data_exp_details}, which also includes details on how we estimated adversarial group calibration.
% Sharpness was measured as the mean width of the $95\%$ centered PI (i.e. between  $p=0.025$ and $0.975$). 
% The proper scoring rules (check and interval scores) were measured as the average of the score on the test set.


% \begin{enumerate}
%     \item Average calibration vs sharpness: We measure the error in average calibration on the test set according to Equation~\ref{eq:ece}.
%     and $p$ is discretized in $0.01$ increments ($0.01,\dots, 0.99)$. Sharpness is measured with the mean of the width of a centered 95\% interval (width between $p=0.025$ and $0.975$). 
%     \item Adversarial group calibration: we draw random subsets from the test set, and scale the size of the subset from 1\% to 100\% of the full test dataset size. For each subset size, we record the \textit{worst} calibration measured across random draws of the subset.
%     \item Interval calibration: we predict centered $(1-\alpha)$ prediction intervals, for all $\alpha=0.01, 0.02,\dots 0.99$ and measure miscalibration according to \ref{eq:ece} with $p^{\text{obs}}_{avg}$ calculated as the proportion of test points falling within the predicted interval.
%     \item Check score: measured as average of check score (pinball loss) on the test set
%     \item Interval score: measured as average of interval score on the test set 
% \end{enumerate}

We provide a comparison against current state-of-the-art UQ methods 
for which computing the above metrics is tractable. 
\textit{SQR} \cite{tagasovska2019single} is an NN model that optimizes the pinball loss
for a batch of random quantile levels $p\sim U(0,1)$.
\textit{mPAIC} \cite{zhao2020individual} is an extension of 
probabilistic neural networks \cite{lakshminarayanan2017simple, nix1994estimating}
that optimizes a combination of the standard Gaussian NLL and 
a loss that induces individual calibration.
While additional quantile and PI based UQ methods exist, 
they are mostly designed to output a single quantile level or interval coverage level,
which makes measuring calibration extremely expensive (training up to 100 models separately).
For these methods, we provide a comparison on a simplified task of predicting $95\%$ PI in Appendix~\ref{app:coverage_95}.
Lastly,
% one method that we could also consider is the
we could also consider the recalibration algorithm of \citet{kuleshov2018accurate},
which is not a standalone UQ method, but a refinement step that can be applied on top of other methods. 
We discuss recalibration results in Appendix~\ref{app:recal}.
%
% All experimental results report the mean and standard error across 5 trials. Error bars and shaded bands in plots indicate $\pm 1$ standard error.
All results report the mean and error across 5 trials. Error bars and shaded bands in plots indicate $\pm 1$ standard error.
% in numeric tables, the mean is presented with 1 standard error in parentheses.  
% \subsection{Toy} \label{sec:toy}
% Show that pinball loss doesn't go to correct true quantiles. Show that all of our methods do. 













% %%%%% \
% %%%%% BEGIN: Original Fusion first 5 Cal-Sharp/AdvGroupCal, two rows
% %%%%% /
% \begin{figure*}[ht!]
%     \centering
%     % \includegraphics[width=8.5cm, height=3.5cm]{AISTATS2021/figs/fusion_cal_sharp.pdf}
%     % \includegraphics[width=8.5cm, height=3.5cm]{AISTATS2021/figs/fusion_group_cali.pdf}
%     % \caption{\textbf{Fusion Calibration-Sharpness} Caption}
%     %
%     \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_first_five.pdf}
%     %
%     % \hspace{3mm}
%     % \includegraphics[width=0.97\textwidth]{AISTATS2021/figs/fusion_cal_sharp_onerow.pdf}
%     % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali_onerow.pdf}
%     \caption{Nuclear Fusion Experiments. \textbf{Top row:} Average calibration and sharpness. \textbf{Bottom row:} Adversarial group calibration (group size refers to proportion of dataset size). Full set of results
%     (additional signals) are in Appendix~\ref{app:all_fusion_results}.}
%     \label{fig:fusion_plots}
%     \vspace{-1mm}
% \end{figure*}
% %%%%% \
% %%%%% END: Original Fusion first 5 Cal-Sharp/AdvGroupCal, two rows
% %%%%% /


% %%%%% \
% %%%%% BEGIN: Original Fusion first 5 Centered Interval Calibration Table
% %%%%% /
% \begin{figure*}[ht!]
% \begin{center} 
% \setlength\doublerulesep{3pt}
% \begin{tabular}{ |c| |c|c|c|c|c|c| } 
%  \hline
%             & \textit{SQR}       & \textit{IndvCal}            & \textit{\textbf{Interval}}           & \textit{\textbf{Cali}}                      \\ \Xhline{3\arrayrulewidth} %\hhline{|=||=|=|=|=|}
%  aminor     & $ 0.081 (0.006) $   & $ 0.268 (0.000) $  & $\textbf{ 0.055 (0.007)} $ & $ 0.058 (0.004)$ \\ \hline
%  dssdenest  & $ 0.072 (0.003) $   & $ 0.162 (0.003) $  & $\textbf{ 0.054 (0.006)} $ & $ 0.071 (0.008)$ \\ \hline
%  efsbetan      & $\textbf{0.051 (0.001)}$   & $ 0.160 (0.012) $  & $ 0.087 (0.009)$  & $ 0.056 (0.007)$ \\ \hline
%  efsli         & $ 0.071 (0.011) $   & $ 0.214 (0.017) $  & $ 0.069 (0.013)$  & $\textbf{ 0.043 (0.003)} $\\ \hline
%  efsvolume     & $ 0.073 (0.007) $   & $ 0.315 (0.022) $  & $ 0.063 (0.007)$  & $\textbf{ 0.056 (0.002)} $\\ \hline
% %  ip         & $ 0.051 (0.003) $   & $ 0.227 (0.020) $  & $ 0.077 (0.015)$  & $\textbf{ 0.036 (0.003)} $\\ \hline
% %  kappa      & $ 0.069 (0.008) $   & $ 0.254 (0.014) $  & $ 0.078 (0.011)$  & $\textbf{ 0.053 (0.004)} $\\ \hline
% %  R0         & $ 0.068 (0.007) $   & $ 0.168 (0.009) $  & $\textbf{ 0.058 (0.007)} $ & $ 0.066 (0.004)$ \\ \hline
% %  tribot     & $ 0.087 (0.006) $   & $ 0.227 (0.016) $  & $\textbf{ 0.074 (0.008)} $ & $ 0.080 (0.007)$ \\ \hline
% %  tritop     & $ 0.077 (0.006) $   & $ 0.231 (0.017) $  & $ 0.058 (0.015)$  & $ \textbf{0.037 (0.004)}$ \\ \hline
% \end{tabular}
% \caption{Interval Calibration on Nuclear Fusion Experiments. 
% The highest scoring results for each signal are shown in \textbf{bold}.
% Full set of results (additional signals and metrics) are in the Appendix~\ref{app:all_fusion_results}. \label{table:fusion_numbers}}
% \end{center}
% \vspace{-4mm}
% \end{figure*}
% %%%%% \
% %%%%% END: Original Fusion first 5 Centered Interval Calibration Table
% %%%%% /

\vspace{-3mm}
\subsection{UCI and Fusion Experiments} \label{sec:uci_fusion}
\vspace{-2mm}

\textbf{UCI datasets:}
We evaluate 5 methods on the 8 UCI benchmark datasets: 
three proposed algorithms---\textit{MAQR}, \textit{Cali} (combined calibration loss), and \textit{Interval} (interval score)---and 2 alternative algorithms---\textit{SQR} and \textit{mPAIC}.
Appendix~\ref{app:uci_exp_details} includes more details on the experiment setup and hyperparameters.

\textbf{Fusion datasets:}
We further evaluate the methods on a 
high-dimensional task from nuclear fusion: quantifying uncertainty in plasma dynamics. 
The plasma data was recorded from the DIII-D tokamak, a nuclear fusion device operated by General Atomics \cite{luxon2002design}. 
Plasma dynamics during fusion reactions are highly stochastic and running live fusion experiments is costly. 
Hence, practitioners use this dataset to learn a dynamics model of the system
for various purposes such as controller learning to optimize reaction efficiency and stability \cite{fu2020machine, boyer2019feedback, boyer2019real}.
There are 10 scalar target signals to model in this dataset (full list in Appendix~\ref{app:fusion_exp_details}), 
each describing a particular aspect of the current state of plasma.
For each signal, the input features are 468 dimensional.
We do not apply \textit{MAQR} on this dataset because of the high computational costs and statistical challenge associated with nonparametric density estimation in high dimensions.
% We do not apply MAQR on this dataset because estimating localities in the domain space for conditional density estimation 
% is intractable in such high dimensions.
Appendix~\ref{app:fusion_exp_details} provides more details on the dataset, experiment setup, and hyperparameters. 


\textbf{Analysis of Results:}
Figure~\ref{fig:uci_table_figure} displays average calibration-sharpness for all 8 UCI datasets and
adversarial group calibration for the first 5 UCI datasets (alphabetical order).
\textit{MAQR} produces the best average calibrated models on 7 of the 8 UCI datasets, 
and adversarial group calibration also indicates \textit{MAQR} 
tends to achieve the lowest calibration error across 
\textit{any} random subgroup of \textit{any} size with more than one point (6 out of 8 datasets).
Excluding \textit{MAQR}, \textit{Interval} and \textit{Cali} achieve competitive average calibration and adversarial group calibration on 7 out of 8 UCI datasets.
Notably, \textit{SQR} tends to produce the sharpest predictions across all 
datasets (often at the cost of worse calibration), 
which is not surprising following the discussion in Section~\ref{sec:metrics}. 
Lastly, we also note that \textit{Interval} and \textit{Cali}  
tend to be
% more robust and consistent
less brittle compared to \textit{SQR} and \textit{mPAIC}, 
which incur major failures in some cases (e.g. \textit{mPAIC} in Kin8nm, \textit{SQR} in Naval).

The fusion experiment results display a similar pattern (Figure~\ref{fig:fusion_table_figure}).
\textit{Interval} and \textit{Cali} achieve competitive average
calibration and adversarial group calibration on 9 out of 10 fusion datasets, 
and \textit{SQR} produces the sharpest UQ at the cost worse average and adversarial group calibration (except on betan).
We also observe that \textit{mPAIC} performs the poorest on the fusion datasets, with least calibrated and least sharp predictions.
It is generally known that plasma dynamics display complex stochasticity
\cite{fu2020machine, kowal2020kelvin}, and hence we suspect \textit{mPAIC}'s
performance degrades significantly because 
it assumes a Gaussian output and is trained according to the Gaussian likelihood.

Only a subset of the plots and metrics are shown in the main paper due to space restrictions. Readers are encouraged to see the full set of results in Appendix~\ref{app:all_experiments}, but we summarize the main findings here.
The check score, interval score, and centered interval calibration
in the tables in Appendix~\ref{app:all_uci_results} also rank 
\textit{MAQR}'s prediction as best on the UCI datasets.
This is surprising since \textit{SQR} and \textit{Interval} train NNs of the same capacity to \textit{explicitly minimize} the check and interval scores, respectively.
This indicates the distribution predicted by \textit{MAQR} is fundamentally different 
as it utilizes direct estimates of the conditional distribution,
while the other methods all optimize a specific loss function.
The centered interval calibration metric on the fusion datasets (Appendix~\ref{app:all_fusion_results}) 
indicates that \textit{Cali} and \textit{Interval} both
produce competitive centered PI's (9 out of 10 fusion datasets), 
suggesting that both methods have generally estimated the conditional quantiles better than the alternative algorithms. 


% Figure~\ref{fig:ece_sharp_table} displays calibration-sharpness
% for all 8 UCI datasets and the first 4 fusion datasets (out of 10 total), in alphabetical order. 
% Figure~\ref{fig:adv_group_cal_partial} displays adversarial group calibration 
% for the first 3 UCI datasets and the first fusion dataset, in alphabetical order.
% Due to space constraints, we refer the reader to Appendix~\ref{app:all_uci_results} for the full
% set of results.

% Figure~\ref{fig:ece_sharp_table} shows that \textit{MAQR} achieves 
% best calibration on 7 out of 8 UCI datasets.
% The three plots from left in Figure~\ref{fig:adv_group_cal_partial} show
% that \textit{MAQR} and \textit{Interval} 
% tend to achieve lowest calibration error across 
% \textit{any} random group of \textit{any} size with more than one point.
% The check score, interval score, and centered interval calibration
% in the tables in Figure~\ref{} also rank 
% \textit{MAQR}'s prediction as best, which is surprising given that 
% \textit{SQR} is an NN of the same capacity that was explicitly trained to optimize the check score, 
% and likewise for \textit{Interval} with the interval score.
% This indicates the distribution predicted by \textit{MAQR} is fundamentally different 
% as it utilizes direct estimates of the conditional distribution,
% while the other methods all optimize a specific loss function.

% Excluding \textit{MAQR},
% \textit{Interval} and \textit{Cali} achieve competitive calibration on 
% 7 out of 8 UCI datasets,
% and 3 out of 4 fusion datasets (and 9 out of the 10 on the full set of 10 fusion datasets (Appendix~\label{app:all_fusion_results})).
% Notably, \textit{SQR} tends to produce the sharpest predictions across all 
% datasets and experiments. 
% This is not surprising following Proposition 1. 
% In particular, it is likely that \textit{SQR} is erroneously too sharp 
% given its high calibration error (Figure~\ref{fig:ece_sharp_table}).
% Adversarial group calibration (Figure~\ref{fig:adv_group_cal_partial}) also suggests that \textit{SQR}'s predictions have not approached the true conditional quantiles well, 
% and that it has significantly traded off calibration for sharpness 
% when compared to \textit{Cali} and \textit{Interval}.

% We observe that \textit{mPAIC} performs the poorest on the fusion datasets, with least calibrated and sharp predictions.
% It is generally known that plasma dynamics display complex stochasticity
% \cite{fu2020machine, kowal2020kelvin}, and hence we suspect \textit{mPAIC}'s
% performance degrades significantly because 
% it assumes a Gaussian output and is trained according to the Gaussian likelihood.

% The centered interval calibration metric (fusion: Figure~\ref{app:}) also indicates that \textit{Cali} and \textit{Interval} both
% produce competitive centered intervals (9 out of 10 fusion datasets), 
% suggesting that both methods have better estimated the conditional quantiles, in general.  
% Lastly, we also note that \textit{Interval} and \textit{Cali}  
% tend to be more robust and consistent compared to \textit{SQR} and \textit{mPAIC}, 
% which incur major failures in some cases (e.g. \textit{mPAIC} in Kin8nm, \textit{SQR} in Naval).


%%% BEGIN: ADD IN ABLATION STUDY
\vspace{-2mm}
\subsection{Ablation Study: Effect of Group Batching} \label{sec:ablation}
\vspace{-2mm}
We provide an ablation study on the effect of group batching (experiment details in Appendix~\ref{app:ablation_study_exp_setting}).
Figure~\ref{fig:group_batch_ablation_main} displays how group batching 
affects average calibration-sharpness of
\textit{Cali} and \textit{SQR} on all 8 UCI datasets.
Average calibration improved on 6 out of 8 datasets for \textit{Cali},
and on 7 out of 8 datasets on \textit{SQR}.
While sharpness tends to increase with group batching, 
higher sharpness \textit{is} desirable if there is high noise 
in the true data distribution.
In Appendix~\ref{app:full_ablation_results}, we show that group batching also improves adversarial group calibration, suggesting that the underlying data distribution truly does have high noise.
This study indicates that deliberately taking batches during training that do not follow $\F_{\mathbf{X}}$ improves UQ performance.

% Improvements in adversarial group calibration (Figure~\ref{fig_in_app:}) 
% suggests that the true data distribution does have high noise, 
% which group batching helps to approach in the distributional predictions.

%%%%% \
%%%%% BEGIN: Dropping the new Ablation Table here
%%%%% /
\begin{figure*}[ht!]
\begin{center} 
\includegraphics[width=0.98\textwidth]{NeurIPS2021/figures/group_batching_ablation.pdf}
\caption{\textbf{Group Batching Ablation: Average Calibration and Sharpness.}
    The table shows mean ECE and sharpness (in parentheses) and their standard error with and without group batching. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined for \textit{Cali} and \textit{SQR} separately. All values have been multiplied by 100 for readability.} \label{fig:group_batch_ablation_main}
\end{center}
\vspace{-5mm}
\end{figure*}
% \vspace{-5mm}
%%%%% \
%%%%% END: Dropping the new Ablation Table here
%%%%% /


%%% END: ADD IN ABLATION STUDY




==> NeurIPS2021/introduction.tex <==
\vspace{-3mm}
\section{Introduction} 
\label{sec:introduction}
\vspace{-1mm}

Uncertainty quantification (UQ) in
%statistics and  machine learning refers to quantifying the confidence of a prediction.
machine learning typically refers to the task of quantifying the confidence of a given prediction.
This measure of certainty can be crucial in a variety of downstream applications, including
Bayesian optimization \citep{shahriari2015taking, mockus1978application},
model-based reinforcement learning \citep{yu2020mopo, malik2019calibrated, chua2018deep, garcia2012safe},
and in high-stakes predictions where mistakes incur large costs
\citep{rudin2019stop, wexler2017computer}.

While the common goal of UQ is to describe predictive distributions over outputs for given inputs,
the representation of the distributional prediction varies across methods.
For example, some methods assume a parametric distribution and return parameter estimates \citep{zhao2020individual, detlefsen2019reliable, lakshminarayanan2017simple}, 
while others return density function estimates, as is common in Bayesian methods 
\citep{maddox2019simple, liu2019accurate, hernandez2015probabilistic, blundell2015weight, koller2009probabilistic, rasmussen2003gaussian}. 
Alternatively, many methods represent predictive uncertainty with quantile estimates \citep{fasiolo2020fast, salem2020prediction, tagasovska2019single, pearce2018high, jeon2016quantile}.

Quantiles provide an attractive representation for uncertainty because they
% Quantiles allow an effective form of representation because they
can be used to model complex distributions without parametric assumptions,
are interpretable with units in the target output space,
allow for easy construction of prediction intervals, 
and can be used to efficiently sample from the predictive distribution via
inverse transform sampling \citep{hao2007quantile, koenker2001quantile}.
%
Learning the quantile for a single quantile level is a well studied problem
in quantile regression (QR) \citep{koenker2005quantile, koenker2001quantile},
which typically involves optimizing the so-called \textit{pinball loss}, 
a tilted transformation of the absolute value function. Given a target $y$, a prediction $\hat{y}$, and quantile level $\tau \in (0,1)$, the pinball loss $\rho_{\tau}$ is defined as
% \vspace{-.5mm}
\begin{align} \label{eq:pinball_loss}
    \rho_{\tau}(y, \hat{y}) = (\hat{y} - y)(\mathbb{I}\{y \leq \hat{y}\} - \tau).
\end{align} 
% \williex{descriptive sentence about pinball loss here?}
By training for all quantiles simultaneously, recent works have made concrete steps in incorporating QR methods 
to form competitive UQ methods which output the full predictive distribution \citep{rodrigues2020beyond, tagasovska2019single}.
% Recent works have made concrete steps in incorporating QR methods 
% to form competitive UQ methods which output the full predictive distribution
% by predicting all quantiles simultaneously \cite{rodrigues2020beyond}, 
% \cite{tagasovska2019single}. These methods focus on optimizing the pinball
% loss simultaneously for all quantiles.

% However, these methods require differentiable models because the loss function 
% is an aggregation of pinball losses at many (possibly random) quantile levels, 
% and gradient-based optimization becomes the only feasible method for this highly complex objective.
% In addition, these methods do not provide the flexibility to emphasize 
% different key quantities of interest (e.g. calibration, sharpness, centered interval coverage),
% and a practitioner may desire to trade-off between these quantities.
% Lastly, the pinball loss can be a poor proxy of the quality of the quantile estimates.

In this work, we highlight some limitations of the pinball loss and propose several methods to address these shortcomings.
Specifically, we explore the following:
% \begin{itemize}[topsep=0mm, leftmargin=5mm, parsep=0mm, itemsep=2mm, partopsep=1mm]
\begin{itemize}[topsep=0mm, leftmargin=5mm]
    \item \textbf{Model agnostic QR.} 
    Optimizing the pinball loss often restricts the choice of model family for which we can
    provide UQ.
    We propose an algorithm to learn all quantiles simultaneously by utilizing methods from 
    conditional density estimation. 
    This algorithm is agnostic to model class and can be applied to \textit{any} regression model.
    \item \textbf{Explicitly balancing calibration and sharpness.} 
    While the pinball loss, as a proper scoring rule, targets both calibration and sharpness, the balance between these two quantities is made implicitly, which may 
    result in a poor optimization objective.
    We propose a tunable loss function that targets calibration and sharpness separately,
    and allows the end-user to set an \textit{explicit} balance.
    % On its own, pinball loss does not directly target calibration and sharpness, 
    % even though these are important quantities for model evaluation.
    % We propose a tunable loss function that targets these quantities directly
    % and show empirically that the trained model can trade-off between calibration and sharpness.
    \item \textbf{Centered intervals.} 
    In practice, we often desire uncertainty predictions made with centered intervals, which
    are not targeted via the pinball loss.
    We propose an alternative loss function that is better suited for this goal.
    \item \textbf{Encouraging individual calibration.}
    Perfect quantile forecasts will satisfy \textit{individual} calibration (Eq.~\ref{eq:indv_cali}), 
    which is a much stricter condition than the
    % notion of calibration commonly used (i.e. \textit{average} calibration, Eq.~\ref{eq:avg_cali}).
    more-commonly used notion of \textit{average} calibration (Eq.~\ref{eq:avg_cali}).
    We introduce a training procedure that aims to improve quantile predictions
    beyond average calibration, and demonstrate its efficacy via \textit{adversarial group}
    calibration (Eq.~\ref{eq:adversarial-group-calibration}).
    % \williex{we need to cite or somehow describe/introduce adversarial group calibration}
\end{itemize}
We proceed by first describing methods of assessing the quality of predictive UQ, 
and the pitfalls of optimizing the pinball loss in Section~\ref{sec:prelim}.
% We proceed by first laying out relevant metrics used 
% to assess the quality of predictive UQ, 
% and discuss the pitfalls of optimizing the pinball loss (Section~\ref{sec:prelim}).
Drawing motivation from this, we then present our proposed methods in Section~\ref{sec:methods}.
In Section~\ref{sec:experiments}, we demonstrate our methods experimentally,
where we model predictive uncertainty on benchmark datasets, and 
on a high-dimensional, real-world uncertainty estimation task in the area of nuclear fusion.


==> NeurIPS2021/methods.tex <==
\vspace{-3mm}
\section{Methods}
\label{sec:methods}
\vspace{-3mm}
We propose four methods that aim to produce an improved quantile model.
% one algorithm, and two different loss functions. 
The first is a model-agnostic procedure that relies on conditional density estimation (Section~\ref{sec:maqr}).
To address settings where density estimation may be difficult, 
we then propose two loss functions to optimize with differentiable models: 
the combined calibration loss (Section~\ref{sec:cali}), which directly optimizes calibration and sharpness, and the interval score (Section~\ref{sec:int}), which is a proper scoring rule for centered intervals.
Finally, we propose a group batching method (Section~\ref{sec:group_batch}) that
can be applied to the batch optimization procedure for any loss function
(e.g. combined calibration loss, interval score, and even pinball loss) to induce better convergence towards adversarial group calibration.


% We propose a suite of methods aimed at learning an accurate quantile model. We first propose a model-agnostic algorithm which relies on conditional density estimation (Section~\ref{sec:maqr}). 
% To address the settings where density estimation may prove difficult, 
% we further propose two loss functions to optimize with differentiable models: 
% the scaled calibration loss (Section~\ref{sec:cali}), which directly optimizes calibration and sharpness, and the interval score (Section~\ref{sec:int}), which is a proper scoring rule for centered intervals.
% The group batching method (Section~\ref{sec:group_batch}) can be applied to 
% the optimization procedure for any loss function (e.g. scaled calibration loss, interval score, and even pinball loss) to induce better convergence towards adversarial group calibration.


\vspace{-3mm}
\subsection{Utilizing Conditional Density Estimation for Model Agnostic QR} \label{sec:maqr}
\vspace{-2mm}
One drawback of many existing quantile-based UQ methods is that 
their training procedure requires differentiable models. 
% is that the loss objective requires differentiable models. 
% For example, the SQR algorithm in \cite{tagasovska2019single} necessitates a differentiable model because gradient based methods are most suitable to optimize the loss \ysc{point here, it's also def possible to optimize the loss in another way, but it just doesn't make sense to not use gradient based optimization} 
In fact, most UQ methods require a specific class of models because of
their modeling structure or their loss objective (e.g. Gaussian processes \citep{rasmussen2003gaussian}, dropout \citep{gal2016dropout}, latent variable models \citep{koller2009probabilistic}, simultaneous pinball loss \citep{tagasovska2019single},
and NLL-based losses \citep{lakshminarayanan2017simple}).
% In fact, the issue of a method's dependence on a specific model class is not only existent in quantile-based methods, 
% but also in UQ methods in general. 
This model restriction can be especially unfavorable in practical settings. 
A domain expert with an established point prediction model and compute infrastructure may want to add UQ without much additional overhead.

% resorting to alternative ...
% without incurring more overhead. 
% In many applications, a domain expert may already have a point prediction model 
% with an established training procedure and compute infrastructure,
% and may want to additionally imbue their models with uncertainty without having to incur much overhead. 
To address these issues, we can consider the following model-agnostic procedure. 
Instead of optimizing a designated loss function, 
we can consider splitting the given problem into two parts: 
estimate conditional quantiles directly from data, 
then regress onto these estimates. 
The benefit of this method is that, granted we can estimate the
conditional quantiles accurately, 
we can use any regression model to predict these quantile estimates.
Further, this regression task directly targets the goal of producing
the true conditional quantiles (i.e. individual calibration).
% and the regression task of this method will directly target the end goal of converging to the conditional quantiles (individual calibration). 
This procedure, which we refer to as \textit{Model Agnostic QR} (MAQR), is outlined in Algorithm~\ref{alg:maqr_main}.
% \williex{Could put inner loop in Alg 1 as separate algorithm (i.e. a named subroutine) have have 2 side-by-side algorithms?}
% Using tools from nonparametric conditional density estimation, outline the this procedure in Algorithm~\ref{alg:mauq}, 
% which we refer to as Model Agnostic QR (MAQR). 
% \ianx{Not sure how I feel abaout ``one specific'' feels a bit weak.}
% \setlength{\textfloatsep}{2mm}% Remove \textfloatsep




% This algorithm is based on the \textit{key assumption} that 
MAQR is based on the key assumption that 
nearby points in $\mathcal{X}$ will have similar conditional distributions, 
i.e. if $x_j \approx x_k$ then $\F_{\bY|x_j} \approx \F_{\bY|x_k}$. 
Given this smoothness assumption,
% assumption on the smoothness of conditional distributions over $\cx$, 
% we can construct groups of neighboring points to estimate the conditional density, at each locality over $\cx$. 
we can group neighboring points to estimate the conditional density at each locality over $\cx$,
% This locality is determined by the hyperparameter $d_N$ (Algorithm~\ref{alg:CondQuantEst}, line 2).
with locality determined by the hyperparameter $d_N$ (Algorithm~\ref{alg:CondQuantEst}, line 2).
We then construct an empirical CDF with the group of neighboring points, 
and conditional quantile estimates are produced with this empirical CDF.
% \williex{From algo: Populate a set, $D_i$, of consistent estimators of the conditional quantiles of the residuals $x_i$ (Algorithm 2)}
% These conditional quantile estimates are collected into $D$, 
These estimates are collected into $D$, 
which is ultimately used as the training set for the quantile model $\hat{g}$.
% In practice, we perform all of these steps with the \textit{residuals} 
In practice, we perform these steps with \textit{residuals},
by first estimating a mean function $\hat{f}$ (Algorithm~\ref{alg:maqr_main}, line 1),
% and subtracting the mean estimates from all target points (line 2). 
which produces more accurate empirical CDFs.
% as the datapoints have sample mean close to 0.
This method takes advantage of the fact that accurate point
prediction models often already exist in many application settings.




\begin{figure*}[ttt!]
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
    \caption{\textsc{MAQR}} 
    \begin{algorithmic}[1] \label{alg:maqr_main}

        \STATE {\bfseries Input:} Train data $\{x_i, y_i\}_{i=1}^{N}$,
        trained regression model $\hat{f}(x)$
        
        \STATE Calculate residuals $\epsilon_i = y_i - \hat{f}(x_i)$, \hspace{1mm}$i\in[N]$
        
        \STATE Initialize $D \leftarrow \varnothing$
        
        \FOR{$i=1$ {\bfseries to} $N$}
            \STATE $D_i$ $\leftarrow$ \textsc{CondQuantilesEstimators}($D$, $i$) (Algorithm 2) 
            \STATE $D$: $D \leftarrow D \cup D_i$
        \ENDFOR 
    %%% BEGIN: ORIGINAL LINES 9~
    % \STATE Use $D$ to fit a regression model $\hat{g}$ \\
    % \hspace{10pt} $\hat{g}: (x_i, p_k) \mapsto \hat{q}_{i, p_k}$, \hspace{2mm}$k=1,\ldots,m$ 
    %%% END: ORIGINAL LINES 9~
    
        \STATE Use $D$ to fit a regression model $\hat{g}$ \\
        \hspace{10pt} $\hat{g}: (x, p) \mapsto \eps$

        \STATE {\bfseries Output:} $\hat{f} + \hat{g}$, \hspace{2mm}$k=1,\ldots,m$
    \end{algorithmic}
% \vspace{-5mm}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
    % \caption{Conditional Quantiles Estimators} 
    \caption{\textsc{CondQuantilesEstimators}} 
    \begin{algorithmic}[1] \label{alg:CondQuantEst}

        \STATE {\bfseries Input:} Dataset $\{x_i, \eps_i\}_{i=1}^{N}$, 
        point index $k\in[N]$
        
        \STATE $E_{k,{d_N}} \leftarrow \{\eps_i: \textrm{dist}(x_k, x_i) \leq d_N, i\in[N] \}$
    
        \STATE Construct an empirical CDF with $E_{k,d_N}$ to produce $\hF_{\mathbf{E}|x_k}: \epsilon \mapsto p\in[0,1]$
        
        %%% BEGIN: ORIGINAL LINES 7, 8
        % \STATE Select a set of quantile levels $\{p_k\}_{k=1}^{m}$, \hspace{1mm}$p_k \in [0,1]$
        % % \vspace{-3mm} % idk why this helps formatting...
        % \STATE $\hat{q}_{i, p_k} \leftarrow \inf \{\epsilon: p_k \leq \hF_{\mathbf{E}|x_i}(\epsilon)\}$, \hspace{2mm}$k=1,\ldots,m$
        % \STATE $D \leftarrow D \cup \{x_i, p_k, \hat{q}_{i, p_k}\}_{k=1}^{m}$
        %%% END: ORIGINAL LINES 7, 8
        \STATE Initialize $D \leftarrow \varnothing$
        \FOR{each $\eps_j$ in $E_{k, d_N}$}
            \STATE Query $\hF_{\mathbf{E}|x_k}$ at $\eps_j$ for 
            $\hat{p}_{k, j} = \hF_{\mathbf{E}|x_k}(\eps_j)$
            \STATE $D$: $D \leftarrow D \cup \{x_k, \hat{p}_{k, j}, \eps_j\}$
        \ENDFOR
    \STATE {\bfseries Output:} $D$
    
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-3mm}
\end{figure*}




%%%
Algorithm~\ref{alg:maqr_main} is a specific implementation of a
% Algorithm~\ref{alg:maqr} is a special case of a
more general model-agnostic algorithm, in which we directly estimate conditional
quantiles from the data with tools from conditional density estimation.
% and regress onto these estimates.
We note that using KDEs for conditional density estimation is a well studied problem with theoretical guarantees \citep{holmes2012fast, hyndman1996estimating, stute1986almost}.
In the case the distance in $\mathcal{X}$ is measured
using a uniform kernel with mild assumptions on the 
bandwidth, Algorithm~\ref{alg:maqr_main} falls under the guarantees stated by \citet{stute1986almost}.
% and the quantile dataset $D$ can be proven to be consistent. 
\vspace{2mm}
\\

\noindent
{\bf Theorem 1}~\citep{stute1986almost}.
{\it Assume $\cy \subset \mathbb{R}$, $\mathcal{X} \subset \mathbb{R}^n$, $\text{dist}(x_i, x_j) := |{x_i - x_j}|_\infty$, and that $\hF_{\mathbf{E}|x}$ is constructed using the procedure given in line 5 of Algorithm~\ref{alg:maqr_main} (i.e. $x_i = x$). Further assume that, as $N \rightarrow \infty$, $d_N \rightarrow 0$ and that $\sum_{N\geq1}\exp(- \rho N d_{N}^{n}) < \infty$, $\forall \rho > 0$. Then, as $N \rightarrow \infty$, for almost all $x\in \mathcal{X}$, 
$\sup_{\eps} [\hF_{\mathbf{E}|x}(\eps) - \F_{\mathbf{E}|x}(\eps)] \rightarrow 0$ with probability 1.
}


% \end{theorem}
% \vspace{-1mm}

% \textbf{Theorem 1}~\cite{stute1986almost}
% For fixed a fixed $d > 0$ and
% % Assume $d$ is any finite constant, 
% $\mathcal{X}\subset\mathbb{R}^{n}$,
% let $dist$ in line 5 of Algorithm~\ref{alg:maqr}
% % is measured using
% be
% a uniform kernel with bandwidth $a_N$, 
% i.e. $dist(x_i, x_j) = K(x_i, x_j) = 1$ if
% $\norm{x_i - x_j}_\infty \leq
% d \cdot a_N$.
% % \frac{d}{a_N}$.
% % $\sup [x_i - x_j] $ and $0$ otherwise, where the supremum is taken over 
% % the $n$ dimensions of $(x_i - x_j)$.
% Further assume that, as $N$ grows, $a_N \rightarrow 0$ and $\sum_{N\geq1}\exp(- \rho N a_{N}^{n}) < \infty$ $\forall \rho > 0$.
% % Further assume the bandwidth $a_N$ approaches 0 as dataset size $N \rightarrow \infty$ s.t. $\sum_{N\geq1}\exp(- \rho N a_{N}^{n}) < \infty$ for all $\rho > 0$. 
% Then, as $N \rightarrow \infty$, for almost all $x\in \mathcal{X}$, 
% $\sup_{\eps} [\hF_{\mathbf{E}|x}(\eps) - \F_{\mathbf{E}|x}(\eps)] \rightarrow 0$ with probability 1.

% In Appendix~\ref{app:maqr}, we state the general form of Algorithm~\ref{alg:maqr}, 
% and show how our quantile estimation procedure falls under the guarantees stated by \cite{stute1986almost}.
% As we will demonstrate in Section~\ref{sec:experiments}, basing predictions on these density estimates sidesteps the issues inherent to pinball loss.
This theorem states that in the limit of data,
for almost all $x \in \mathcal{X}$, 
the CDF estimate $\hF_{\mathbf{E}|x}$ will converge
uniformly to the true CDF $\F_{\mathbf{E}|x}$ with probability 1. 
The dataset, $D$, will therefore be populated
with 
% the true
good estimates of the
conditional quantile and quantile level pair for $x$.
In Appendix~\ref{app:maqr}, we state the general form of Algorithm~\ref{alg:maqr_main} and also demonstrate how the algorithm is model agnostic.
Through our experiments in Section~\ref{sec:experiments}, we will show empirically that utilizing these density estimates sidesteps the issues inherent to pinball loss and produces much higher quality quantile predictions.



% Lines 5 and 6 focus on estimating the conditional quantiles, which we achieve using conditional kernel density estimation (KDE). 
% KDE for conditional density estimation is a well studied problem with theoretical guarantees on consistency.
% Based on work by \ysc{~\cite{}}, we can show that our quantile dataset $D$ is consistent \williex{Is our dataset consistent? Can we be more accurate?}.
%
% We provide more details on the theoretical claims in Appendix~\ref{app:maqr}.

% \notes
% In the case that \ysc{review the conditions of that other proof}, we can show that this dataset is consistent. 



% Step 6 of Algorithm~\ref{alg:main} requires more formalism, which we describe here. 
% Methods to determine distances and similarities in various spaces is a vast field by itself \cite{hofmann2008kernel, singh2013k, xiang2008learning},
% but we will suggest some simple methods for implementation that we show work well in practice.
% The most naive method to determine the neighboring points is by thresholding the Euclidean distance $||x_i-x_j|| \leq d$. 
% One could also define a kernel $K:\mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}$ and threshold the similarity measure from the kernel outputs $K(x_i, x_j) \geq d$.
% % In fact, thresholding the Euclidean distance is equivalent to threholding the boxcar kernel to be positive.
% By using kernels, such as the squared exponential kernel $K(x_i, x_j) = \exp \left( -\frac{1}{2} \sum_{d=1}^{D} (x_{i,d} - x_{j,d})^{2}/l_{d}^{2} \right)$, 
% one can tune the kernel bandwidths $l_{d}$ to scale the distances in each dimension based on a user's beliefs about the noise distribution along different dimensions. 

% In step 6 of Algorithm~\ref{alg:main}, once the set of residuals of the
% neighboring points of $x_i$ has been determined, we estimate the the conditional
% distribution of the residuals with an empirial CDF estimate. Constructing CDF
% estimates is also a large subfield within statistics and machine learning
% \cite{sheather2004density, wasserman2006all}, and here we will suggest some practical
% methods. The simplest method is to construct an empirical CDF with uniform weights for
% each point. To emphasize the influence of points
% closer to $x_i$, a weighted empirical CDF can be constructed by assigning each point a weight
% inversely proportional to distance from $x_i$. Since empirical CDFs are discontinuous step
% functions, a smoothed estimate can be constructed with methods from kernel density estimation
% (KDE). If each point is assigned a Gaussian density, the CDF can be easily computed with
% the closed form Gaussian CDF formula. The density assigned to each point by the KDE
% can also be weighted according to its distance from $x_i$. 

% It is important to note that the quantile dataset created in Step ?? is crucial in deciding the performance of the resulting QR model because they are in fact estimated target points for the regression task. However, in the case that 
% \ysc{review the conditions of that other proof}, 
% we can show that this dataset is consistent. 
% \ianx{The way you have talked about it here sounds like these are our results. My preference on this is instead of writing it here, like this, before you even get into the details above I would write... ``Step 6 of the algorithm focuses on estimating quantiles which we achieve using KDE for conditional density estimation. KDE for conditional density estimation is a well studied problem and has been shown to achieve theoretical guarantees such as consistency CITE. Below we describe some tricks/details one can apply specifically for estimating quantiles.}

% \ysc{block on theoretical statement about consistency of the dataset}

% The remaining task of regressing onto this dataset can be done with standard empirical risk minimization of the MSE loss. 

% \\===========Notes Below===========\\
% One drawback of existing QR is that they require differentiable models. Further, there is a limit to how much you can verify that the true conditional quantiles have been achieved. 

% One method to tackle these together is to split the problem into 2: estimating conditional quantiles, and fitting a general regression model to ecapsulate all quantiles simultaneously. 
% This requires some assumptions: (...)
% The benefits of this approach are
% \begin{enumerate}
%     \item very applicable, preserve training infrastructure, preserve accuracy of a point prediction model
%     \item additional benefits from MAUQ submission
%     \item consistency guarantees
% \end{enumerate}
% 7\ianx{You can't say consistency guarantees for the overall method. One piece of it is consistent (maybe lol). To ground this method I would instead say. "We focus on splitting this problem into two subproblems. The first is conditional density estimation to create conditional quantiles. This problem has been well studied by CITE HERE and comes with theoretical guarantees. The second problem is regression bla bla bla.}
% \subsection{Selecting a calibration-sharpness trade-off with the penalized calibration loss} \label{sec:cali}


%%%%% \
%%%%% BEGIN: Original Figure 1: lambda tuning/adv group helps, 1 col
%%%%% /



\vspace{-2mm}
\subsection{Explicitly balancing calibration and sharpness with the combined calibration loss} \label{sec:cali}
\vspace{-1mm}
While MAQR can produce strong results, its performance can suffer in high-dimensional settings, 
where nonparametric conditional density estimation methods falter.
Neural networks (NNs) have shown good performance in high
dimensional settings, given their high capacity to approximate
complex functions and recent advances in fast gradient-based optimization.
% classification and regression problems, 
% as they can have high capacity to approximate complex functions, 
% and can be efficient to train with a differentiable loss function. 
We therefore propose a loss-based approach to estimating conditional quantiles for NNs and other differentiable models. 
% Hence, assuming NN models, we propose a loss based approach to estimating conditional quantiles. 

Drawing motivation from the \textit{arbitrary} balance between calibration and sharpness
that pinball loss \textit{implicitly} provides, 
we propose objectives separately for calibration and sharpness,
Then, we combine the two objectives into a single loss function that provides an 
explicit balance between calibration and sharpness which can be chosen by the end user.

We first consider calibration of a quantile prediction, $\hQ_p \in \mathcal{Y}$ 
for quantile level $p \in (0, 1)$.
Here, we omit conditioning on $x$ for clarity.
For this prediction to be average calibrated,
exactly a $p$ proportion of the true density 
% (\ysc{mass?}) of the true distribution
should lie below $\hQ_p$, i.e. $\ppobs = P(Y \leq \hQ_p) = p$.
While calibration (e.g. $|\ppobs-p|$) is a non-differentiable objective,
by inducing a truncated distribution based on the current level of calibration, 
we can construct the following calibration objective, which is minimized
if and only if the prediction is average calibrated:
%
% BTW, below is the SCALED cali loss version
% \begin{align*}
%     C(\hq_p, p) 
%     &= \mathbb{I}\{\hat{p}_p < p\} * (\hat{p}_p - p)^{2} * \E[Y-\hat{q}_p | Y > \hat{q}_p] * \Prob(Y > \hat{q}_p) \\ 
%     & \hspace{5pt} + \mathbb{I}\{\hat{p}_p > p\} * (\hat{p}_p - p)^{2} * \E[\hat{q}_p - Y | \hat{q}_p > Y] * \Prob(\hat{q}_p > Y)\\
%     & \hspace{70pt} \text{where} \hspace{5pt} \hp_p = \mathbb{P}(Y \leq \hq_p)
% \end{align*}
\begin{align}
    % \mathcal{C}(\hq_p, p) 
    % &= \mathbb{I}\{\hat{p}_p < p\} * \E[Y-\hat{q}_p | Y > \hat{q}_p] * \Prob(Y > \hat{q}_p) \\ 
    % & \hspace{5pt} + \mathbb{I}\{\hat{p}_p > p\} * \E[\hat{q}_p - Y | \hat{q}_p > Y] * \Prob(\hat{q}_p > Y)\\
    % & \hspace{70pt} \text{where} \hspace{5pt} \hp_p = \mathbb{P}(Y \leq \hq_p)
    %
    \mathcal{C}(\hQ_p, p) 
    &= \mathbb{I}\{\hat{p}_p < p\} * \E[Y-\hQ_p | Y > \hQ_p] * P(Y > \hQ_p) \\ 
    & \hspace{5pt} + \mathbb{I}\{\hat{p}_p > p\} * \E[\hQ_p - Y | \hQ_p > Y] * P(\hQ_p > Y), 
    \text{where} \hspace{5pt} \hp_p = P(Y \leq \hQ_p). \nonumber
\end{align}
The empirical calibration objective, $\mathcal{C}(D, \hQ_p, p)$ is defined in Equation~\ref{eq:emp_cal_obj} (Appendix~\ref{app:definition}).
% \williex{An empirical estimate (sample-estimate?) of this loss, $\mathcal{C}(D, \hQ_p, p)$, is defined in XYZ??}
% We can plug in empirical estimators for a finite sample estimate, $C(D, \hQ, p)$:
% \begin{align*}
%     \begin{split}
%         \mathcal{C}(D, \hQ, p) 
%         & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         % &\mathcal{C}(D, \hQ, p) = \\
%         % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
%     \end{split}
% \end{align*}

\textit{\textbf{Note 1:} Intuition of the calibration objective.}
For any given $p$, consider the case when the quantile estimate $\hQ_p$ is 
below the true $p\sth$ quantile $\mathbb{Q}_p$. 
Since $\hQ_p < \mathbb{Q}_p \iff \hat{p}_p < p$, this implies that 
% either too
% little density mass lies below $\hQ_p$, or 
too much density mass lies above $\hQ_p$.
In this case, $\mathcal{C}(\hQ_p, p)$ reduces to $\E[Y-\hQ_p | Y > \hQ_p] * P(Y > \hQ_p)$. $\hQ_p$ is pulled higher with the expectation of the truncated distribution that
places $\hQ_p$ at the lower bound of the support. 
In the opposite case, when $\hQ_p > \mathbb{Q}_p$, $\hQ_p$ is pulled lower 
by the same logic.
% by the truncated distribution whose support is upper bounded by $\hQ_p$.

\textit{\textbf{Note 2:} Is the proposed calibration objective a proper scoring rule?}
Strictly speaking, the calibration objective is a non-decomposable function,
hence deviates from the standard convention of proper scoring
rules \cite{gneiting2007strictly}, which
can be ``decomposed'' into scores for individual examples $(x_i, y_i)$.
This simply arises from the fact that
measuring average calibration (i.e. $\pobs$) is non-decomposable.
Proper scoring rules are defined such that an optimum of the \textit{expected score} (or \textit{risk}, if we consider the score as a \textit{loss function}) occur at the true distribution quantity.
While an example level \textit{loss} or \textit{score} does
not exist due to non-decomposability, 
% we can still show the (expectation-level) risk
we can still show the (expectation-level) score
(i.e. $\mathcal{C}(\hQ_p, p)$) is minimized by the true
distribution and hence enjoys the optimum property of proper scoring rules.
% Nevertheless, the proposed objective still enjoys the optimum property of proper scoring rules, i.e. the true quantile $q_p$ minimizes $C(\hq, p)$.
% the proposed objective still enjoys the optimum property of proper scoring rules, i.e. the true quantile $q_p$ minimizes $C(\hq, p)$.

{\bf Proposition 2}. \label{prop:cal_obj}
{\it For any quantile level $p \in (0, 1)$, 
the true quantile function $\mathbb{Q}_p$ minimizes the calibration objective, 
$\mathcal{C}(\hat{\mathbb{Q}}_p, p)$.
Further, on a finite dataset $D$, the empirical calibration objective, $\mathcal{C}(D, \hat{\mathbb{Q}}_p, p)$,
is minimized by an average calibrated solution on $D$, i.e. when $\pobs(D, p) = p$.}

% $\mathcal{C}(\hq_p, p)$ is minimized at a calibrated solution, when $\hp_p = p$. 
% Further, the empirical calibration objective, $\mathcal{C}(D, \hq_p, p)$ is minimized at
% an empirically calibrated solution, i.e. when $\pobs = p$.}

\textbf{Proof:} The proof is given in Appendix~\ref{app:prop_2}.

% \noindent \textbf{Proof} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN: original proposition 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {\bf Proposition 2} \label{prop:cal_loss}
% {\it Consider a finite dataset $D = \{(x_i, y_i)\}_{i = 1}^N$ and an estimate $\hQ$ such that $\widehat{\text{ECE}}(D, \hQ) = 0$. Then $\hQ$ is a minimum of both scaled and non-scaled calibration loss for all $p \in \{n/N\}_{n=1}^{N-1}$ on $D$.}
% \end{proposition}
% \noindent \textbf{Proof} The definition of $\widehat{ECE}$ implies the two, non-negative losses are 0 for $p \in \{n/N\}_{n=1}^{N-1}$.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END: original proposition 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \underline{Note 3: Gradients for a miscalibrated prediction $\hq_p$.}
\textit{\textbf{Note 3:} Non-zero gradients for miscalibrated predictions $\hQ_p$.}
We can further show that for a miscalibrated quantile prediction, 
% the gradients of $\mathcal{C}$ always push the prediction towards a calibrated one. 
the gradients of $\mathcal{C}$ are always non-zero. 
When $\hp_p < p$,
% $\frac{\partial \mathcal{C}(\hQ_p, p)}{\partial \hQ_p}$
$\partial \mathcal{C}(\hQ_p, p)/\partial \hQ_p$ $=$ $-P(Y > \hQ_p) < 0$.
Thus increasing $\hQ_p$
% ($\iff$ increasing $\hp_p$)
decreases the objective $\mathcal{C}$.
Similarly, when $\hp_p > p$,
% $\frac{\partial \mathcal{C}(\hQ_p, p)}{\partial \hQ_p}$
$\partial \mathcal{C}(\hQ_p, p) / \partial \hQ_p$
$=$ $P(Y < \hQ_p) > 0$, and an analogous argument follows (proof in Appendix~\ref{app:note_3}).





% \textbf{Proposition 2} 
% \textit{Consider a dataset $D = \{(x_i, y_i)\}_{i = 1}^N$ with unique
% $x_i \in \mathcal{X}$, model class $F$ with an infinite capacity, and the scaled calibration loss $\mathcal{C}_{\text{scaled}}(D, \hQ, \tau)$ as defined in Eq.~\ref{eq:scaled_cali_loss}.
% For any level $\tau \in [0, 1]$, the minimizer
% $\textrm{argmin}_{f \in F}\left[\sum_{i=1}^{N}\mathcal{C}_{\text{scaled}}(D, f, \tau))\right]$ is always perfectly average calibrated 
% on $D$ with ECE=0.}

% \ianx{Should add a note saying something like ``Unlike the pinball loss, even when considering a model class with infinite capacity one of the minimizers is the quantile." Basically need to be more clear why this has some advantage over pinball loss.}
% It is trivial to show that a minimizer of the calibration loss, for any given $p$, is a prediction such that $\hp = p$.
% We prove Proposition 2 in Appendix ~\ref{app:proposition}.
% \begin{proof}
% Since both losses are non-negative, the proposition follows trivially from the fact $\hp^{\text{obs}}_{avg} = p$ for all $p$ when using
% This follows trivially from the fact that both losses are non-negative, equal 0 when $\hp^{\text{obs}}_{avg} = p$, and that $\hQ$ has 
% \end{proof}

As discussed in Section~\ref{sec:metrics}, average calibration by itself is not 
a sufficient condition for meaningful UQ, 
hence we also
% need to consider the \textit{sharpness} of the quantile model.
% Sharpness prefers tighter distributional predictions over flatter distributions,
desire \textit{sharp} quantile models, with more-concentrated (less flat) distributions.
% and we can induce this property in quantile predictions by 
We can induce this property in quantile predictions by 
predicting the $(1-p)$\textsuperscript{th} quantile $\hQ_{1-p}(x_i)$ alongside each
prediction $\hQ_p(x_i)$ and penalizing the width between the quantile predictions:
\begin{align}
    \mathcal{P}(\hQ_p, p) = \E \left[ \left| \hQ_p - \hQ_{1-p} \right| \right].
\end{align}
The empirical sharpness objective, $\mathcal{P}(D, \hQ_p, p)$ is defined in Equation~\ref{eq:emp_sharp_obj} (Appendix~\ref{app:definition}).
% \williex{An empirical estimate (sample-estimate?) of this loss, $\mathcal{P}(D, \hQ_p, p)$, is defined in XYZ??}
It is important to note that the true underlying distribution will not have $0$ sharpness if there is significant noise, and sharpness should be optimized subject to calibration.
Therefore, we should only penalize sharpness when the data suggests our quantiles are too dispersed, 
i.e. when $\left| p^{\text{obs}}_{avg}(p) - p^{\text{obs}}_{avg}(1-p) \right|$, the \textit{observed coverage} between the pair of quantiles $\hQ_p(x_i)$ and $\hQ_{1-p}(x_i)$,
is greater than $ \left| 2p-1 \right|$, the \textit{expected coverage}.

Combining the calibration and sharpness terms, we have the \textbf{combined calibration loss}
\begin{align}
    \label{eq:combined-calibration-loss}
    % \mathcal{L}(D, \hQ, p) = (1-\lambda)\mathcal{C}_{\text{scaled}}(D, \hQ, p) + \lambda \mathcal{P}(D, \hQ, p).
    \mathcal{L}(D, \hQ_p, p) = (1-\lambda)\mathcal{C}(D, \hQ_p, p) + \lambda \mathcal{P}(D, \hQ_p, p).
\end{align} 
The hyperparameter $\lambda \in [0, 1]$ sets the explicit balance between calibration and sharpness. 
Note that setting $\lambda = 0$ may not always be desirable, since optimizing $\mathcal{C}(D, \hQ_p, p)$ alone may converge to quantiles of the marginal distribution, $\marginal$.
Further, in certain downstream applications that utilize UQ,
a sharper prediction, even at the cost of worse calibration, 
may result in higher utility, and $\lambda$ can be tuned according to the utility function of the application.
In our experiments, we tune $\lambda$ by cross-validating with adversarial group calibration as it is the strictest notion of 
calibration that can be estimated with a finite dataset.


% \begin{align}
%     \mathbb{E}_{p\sim U[0, 1]}  \mathcal{L}(D, \hQ, p).
% \end{align}



% \begin{align}
%     \mathbb{E}_{p\sim U[0, 1]}  \mathcal{L}(D, \hQ, p)
% \end{align}

% \notes
% The major drawback of model agnostic introduced above is that the trained model is only as good as the conditional quantile estimates, which deteriorates in high dimensions. 

% NN's are very high capacity models that have proven to be effective in high dimensions (all the good stuff here aboud NN's in high-dim, like feature extraction, smoothing in high dimensions, efficient training, ...).
% Also, with differentiable models, we have more flexible with engineering a new loss function. 

% Go back to calibration metric, which is estimated this way. It is non-differentiable, but we can try to optimize this way....
% Oftentimes, calibration is not enough, so we can add a sharpness penalty.


\vspace{-1mm}
\subsection{Encouraging calibration of centered intervals with the interval score}
\label{sec:int}
\vspace{-2mm}
The combined calibration loss (Eq.~\ref{eq:combined-calibration-loss}) optimizes
average calibration, which targets observed probabilities below a quantile.
In many applications, however, we may desire a centered prediction interval (PI)
which requires a pair of quantile predictions. A centered $95\%$ PI, for example,
is a pair of quantile predictions at quantile levels $0.025$ and $0.975$.
Hence, for the average calibration of the $p\sth$ \textit{centered interval}, we want
$\left[\pobs(0.5+\frac{p}{2}) - \pobs(0.5-\frac{p}{2})\right]$
(the PI observed probability, a.k.a. prediction interval coverage probability (PICP)
\citep{tagasovska2019single, kabir2018neural, pearce2018high}) to be equal to the expected probability $p$.
While we can modify the objective in Eq.~\ref{eq:combined-calibration-loss} to adhere to this altered goal, 
here we propose simultaneously optimizing the \textbf{interval score} (or Winkler score) \citep{gneiting2007strictly, winkler1972decision} 
for all expected probabilities $p\in (0, 1)$, 
and bring to light a proper scoring rule that has largely been neglected for the purpose of \textit{learning quantiles}. 
While some previous works utilize the interval score to \textit{evaluate} interval predictions~\citep{bracher2021evaluating, bowman2020uncertainty, askanazi2018comparison, maciejowska2016probabilistic},
to the best of our knowledge, no previous work has focused on simultaneously optimizing it and
% utilized a simultaneous optimization and
shown a thorough experimental evaluation as we provide in Section~\ref{sec:experiments}.

For a point $(x, y)$, if we denote a $(1-\alpha)$ centered PI as $\hat{l}, \hat{u}$,
i.e. $\hat{l} = \hQ_{\frac{\alpha}{2}}(x)$ and $\hat{u} = \hQ_{1-\frac{\alpha}{2}}(x)$,
% For a $(1-\alpha)$ centered PI, with $\hat{l}$ and $\hat{u}$ the 
% predictive quantiles at levels $\frac{\alpha}{2}$ and $1-\frac{\alpha}{2}$,  \ysc{fix the notation, then note}
% respectively (i.e. $\hat{l} = \hQ(\cdot, \frac{\alpha}{2}), \hat{u} = \hQ(\cdot, 1-\frac{\alpha}{2})$), 
% given a target datapoint $y$, the interval score is defined to be
the interval score is defined as 
$S_{\alpha}(\hat{l}, \hat{u}; y) = 
(\hat{u} - \hat{l}) + \frac{2}{\alpha}(\hat{l} - y)\mathbb{I}\{y < \hat{l}\} + \frac{2}{\alpha}(y - \hat{u})\mathbb{I}\{y > \hat{u}\}$.
% \begin{align*}
%     S_{\alpha}(\hat{l}, \hat{u}; y) = 
%     (\hat{u} - \hat{l}) + \frac{2}{\alpha}(\hat{l} - y)\mathbb{I}\{y < \hat{l}\} + \frac{2}{\alpha}(y - \hat{u})\mathbb{I}\{y > \hat{u}\}.
% \end{align*}
We show in Appendix~\ref{app:int_score} that the minimum of the expectation of the interval score is attained at the
true conditional quantiles,
$\hat{l} = \Q_{\frac{\alpha}{2}}(\cdot)$,
$\hat{u} = \Q_{1 - \frac{\alpha}{2}}(\cdot)$.
% \ysc{I want to say here that there's a close relationship between "usual" calibration and interval calibration and a perfect quantile model will be calibrated both ways, but if we must incur error in quantile predictions, optimizing this score will output quantile estimates with better interval calibration.}
We train our quantile model for all centered intervals (and hence all quantile levels)
simultaneously by setting our loss objective as
$\mathbb{E}_{\alpha \sim U(0,1)} S_{\alpha}$.

% %%%%% \
% %%%%% BEGIN: Original 5 UCI first five, 2 rows
% %%%%% /
% \begin{figure*}[t]
%     \centering
%     % \includegraphics[width=0.6\textwidth]{figs/fusion_gc.png}
%     % \includegraphics[width=1.0\textwidth]{AISTATS2021/figs/fusion_gc.png}
%     %
%     % \includegraphics[width=8.5cm, height=4cm]{AISTATS2021/figs/uci_cal_sharp.pdf}
%     % \includegraphics[width=8.5cm, height=4cm]{AISTATS2021/figs/uci_group_cali.pdf}
%     %
%     \hspace{3mm}
%     \includegraphics[width=\textwidth]{AISTATS2021/figs/uci_first_five.pdf}
%     % \includegraphics[width=0.97\textwidth]{AISTATS2021/figs/fusion_cal_sharp_onerow.pdf}
%     % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali_onerow.pdf}
%     \caption{UCI Experiments. \textbf{Top row:} Average calibration and sharpness. \textbf{Bottom row:} Adversarial group calibration (group size refers to the proportion of dataset size). Full set of results (additional datasets) are in Appendix~\ref{app:all_uci_results}.}
%     % \williex{fusion plots a placeholder for now, will replace with UCI plots} 
%     % \williex{TODO: write that all plots are in the appendix}}
%     \label{fig:uci_plots}
%     % \vspace{-4mm}
% \end{figure*}
% %%%%% \
% %%%%% END: Original 5 UCI first five, 2 rows
% %%%%% /


% %%%%% \
% %%%%% BEGIN: Original UCI three horizontal tables, scoring rules
% %%%%% /
% \begin{figure*}[t] 
% % \begin{table}[ht!]
% % \begin{adjustbox}{width=8.5cm, height=1.5cm}
% % \begin{adjustbox}{width=1.1\columnwidth,center}
% \setlength\doublerulesep{3pt}
% \begin{center} 
% \begin{tabular}{ |c|  |c|c|c|c|c|c| } 
%  \hline
%          & \textit{SQR}                         & \textit{\textbf{MAQR}}             \\ \Xhline{3\arrayrulewidth} %\hhline{|=||=|=|}
% Boston   & $ 0.088 (0.008) $           & $\mathbf{ 0.063 (0.016)}$ \\ \hline
% Concrete & $ 0.085 (0.006) $           & $\mathbf{ 0.059 (0.008)}$ \\ \hline
% Energy   & $ 0.014 (0.000) $           & $\mathbf{ 0.010 (0.001)}$ \\ \hline
% Kin8nm   & $ 0.078 (0.001) $           & $\mathbf{ 0.070 (0.001)}$ \\ \hline
% Naval    & $ 0.070 (0.001) $           & $\mathbf{ 0.004 (0.000)}$ \\ \hline
% % power    & $\mathbf{ 0.057 (0.001) }$  & $ 0.058 (0.001) $         \\ \hline
% % wine     & $ 0.205 (0.008) $           & $\mathbf{ 0.191 (0.003)}$ \\ \hline
% % yacht    & $ 0.012 (0.002) $           & $\mathbf{ 0.007 (0.001)}$ \\ \hline
% \end{tabular}
% \hspace{0.5pt}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%  \textit{\textbf{Interval}}  & \textit{\textbf{MAQR}}              \\ \Xhline{3\arrayrulewidth} %\hhline{|=|=|}
%  $ 1.010 (0.118)$   & $ \mathbf{0.864 (0.287)}$  \\ \hline
%  $ 0.943 (0.053)$   & $ \mathbf{0.672 (0.118)}$  \\ \hline
%  $ 0.182 (0.026)$   & $ \mathbf{0.101 (0.006)}$  \\ \hline
%  $ 0.776 (0.017)$   & $ \mathbf{0.691 (0.015)}$  \\ \hline
%  $ 0.620 (0.114)$   & $ \mathbf{0.044 (0.001)}$  \\ \hline
% %  $ 0.620 (0.010)$   & $ \mathbf{0.592 (0.009)}$  \\ \hline
% %  $ 2.197 (0.045)$   & $ \mathbf{2.052 (0.052)}$  \\ \hline
% %  $ 0.190 (0.021)$   & $ \mathbf{0.086 (0.016)}$  \\ \hline
% \end{tabular}
% \hspace{0.5pt}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%  \textit{\textbf{Interval}}  & \textit{\textbf{MAQR}}     \\ \Xhline{3\arrayrulewidth} %\hhline{|=|=|}
%  $ \mathbf{0.079 (0.015)}$   & $ 0.092 (0.041)$  \\ \hline
%  $ 0.061 (0.008)$   & $ \mathbf{0.059 (0.020)}$  \\ \hline
%  $ 0.060 (0.010)$   & $ \mathbf{0.052 (0.018)}$  \\ \hline
%  $ 0.048 (0.006)$   & $ \mathbf{0.019 (0.008)}$  \\ \hline
%  $ 0.043 (0.014)$   & $ \mathbf{0.012 (0.002)}$  \\ \hline
% %  $ 0.023 (0.003)$   & $ \mathbf{0.010 (0.002)}$  \\ \hline
% %  $ 0.079 (0.014)$   & $ \mathbf{0.045 (0.005)}$  \\ \hline
% %  $ 0.121 (0.005)$   & $ \mathbf{0.085 (0.024)}$  \\ \hline
% \end{tabular}
% \caption{UCI Experiments. \textbf{Left}: Check  score. \textbf{Middle}: Interval score. 
% \textbf{Right}: Interval Calibration. Each table shows the top two methods only, in
% terms of average performance. Full set of results (additional methods and datsets) are
% in Appendix~\ref{app:all_uci_results}. The highest scoring results for each
% dataset are shown in \textbf{bold}.
% \label{fig:uci_numbers}}
% \end{center}
% \vspace{-4mm}
% \end{figure*}
% %%%%% \
% %%%%% END: Original UCI three horizontal tables, scoring rules
% %%%%% /

%
%
% \caption{\textbf{UCI Check Score} Caption}
% &
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%           & \textbf{Int}       & \textbf{MAQR}              \\ \hline
%  concrete  & $ 0.943 (0.053)$   & $ \mathbf{0.672 (0.118})$  \\ \hline
%  power     & $ 0.620 (0.010)$   & $ \mathbf{0.592 (0.009)}$  \\ \hline
%  wine      & $ 2.197 (0.045)$   & $ \mathbf{2.052 (0.052)}$  \\ \hline
%  yacht     & $ 0.190 (0.021)$   & $ \mathbf{0.086 (0.016)}$  \\ \hline
%  naval     & $ 0.620 (0.114)$   & $ \mathbf{0.044 (0.001)}$  \\ \hline
%  energy    & $ 0.182 (0.026)$   & $ \mathbf{0.101 (0.006)}$  \\ \hline
%  boston    & $ 1.010 (0.118)$   & $ \mathbf{0.864 (0.287)}$  \\ \hline
%  kin8nm    & $ 0.776 (0.017)$   & $ \mathbf{0.691 (0.015)}$  \\ \hline
% \end{tabular}
% \caption{\textbf{UCI Interval Score} Caption}
% \end{center}

% \end{adjustbox}
% \end{table}






\vspace{-2mm}
\subsection{Inducing adversarial group calibration with group batching}
\label{sec:group_batch}
\vspace{-2mm}
% The calibration loss from~\ref{sec:cali} and the interval score from~\ref{sec:int} optimize for the \textit{average} calibration of quantiles and centered intervals, respectively. 
% We emphasize again that this is only a relaxed condition of the main goal of individual calibration.
% \ianx{Don't think this paragraph is needed.}

The calibration loss (Section~\ref{sec:cali}) and the interval score (Section~\ref{sec:int}) optimize for the 
\textit{average} calibration of quantiles and centered intervals, respectively.
To get closer to individual calibration, %than average calibration, 
one condition we can additionally require is \textit{adversarial group calibration}.
Since adversarial group calibration requires average calibration over any subset of non-zero measure over the domain, 
this is not fully observable with finite datasets $D$ for all subset sizes.
However, for any subset in $D$ with enough datapoints, we can still estimate average calibration over the subset.
Hence, we can apply our optimization objectives onto appropriately large subsets 
to induce adversarial group calibration.
%, which is a much stronger condition than average calibration. 

In practice, this involves constructing subsets within the domain and 
taking gradient steps based on the loss over each subset.
In naive implementations of stochastic gradient descent,
a random batch is drawn \textit{uniformly} from the 
training dataset $D$, and a gradient step is taken according to the loss over
this batch. This is also the case in \textit{SQR} \citep{tagasovska2019single}.
The uniform draw of the batch will tend to preserve $\F_{\bX}$ (the marginal distribution over $\cx$),
hence optimizing average calibration over this batch will only induce average calibration of the model.

Instead, deliberately grouping the datapoints based on input features, and then batching
and taking gradient steps based on these groups, induces 
% By deliberately grouping the datapoints based on input features and batching
% based on these groups, 
% the distribution of each batch will not follow $\F_{\bx}$,
% and taking optimization steps w.r.t. this group will induce
better adversarial group calibration.
We find in our experiments that adversarial group calibration improves significantly
with simple implementations of group batching,
and in Section~\ref{sec:ablation}, we show through an ablation study 
that group batching can improve average calibration and
adversarial group calibration of \textit{SQR} as well.
In Appendix~\ref{app:group_batching} we provide details on how we implemented group batching in our ablation study and the experiments.
% \ianx{I don't like pointing out that it may be viewed as a minor technical trick because if people didn't think that before they definitely will after}
% While this may seem like only a minor technical ``trick'' during  the training procedure, we find in our experiments that adversarial group calibration improves significantly with group batching. 

% \notes
% \williex{
% What is a basic structure (i.e. sections and subsections) for how we
% could present the set of material/methods that we have?}

% \ianx{Based on what I have above I would suggest:
% \begin{itemize}
%     \item Section 1: Intro
%     \item Section 2: Preliminaries
%     \item Section 3: Flexibility in loss functions (each subsection could be method Young has explored + experiment showing it works)
%     \item Section 4: Flexibility in model class (describe then show experiment)
%     \item Section 5: Conclude
% \end{itemize}}



==> NeurIPS2021/original_blocks.tex <==
\newpage
\section{Original Blocks}

\ysc{BEGIN: Original Block 1 -----}\\
One alternative family of evaluation metrics is \textbf{proper scoring rules} \citep{gneiting2007strictly}. 
Proper scoring rules are summary statistics of overall performance of a
distributional prediction and consider both calibration and sharpness
jointly \citep{gneiting2007probabilistic}. 
% A (possibly non-unique) optimum of a proper scoring rule is attained when the prediction matches the true underlying distribution. 
For example, negative log-likelihood (NLL) is a proper scoring rule
that is commonly used with density predictions \citep{detlefsen2019reliable, pearce2018uncertainty, lakshminarayanan2017simple}. 
For quantile predictions, one proper score is the \textbf{check score}, \textit{which is identical to the pinball loss}.
This gives more ground to optimizing the pinball loss, which is the traditional method in quantile regression \citep{koenker1978regression},
and recent quantile-based UQ methods focus on optimizing the pinball loss \citep{rodrigues2020beyond, tagasovska2019single, cannon2018non, xu2017composite}.
% most work in within quantile regression have focused around the pinball loss, e.g. by applying various models and optimization methods (\cite{takeuchi2006nonparametric, li2007quantile}), utilizing a smoothed approximation of the pinball loss (\cite{fasiolo2020fast}) or taking a Bayesian approach with a pinball-based likelihood (\cite{yu2001bayesian}). \ysc{more citations here}.

% In expectation, the minimizer of the pinball loss converges to the true conditional quantiles
% \williex{convergence with respect to what? amount of data?}. 

The minimum of the expectation of the pinball loss is attained at the true conditional quantile. 
However, for finite datasets,
we can show that minimizing the pinball loss does not necessarily
lead to average calibration on the dataset.
\\\\
\noindent
{\bf Proposition 1}  \label{prop:pinball}
% \begin{proposition}
{\it Consider a dataset $D = \{(x_i, y_i)\}_{i = 1}^N$ with unique
$x_i \in \mathcal{X}$, model class $F$ with an infinite capacity, and pinball
loss $\rho_{\tau}(y, \hat{y})$ as defined in Eq.~\ref{eq:pinball_loss}.
For any level $\tau \in [0, 1]$, the minimizer
$\textrm{argmin}_{f \in F}\left[\sum_{i=1}^{N}\rho_{\tau}(y_i, f(x_i, \tau))\right]$
achieves 0 pinball loss.
% However, a QR model composed of these minimizers is miscalibrated with an ECE of 0.5.
However, these minimizers yield a miscalibrated uncertainty prediction with $\widehat{\text{ECE}}(D, \hQ)=0.5$.}\\

% \end{proposition}
%%%
% Then $\forall \tau \in (0, 1)$, the minimizer $f^{*} = \textrm{argmin}_{f \in F}\left[\sum_{i=1}^{N}\rho_{\tau}(y_i, f(x_i))\right]$
% achieves 0 pinball loss (lowest score possible) while simultaneously
% achieving \williex{an ECE of $\frac{1}{2}$}.
%
% worst average calibration possible \williex{MAKE SPECIFIC} on D.}


% This further imples that for any $f$ which achieves average calibration on $D$, there exists $f' \in F$ which has a lower pinball loss but arbitrarily worse average calibration.
% This further implies that for any $f$ that achieves average calibration on $D$,
% we can always find another $f' \in F$ such that the pinball loss of $f'$ evaluated on $D$ is lower than that of $f$, 
% but the average calibration of $f'$ is arbitrarily worse.
% Proofs of Proposition 1. is in Appendix~\ref{app:}.

The proof of Proposition 1 is in Appendix~\ref{app:proposition}.
At first glance, this proposition may not be surprising since overfitting is 
an inherent problem that one needs to account for in most machine learning problems. 
The key difference here is the magnitude of the problem that overfitting causes.
When $F$ has infinite capacity, 
a perfectly calibrated solution will never be a 
minimizer of the pinball loss.
By achieving perfect pinball loss, one is left with an inaccurate UQ model that is
highly miscalibrated, \textit{even on the training dataset}.


The intuition is that the pinball loss implicitly decides a balance betweeen calibration and sharpness
\textit{based on the expressivity of the model class}.
With high-capacity models such as neural networks (NNs),
the pinball loss unequally favors sharpness over calibration.
When using the pinball loss in practice, the correct balance
between calibration and sharpness depends on 
either choosing the correct class of models with an appropriate level of capacity, or 
applying the correct amount of constraint or regularization on a chosen model class, 
both of which may be difficult to specify with arbitrary function approximators
(e.g. NNs).
% We demonstrate this behavior empirically in Appendix~\ref{app:pinball_pitfall},
% where we optimize the pinball loss with varying model sizes.
% These pitfalls motivate our loss function in Section~\ref{sec:cali}, 
% which allows \textit{the user to directly select a trade-off} between calibration and sharpness
% within a given class of models.
These pitfalls motivate our loss function in Section~\ref{sec:cali}, 
which directly targets calibration and sharpness, and explicitly selects a trade-off between the two.

\ysc{END: Original Block 1 -----}\\

\ysc{BEGIN: Original Block 2 -----}\\
We draw motivation from the conflict between finite sample average calibration and pinball loss from Section~\ref{sec:metrics}.
Suppose that our explicit goal is to optimize average calibration, which corresponds to optimizing Equation~\ref{eq:finite_avg_cali}.
% Suppose we explicitly set our goal to optimizing the average calibration of our quantile model, 
% which corresponds to optimizing Equation~\ref{eq:avg_cali}.
% We first inspect average calibration (an observable \ianx{Still not entirely observable. I would say a more relaxed quantity and more feasible to estimate.} and relaxed objective from individual calibration) for a given quantile level $p$. With a finite set of $N$ points $\{(x_i, y_i)\}_{i=1}^{N}$, this is estimated according to Equation~\ref{}.
% \begin{align}
%     \mid p - \hat{p} \mid, \text{  where  } \hat{p} = \frac{\sum_{i=1}^{N} \mathbb{I}\{y_i \leq \hQ(x_i, p)\}}{T}
% \end{align}
% Suppose we relax our goal from achieving individual calibration to achieving average calibration, and we try to optimize Equation~\ref{}.
For any given $p$, Equation~\ref{eq:finite_avg_cali} is non-differentiable because of the indicator function (an estimate of the true CDF).
However, one workaround to this is the following:
% However, one optimization method can be the following: 
% \vspace{-3mm}
\begin{enumerate}
    \item Observe the current coverage $\hp^{\text{obs}}_{avg}$.
    % \vspace{-2mm}
    \item If $\hp^{\text{obs}}_{avg} < p$, raise $\hQ$ to increase coverage below $\hQ$; \\
    if $\hp^{\text{obs}}_{avg} > p$, lower $\hQ$ to reduce coverage below $\hQ$.
    % \vspace{-2mm}
    \item Repeat steps 1, 2 until $\hp^{\text{obs}}_{avg}$ has converged to $p$.
\end{enumerate}

These steps prescribe whether to lower or raise $\hQ$, and guide the observed probability, $\hp^{\text{obs}}_{avg}$, towards $p$, thus improving average calibration.
%
% This provides a signal to lower or raise $\hQ$ given the observed discrepancy
% between $\hp^{\text{obs}}_{avg}$ and $p$, which [optimizes for] [improves] average
% calibration for the given $p$.
%
% By providing an adequate signal in step 2 
% to lower or raise $\hQ$ appropriately for the observed discrepancy between $\hp^{\text{obs}}_{avg}$ and $p$, 
% $\hp^{\text{obs}}_{avg}$ should be able to converge to $p$, achieving average calibration for the given $p$. \williex{UPDATE THIS.}
%
Given a finite dataset $D = \{(x_i, y_i)\}_{i=1}^{N}$, a quantile model $\hQ$, and a
probability $p$, we propose the \textbf{calibration loss}
%$\mathcal{C}(D, \hQ, p)$ as, 
%$\mathcal{C}(D, \hQ, p)$ as follows in Equation~\ref{eq:cali_loss}.  
% Our calibration loss is designed to optimize \textit{average calibration}.
% \vspace{-2mm}
\begin{align*}
    \begin{split}
        \mathcal{C}(D, \hQ, p) & =
        \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        % &\mathcal{C}(D, \hQ, p) = \\
        % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        & +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
    \end{split}
\end{align*}

% \begin{align} \label{eq:cali_loss}
%     \begin{split}
%         &\mathcal{L}(\{y_i, \hQ(x_i, p)\}_{i=1}^{N}) = \\
%         & \mathbb{I}\{\hp^{\text{obs}}_{avg} \leq p\}\frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         & +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\}\frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right]   
%     \end{split}
% \end{align}
% \vspace{-2mm}
In words, the calibration loss is calculated as follows: if coverage is lower than desired ($\hp^{\text{obs}}_{avg} < p$), then penalize the predictions that are lower than the datapoints by the magnitude of their residuals $(y_i - \hQ(x_i, p))$, and vice versa.
% We can also scale the loss by the magnitude of
We additionally scale the loss by the magnitude of
miscalibration $|\hp^{\text{obs}}_{avg} - p|$, which we call \textbf{scaled calibration loss} 
\begin{align}
    \label{eq:scaled_cali_loss}
    \mathcal{C}_{\text{scaled}}(D, \hQ, p) = |\hp^{\text{obs}}_{avg} - p|
    \hspace{1mm} \mathcal{C}(D, \hQ, p)
\end{align}
% Unlike the pinball loss, even when considering a model with infinite capacity, 
% a minimizer of the calibration loss occurs when the prediction is average calibrated $\hp^{\text{obs}}_{avg} = p$.
% Unlike the pinball loss, scaled calibration loss is minimized at perfect average calibration, even when considering a model with infinite capacity.
Unlike pinball loss, minimizing calibration loss does not necessarily mean a high capacity model will be miscalibrated.
\\

% \begin{proposition} \label{prop:cal_loss}

\noindent
{\bf Proposition 2} \label{prop:cal_loss}
{\it Consider a finite dataset $D = \{(x_i, y_i)\}_{i = 1}^N$ and an estimate $\hQ$ such that $\widehat{\text{ECE}}(D, \hQ) = 0$. Then $\hQ$ is a minimum of both scaled and non-scaled calibration loss for all $p \in \{n/N\}_{n=1}^{N-1}$ on $D$.}
% \end{proposition}
\\

% \begin{proof}
\noindent \textbf{Proof} The definition of $\widehat{ECE}$ implies the two, non-negative losses are 0 for $p \in \{n/N\}_{n=1}^{N-1}$.\\
% \end{proof}

Proposition 2 shows that any model that is calibrated on the dataset will be a minimizer of the two calibration losses at the observable values of $p$. Importantly, there exists no quantile function that achieves a lower loss than one calibrated on the data, unlike pinball loss (Proposition 1).

As discussed in Section~\ref{sec:metrics}, average calibration by itself is not 
a sufficient condition for meaningful UQ, 
hence we also need to consider the \textit{sharpness} of the quantile model.

One instantiation of a sharpness penalty can be to predict the
$(1-p)$\textsuperscript{th} quantile $\hQ(x_i, 1-p)$ alongside each
prediction $\hQ(x_i, p)$ and penalize the width between these two outputs,
using

\begin{align*}
    &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} 
        \begin{cases} 
            \hQ(x_i, 1-p) - \hQ(x_i, p) \hspace{5pt} (p \leq 0.5)\\
            \hQ(x_i, p) - \hQ(x_i, 1-p) \hspace{5pt} (p > 0.5)
        \end{cases}
\end{align*}

In early training stages, the model output $\hQ(x,p)$ may not be increasing in $p$, hence we penalize only when it is positive.
In addition, it is important to note that the true underlying distribution will not have $0$ sharpness if there is significant noise. 
Therefore, we should only penalize sharpness when the data suggests our quantiles are too dispersed, 
i.e. when $\mid p^{\text{obs}}_{avg}(1-p) - p^{\text{obs}}_{avg}(p) \mid$, the \textit{observed coverage} between the pair of quantiles $\hQ(x_i, 1-p)$ and $\hQ(x_i, p)$,
is greater than $\mid2p-1\mid$, the \textit{expected coverage}.

Combining the calibration and sharpness terms, we have the full loss, the \textbf{combined calibration loss}
\begin{align*}
    \mathcal{L}(D, \hQ, p) = (1-\lambda)\mathcal{C}_{\text{scaled}}(D, \hQ, p) + \lambda \mathcal{P}(D, \hQ, p).
\end{align*}

By scaling the hyperparameter $\lambda \in [0, 1]$, we can trade-off between the calibration and sharpness objectives.
This is especially useful when working with real-world data.
Because it is impossible to verify the exact correctness of the calibration-sharpness pair of a prediction, 
a practitioner may want to choose to emphasize one aspect over the other, depending on their application \citep{malik2019calibrated, murphy1973new}.
% We show in Figure~\ref{fig:demo} how scaling $\lambda$ allows predictions to traverse the calibration-sharpness Pareto front.
We show in Figure~\ref{fig:demo} how different choices of 
$\lambda$ trades off between calibration-sharpness in 
the predictions.
Since we learn a quantile model $\hQ$ that outputs the conditional quantile estimates for all probabilities, following \citep{tagasovska2019single}, our training objective is: 
$\mathbb{E}_{p\sim U[0, 1]}  \mathcal{L}(D, \hQ, p)$.

\ysc{END: Original Block 2-----}\\


\ysc{BEGIN: Original Block 3 (algorithm) -----}\\
\setlength{\textfloatsep}{2mm}% Remove \textfloatsep
\begin{algorithm}[h!]
  \caption{Model Agnostic Quantile Regression} 
\begin{algorithmic}[1]

    \STATE {\bfseries Input:} Train data $\{x_i, y_i\}_{i=1}^{N}$,

    trained regression model $\hat{f}(x)$

    \STATE Calculate the residuals $\epsilon_i = y_i - \hat{f}(x_i)$, \hspace{2mm}$i\in[N]$
    
    \STATE Initialize $D \leftarrow \varnothing$
    
    \FOR{$i=1$ {\bfseries to} $N$}
    \STATE $E_{i,{d_N}} \leftarrow \{\eps_j: \textrm{dist}(x_i, x_j) \leq d_N, 1 \leq j \leq N \}$

    \STATE Construct an empirical CDF with $E_{i,d_N}$ to produce $\hF_{\mathbf{E}|x_i}: \epsilon \mapsto p\in[0,1]$
    
    %%% BEGIN: ORIGINAL LINES 7, 8
    % \STATE Select a set of quantile levels $\{p_k\}_{k=1}^{m}$, \hspace{1mm}$p_k \in [0,1]$
    % % \vspace{-3mm} % idk why this helps formatting...
    % \STATE $\hat{q}_{i, p_k} \leftarrow \inf \{\epsilon: p_k \leq \hF_{\mathbf{E}|x_i}(\epsilon)\}$, \hspace{2mm}$k=1,\ldots,m$
    % \STATE $D \leftarrow D \cup \{x_i, p_k, \hat{q}_{i, p_k}\}_{k=1}^{m}$
    %%% END: ORIGINAL LINES 7, 8
    
    \FOR{each $\eps_j$ in $E_{i, d_N}$}
    \STATE Query $\hF_{\mathbf{E}|x_i}$ at $\eps_j$ for 
    $\hat{p}_{i, j} = \hF_{\mathbf{E}|x_i}(\eps_j)$
    \STATE $D$: $D \leftarrow D \cup \{x_i, \hat{p}_{i, j}, \eps_j\}$
    \ENDFOR
    
    

    \ENDFOR 
    %%% BEGIN: ORIGINAL LINES 9~
    % \STATE Use $D$ to fit a regression model $\hat{g}$ \\
    % \hspace{10pt} $\hat{g}: (x_i, p_k) \mapsto \hat{q}_{i, p_k}$, \hspace{2mm}$k=1,\ldots,m$ 
    %%% END: ORIGINAL LINES 9~
    
    \STATE Use $D$ to fit a regression model $\hat{g}$ \\
    \hspace{10pt} $\hat{g}: (x, p) \mapsto \eps$

  \STATE {\bfseries Output:} $\hat{f} + \hat{g}$, \hspace{2mm}$k=1,\ldots,m$
\end{algorithmic}
% \vspace{-5mm}
\end{algorithm}

\ysc{END: Original Block 3 (algorithm) -----}\\


\ysc{BEGIN: Original Figure 1: lambda tuning/adv group helps, 1 col}
%%%%% \
%%%%% BEGIN: Original Figure 1: lambda tuning/adv group helps, 1 col
%%%%% /

\begin{figure}[t] 

    % \begin{minipage}[c]{0.4\textwidth} 
    %     \vspace{5mm}
    %     \includegraphics[width=\textwidth]{AISTATS2021/figs/pareto.pdf}
    % \end{minipage}
    % \begin{minipage}[c]{0.48\textwidth}
    %     \caption{By tuning the sharpness penalty coefficient in the combined calibration loss, 
    %     we can trade-off calibration and sharpness in the prediction (example on Wine dataset).}
    %     \label{fig:demo}
    % \end{minipage}\hfill

    \begin{minipage}[c]{0.4\textwidth} 
        \caption{By tuning the sharpness penalty coefficient in the combined calibration loss, 
        we can trade-off calibration and sharpness in the prediction (example on Wine dataset).}
        \label{fig:demo}
    \end{minipage}
    \hspace{5mm}
    \begin{minipage}[c]{0.48\textwidth}
        \vspace{5mm}
        \includegraphics[width=\textwidth]{NeurIPS2021/figures/pareto.pdf}
    \end{minipage}\hfill

    
    % \includegraphics[width=0.235\textwidth]{AISTATS2021/figs/pareto.pdf}
    % \includegraphics[width=0.235\textwidth]{AISTATS2021/figs/qr_group_batch.pdf}
    % \caption{\textbf{Left:} By tuning the sharpness penalty coefficient in the combined calibration loss, 
    % we can trade-off calibration and sharpness in the prediction (example on Wine dataset).
    % \textbf{Right:} Increasing the frequency of group batching epochs (with uniform batching in other epochs) during training also helps SQR (which optimizes pinball loss) achieve better adversarial group calibration (example on Concrete dataset).} 
    % \vspace{-2mm}
    
\end{figure} 
%%%%% \
%%%%% END: Original Figure 1: lambda tuning/adv group helps, 1 col
%%%%% /

\ysc{END: Original Figure 1: lambda tuning/adv group helps, 1 col}


\ysc{BEGIN: Original empirical risk of calibration loss, sharpness penalty}

We can plug in empirical estimators for a finite sample estimate, $C(D, \hQ, p)$:
\begin{align*}
    \begin{split}
        \mathcal{C}(D, \hQ, p) 
        & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        % &\mathcal{C}(D, \hQ, p) = \\
        % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
    \end{split}
\end{align*}

\begin{align*}
    &\mathcal{P}(\hq_p, p) = \E \left[|\hq_p - \hq_{1-p}|\right] \\ 
    &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} |\hQ(x_i, 1-p) - \hQ(x_i, p)| 
\end{align*}

\ysc{END: Original empirical risk of calibration loss, sharpness penalty}


\ysc{BEGIN: Original Section 3.3}
The calibration loss from Section~\ref{sec:cali} optimizes the average calibration of each quantile, i.e. the correct intended coverage below a quantile estimate.
This can be considered optimizing for the correct coverage of a non-centered, $p$ prediction interval (PI) between the levels $[0, p]$. 
In many applications, however, it is much more common to utilize a PI that is
centered at the mean or median prediction For an intended coverage of $p$, this
would correspond to quantile estimates for the levels $(0.5 - \frac{p}{2})$ and
$(0.5 + \frac{p}{2})$.

% We can easily modify the calibration loss to always predict a pair of centered intervals and widen or reduce the intervals based on the coverage within the interval and the intended coverage.
% \ianx{This motivation here is a little unclear to me. Are we saying this intervals score is actually going to win out? Seems like you're just listing possible methods right now.}
To this end, we propose optimizing the \textbf{interval score}, 
which is a proper scoring rule for centered interval predictions \citep{gneiting2007strictly}. 
For a given point $(x, y)$, denote a $(1-\alpha)$ centered PI as $\hat{l}, \hat{u}$, i.e. $\hat{l} = \hQ(x, \frac{\alpha}{2})$ and $\hat{u} = \hQ(x, 1-\frac{\alpha}{2})$. We omit conditioning on $x$ for clarity.
% For a $(1-\alpha)$ centered PI, with $\hat{l}$ and $\hat{u}$ the 
% predictive quantiles at levels $\frac{\alpha}{2}$ and $1-\frac{\alpha}{2}$,  \ysc{fix the notation, then note}
% respectively (i.e. $\hat{l} = \hQ(\cdot, \frac{\alpha}{2}), \hat{u} = \hQ(\cdot, 1-\frac{\alpha}{2})$), 
% given a target datapoint $y$, the interval score is defined to be
Then the interval score is defined as:
\begin{align*}
    S_{\alpha}(\hat{l}, \hat{u}; y) = 
    (\hat{u} - \hat{l}) + \frac{2}{\alpha}(\hat{l} - y)\mathbb{I}\{y < \hat{l}\} + \frac{2}{\alpha}(y - \hat{u})\mathbb{I}\{y > \hat{u}\}.
\end{align*}
This score presents an intuitive interpretation of the desirable components from a centered interval: the first term penalizes the width (sharpness), and the second and third terms penalize calibration (i.e. correct coverage of PI) by penalizing the prediction when the datapoint falls outside the PI. 
For a higher intended coverage (i.e. lower $\alpha$), the coverage penalty is scaled higher (scaled by $\frac{2}{\alpha}$). 

We can show that the minimum of the expectation of the interval score is attained at the
true quantiles,
$\hat{l} = \Q(\cdot, \frac{\alpha}{2})$, $\hat{u} = \Q(\cdot, 1 - \frac{\alpha}{2})$ (Appendix~\ref{app:int_score}), which motivates using empirical risk minimization to optimize the interval score.
% \ysc{I want to say here that there's a close relationship between "usual" calibration and interval calibration and a perfect quantile model will be calibrated both ways, but if we must incur error in quantile predictions, optimizing this score will output quantile estimates with better interval calibration.}
We train our quantile model for all centered intervals (and hence quantile levels)
simultaneously by setting our loss objective as
$\mathbb{E}_{\alpha \sim U[0,1]} S_{\alpha}$.

\ysc{END: Original Section 3.3}

\ysc{BEGIN: Original Group Batching Ablation Table}

%%%%% \
%%%%% BEGIN: Dropping the new Ablation Table here
%%%%% /
\begin{figure*}[h!]
\begin{center} 
\begin{tabular}{ |c||c|c || c|c|c|}
 \hline & \multicolumn{2}{c||}{\textit{Cali}} & \multicolumn{2}{c|}{\textit{SQR}} \\
 \hline
          & \textit{Random Batch}                 & \textit{Group Batch}            & \textit{Random Batch}      & \textit{Group Batch}   \\\hline
Boston & $9.7\pm1.3(\underline{10.2}\pm0.7)$ & $\textbf{8.5}\pm1.5(10.9\pm0.6)$ & $10.9\pm1.0(\underline{8.8}\pm1.1)$ & $\textbf{9.8}\pm1.2(9.5\pm0.9)$ \\ \hline
Concrete & $6.6\pm0.9(17.6\pm2.3)$ & $\textbf{5.6}\pm0.8(\underline{17.3}\pm1.5)$ & $9.8\pm1.3(\underline{7.0}\pm0.6)$ & $\textbf{7.1}\pm0.9(8.5\pm0.6)$ \\ \hline
Energy & $9.2\pm0.3(\underline{2.8}\pm0.1)$ & $\textbf{5.8}\pm0.4(3.6\pm0.3)$ & $10.2\pm0.8(\underline{1.8}\pm0.1)$ & $\textbf{6.9}\pm1.1(2.4\pm0.2)$ \\ \hline
Kin8nm & $\textbf{3.4}\pm0.3(\underline{13.7}\pm0.4)$ & $3.5\pm0.3(\underline{13.7}\pm0.7)$ & $4.7\pm0.3(\underline{11.1}\pm0.1)$ & $\textbf{3.9}\pm0.4(11.3\pm0.2)$ \\ \hline
Wine & $4.4\pm0.5(\underline{25.6}\pm0.8)$ & $\textbf{4.2}\pm0.4(26.0\pm0.8)$ & $4.5\pm0.4(29.7\pm0.5)$ & $\textbf{4.0}\pm0.4(\underline{28.5}\pm0.8)$ \\ \hline
Yacht & $11.1\pm1.8(\underline{1.8}\pm0.1)$ & $\textbf{8.3}\pm0.6(2.0\pm0.4)$ & $9.0\pm0.9(\underline{0.9}\pm0.1)$ & $\textbf{8.9}\pm0.9(2.3\pm0.2)$ \\ \hline
Power & $\textbf{1.7}\pm0.2(14.2\pm0.3)$ & $2.0\pm0.1(\underline{13.1}\pm0.1)$ & $\textbf{2.5}\pm0.3(14.0\pm0.5)$ & $2.9\pm0.5(\underline{13.6}\pm0.8)$ \\ \hline
Naval & $2.8\pm0.2(\underline{12.1}\pm3.1)$ & $\textbf{2.4}\pm0.3(50.6\pm8.6)$ & $8.6\pm1.6(\underline{3.6}\pm0.1)$ & $\textbf{5.3}\pm0.8(6.0\pm0.5)$ \\ \hline
\end{tabular}
\caption{\textbf{Group Batching Ablation: Average Calibration and Sharpness.}
    The table shows mean ECE and sharpness (in parentheses) and their standard error with and without group batching. The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined for \textit{Cali} and \textit{SQR} separately. All values have been multiplied by 100 for readability.} \label{fig:group_batch_ablation}
\end{center}
\vspace{-5mm}
\end{figure*}
% \vspace{-5mm}
%%%%% \
%%%%% END: Dropping the new Ablation Table here
%%%%% /


\ysc{END: Original Group Batching Ablation Table}

\ysc{BEGIN: Original Full Cal-Sharp Table UCI and Fusion}
%%%%% \
%%%%% BEGIN: Dropping the new Cal-Sharp UCI, Fusion table here
%%%%% /
\begin{figure*}[ht!]
    \centering
    
    \includegraphics[width=\textwidth]{ICML2021/figs/full_calibration_table.pdf}
    
    \caption{\textbf{Average Calibration and Sharpness.}
    The table shows mean average calibration (measured by ECE) and sharpness in parentheses, along with $\pm 1$ standard error.
    % Because of limited space, only the first four fusion datasets are shown here, but the full table can be found in Appendix~\ref{app:all_experiments}.
    The best mean ECE for each dataset has been bolded and the best mean sharpness has been underlined. All values have been multiplied by 100 for readability.}
    \label{fig:ece_sharp_table}
    \vspace{-1mm}
\end{figure*}
%%%%% \
%%%%% END: Dropping the new Cal-Sharp UCI, Fusion table here
%%%%% /
\ysc{END: Original Full Cal-Sharp Table UCI and Fusion}


\ysc{BEGIN: Original ICML Full AdvGroupCal Figures (3 UCI, 1 Fusion)}
%%%%% \
%%%%% BEGIN: Dropping the new AdvGroupCal figure here
%%%%% /
\begin{figure*}[ht!]
    \centering

    %%% Include 3 UCI, 2 fusion
    % \includegraphics[width=0.59\textwidth]{ICML2021/figs/uci_group_cali_first_3.pdf}
    % \includegraphics[width=0.39\textwidth]{ICML2021/figs/fusion_group_cali_first_2.pdf}
    
    %% Include 4 UCI, 1 fusion 
    % \includegraphics[width=0.79\textwidth]{ICML2021/figs/uci_group_cali_first_4.pdf}
    % \includegraphics[width=0.197\textwidth]{ICML2021/figs/fusion_group_cali_first_1.pdf}
    
    %% Include 3 UCI, 1 fusion 
    \includegraphics[width=0.74\textwidth]{ICML2021/figs/uci_group_cali_first_3.pdf}
    \includegraphics[width=0.248\textwidth]{ICML2021/figs/fusion_group_cali_first_1.pdf}
    
    
    % %% Include 5 UCI, 5 fusion --> 2 rows
    % \includegraphics[width=\textwidth]{ICML2021/figs/uci_group_cali_first_5.pdf}
    % \includegraphics[width=\textwidth]{ICML2021/figs/fusion_group_cali_first_5.pdf}
    
    % %% Include 4 UCI, 4 fusion  --> 2 rows
    % \includegraphics[width=\textwidth]{ICML2021/figs/uci_group_cali_first_4.pdf}
    % \includegraphics[width=\textwidth]{ICML2021/figs/fusion_group_cali_first_4.pdf}
    
    \caption{\textbf{Adversarial Group Calibration}. Here, group size refers to proportion of test dataset size. \textbf{Left three:} First three UCI datasets, in alphabetical order. \textbf{Right one:} First fusion dataset, in alphabetical order. Full set of results
    (additional signals) are in Appendix~\ref{app:all_experiments}.}
    \label{fig:adv_group_cal_partial}
    \vspace{-5mm}
\end{figure*}
%%%%% \
%%%%% END: Dropping the new AdvGroupCal figure here
%%%%% /
\ysc{END: Original ICML Full AdvGroupCal Figures (3 UCI, 1 Fusion)}


\ysc{BEGIN: First 5 Fusion: cal-sharp scatter, AdvGroupCal }
\begin{figure*}[ht!]
    \centering
    % \includegraphics[width=8.5cm, height=3.5cm]{AISTATS2021/figs/fusion_cal_sharp.pdf}
    % \includegraphics[width=8.5cm, height=3.5cm]{AISTATS2021/figs/fusion_group_cali.pdf}
    % \caption{\textbf{Fusion Calibration-Sharpness} Caption}
    %
    \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_first_five.pdf}
    %
    % \hspace{3mm}
    % \includegraphics[width=0.97\textwidth]{AISTATS2021/figs/fusion_cal_sharp_onerow.pdf}
    % \includegraphics[width=\textwidth]{AISTATS2021/figs/fusion_group_cali_onerow.pdf}
    \caption{Nuclear Fusion Experiments. \textbf{Top row:} Average calibration and sharpness. \textbf{Bottom row:} Adversarial group calibration (group size refers to proportion of dataset size). Full set of results
    (additional signals) are in Appendix~\ref{app:all_fusion_results}.}
    \label{fig:fusion_plots}
    \vspace{-1mm}
\end{figure*}
\ysc{END: First 5 Fusion: cal-sharp scatter, AdvGroupCal }


\ysc{BEGIN: Original Experiments Analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The top tables in Figures~\ref{fig:uci_table_figure} and~\ref{fig:fusion_table_figure}
display average calibration-sharpness for all 8 UCI datasets and all 10 fusion datasets.
\textit{MAQR} produces the best average calibrated models on 7 of the 8 UCI datasets.
Excluding \textit{MAQR},
\textit{Interval} and \textit{Cali} achieve competitive calibration on 
7 out of 8 UCI datasets
and 9 out of 10 fusion datasets.
Notably, \textit{SQR} tends to produce the sharpest predictions across all 
datasets, with worse calibration. 
This is not surprising following Proposition 1.
Lastly, we also note that \textit{Interval} and \textit{Cali}  
tend to be more robust and consistent compared to \textit{SQR} and \textit{mPAIC}, 
which incur major failures in some cases (e.g. \textit{mPAIC} in Kin8nm, \textit{SQR} in Naval).

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%



Figure~\ref{fig:ece_sharp_table} displays average calibration-sharpness
for all 8 UCI datasets and all 10 fusion datasets.
\textit{MAQR} seems to be best at producing calibrated models, winning out on 7 of the 8 UCI datasets.
Excluding \textit{MAQR},
\textit{Interval} and \textit{Cali} achieve competitive calibration on 
7 out of 8 UCI datasets
and 9 out of 10 fusion datasets.
% and 3 out of 4 fusion datasets (and 9 out of 10 on the full set of 10 fusion datasets (Appendix~\ref{app:all_fusion_results})).
Notably, \textit{SQR} tends to produce the sharpest predictions across all 
datasets. 
This is not surprising following Proposition 1. 
In particular, it is likely that \textit{SQR} is erroneously too sharp 
given its high calibration error. Lastly, we also note that \textit{Interval} and \textit{Cali}  
tend to be more robust and consistent compared to \textit{SQR} and \textit{mPAIC}, 
which incur major failures in some cases (e.g. \textit{mPAIC} in Kin8nm, \textit{SQR} in Naval).

We observe that \textit{mPAIC} performs the poorest on the fusion datasets, with least calibrated and sharp predictions.
It is generally known that plasma dynamics display complex stochasticity
\cite{fu2020machine, kowal2020kelvin}, and hence we suspect \textit{mPAIC}'s
performance degrades significantly because 
it assumes a Gaussian output and is trained according to the Gaussian likelihood.

Adversarial group calibration shown in 
Figure~\ref{fig:adv_group_cal_partial} indicates
that \textit{MAQR} and \textit{Interval} also 
tend to achieve lowest calibration error across 
\textit{any} random group of \textit{any} size with more than one point. Adversarial group calibration also suggests that \textit{SQR}'s predictions have not approached the true conditional quantiles well, 
and that it has significantly traded off calibration for sharpness 
when compared to \textit{Cali} and \textit{Interval}.

Only a subset of the plots and metrics are shown in the main paper because of space restrictions. Readers are encouraged to see the full results in Appendix~\ref{app:all_experiments}, but we will summarize the main findings here. 

The check score, interval score, and centered interval calibration
in the tables in Appendix~\ref{app:all_experiments} also rank 
\textit{MAQR}'s prediction as best.
This is surprising since \textit{SQR} and \textit{Interval} train NNs of the same capacity to explicitly minimize the check and interval scores, respectively.
This indicates the distribution predicted by \textit{MAQR} is fundamentally different 
as it utilizes direct estimates of the conditional distribution,
while the other methods all optimize a specific loss function.

The centered interval calibration metric (Appendix~\ref{app:all_fusion_results}) also indicates that \textit{Cali} and \textit{Interval} both
produce competitive centered intervals (9 out of 10 fusion datasets), 
suggesting that both methods have better estimated the conditional quantiles than the alternative algorithms, in general.  
\ysc{END: Original Experiments Analysis}

\ysc{BEGIN: Original $\lambda$ block}
By scaling the hyperparameter $\lambda \in [0, 1]$, we can trade-off between the calibration and sharpness objectives.
This is especially useful when working with real-world data.
Because it is impossible to verify the exact correctness of the calibration-sharpness pair of a prediction, 
a practitioner may want to choose to emphasize one aspect over the other, depending on their application \citep{malik2019calibrated, murphy1973new}.
We show in Figure~\ref{fig:demo} how different choices of 
$\lambda$ trades off between calibration-sharpness in 
the predictions.
Since we learn a quantile model $\hQ$ that outputs the conditional quantile estimates for all probabilities, following \citep{tagasovska2019single}, our training objective is: 
$\mathbb{E}_{p\sim U[0, 1]}  \mathcal{L}(D, \hQ_p, p)$.
\ysc{END: Original $\lambda$ block}

==> NeurIPS2021/prelim.tex <==
\vspace{-2mm}
\section{Preliminaries and Background}
\label{sec:prelim}
\vspace{-2mm}


We first lay out the notation, terminology, and class of models considered in this paper.
Then we provide an overview of evaluation metrics in UQ and demonstrate 
how the pinball loss may be inadequate both as an evaluation metric 
and as an optimization objective.

\vspace{-1mm}
\subsection{Notation} \label{sec:notation}
\vspace{-2mm}
Bold upper case letters \textbf{X, Y} denote random variables, 
lower case letters $x, y$, denote their values, 
and calligraphic upper case letters $\mathcal{X, Y}$ denote sets of possible values. 
We use $x\in \mathcal{X}$ to denote the input feature vector and $y \in \mathcal{Y}$ to denote the corresponding target.
Additionally, we consider the regression setting where $\cy \subset \mathbb{R}$ and $\mathcal{X} \subset \mathbb{R}^n$.
We use $\mathbb{F}_{\textbf{X}}, \mathbb{F}_{\textbf{Y}\mid x}, \mathbb{F}_{\textbf{Y}}$ 
to denote the true cumulative distribution of the subscript random variable. 
For any $x \in \mathcal{X}$, we assume there exists a true conditional distribution 
$\mathbb{F}_{\textbf{Y}\mid x}$ over $\cy$, 
and we assume $\Q_p(x)$ denotes the true $p$\textsuperscript{th} quantile of this distribution, 
% \ianx{before you were calling $p$ probability but now it is $p^{th}$ quantile. Does that track?}
i.e. $\mathbb{F}_{\textbf{Y}\mid x}(\Q_p(x)) = p$.
Any estimates of the true functions $\mathbb{F}, \Q_p$ will be denoted with a hat, 
$\hat{\mathbb{F}}, \hQ_p$.
We will specifically refer to any family of estimates for $\Q_p$, with $p \in (0, 1)$,
as a ``quantile model'', denoted
$\hQ: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$.
% as a ``quantile model''.
Unless otherwise noted, we will always consider the \textit{conditional} problem of
estimating quantities in the target space $\cy$, conditioned on a value $x \in \cx$.

% \subsection{Terms}
% By ``quantile regression", we will refer to the problem of regressing 
% onto all conditional quantiles, for all probabilities $p \in (0,1)$ simultaneously.
% We will refer to the output of this regression as a ``quantile model": 
% $\hat{\mathbb{Q}}: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$, 
% which takes as input a point $x$ and a probability value $p$, 
% and outputs an estimate of the $p$\textsuperscript{th} conditional quantile given $x$, 
% $\hat{\mathbb{Q}}(x, p) \in \mathcal{Y}$.
% \ianx{Might be good to add a quick note here about how traditionally quantile models will only learn a single $p$, so you have to learn multiple models to get full coverage of $p$s or use SQR}

% \subsection{Metrics for Assessing UQ Quality}
\vspace{-1mm}
\subsection{Assessing the Quality of Predictive UQ}
\label{sec:metrics}
\vspace{-2mm}

% While the common goal of UQ is to describe the conditional distribution of outputs $y$ given inputs $x$, 
% the metrics used to evaluate the quality of distributional predictions is varied across different methods.
% Methods that make assumptions about the data distribution often output a density estimate,
% and if the true data distribution is available, one can measure various numerical distribution distances 
% (L1 distance, KL divergence), as done in \cite{NIPS2019_9097}.
% This is usually not feasible in real world situations, and such distance values are not interpretably meaningful to practitioners

% More commonly, many works have instead turned to proper scoring rules (\cite{gneiting2007strictly}), 
% such as the negative log-likelihood (\cite{lakshminarayanan2017simple, NIPS2019_8862, blundell2015weight}).
% However, proper scoring rules may have pitfalls as an evaluation metric. 

% Suppose we have a trained quantile model. How will we verify it's performance? 
% Further, how will we do so with a finite set of test points?

% Following the definition of quantiles, we can see that a quantile's correctness is
% directly connected to ``calibration".



% Here, another benefit of quantile predictions arises, because by definition, 
% a quantile estimate's correctness is directly connected to calibration. 

% \cite{zhao2020individual} provides an excellent overview on the notion of calibration,
% which we reformulate here in the form of quantile predictions. 


While various metrics have been
% used in literature
proposed to assess the quality of UQ, there has been a great deal of recent focus on the notions of \textit{calibration} and \textit{sharpness}
\citep{fasiolo2020fast, cui2020calibrated, zhao2020individual, tran2020methods, song2019distribution, kuleshov2018accurate, guo2017calibration, gneiting2007probabilistic}.
We introduce calibration here, but for a more thorough treatment, see
\citet{zhao2020individual}.
Broadly speaking, calibration in the regression setting
requires that the probability of observing the target random variable below a predicted $p$\textsuperscript{th} quantile is equal to the \textit{expected probability} $p$, for all $p \in (0, 1)$.
% We refer to the former quantity as the \textit{observed probability} and denote it $p^{\text{obs}}(p)$, for an \textit{expected probability}, $p$.
% We will often drop the reliance on $p$ and simply write $p^{\text{obs}}$ when it is clear from context.
We refer to the former quantity as the \textit{observed probability} and denote it 
$p^{\text{obs}}(p)$, for an expected probability $p$, which we will write as
$p^{\text{obs}}$ when it is clear from context.
Calibration requires $p^{\text{obs}}(p) = p$, $\forall p \in (0,1)$.
From this generic statement, we can describe different notions of calibration
based on how $p^{\text{obs}}$ is defined.


% If the model achieves perfect quantile prediction which is exactly the true conditional quantile,
% If a model outputs the true conditional quantiles,
% $\hQ(x, p) = \Q(x, p)$, 
% by definition, the model will satisfy \textbf{individual calibration}:
A model is \textbf{individually calibrated} if it outputs the true conditional quantiles, i.e. $\hQ_p(x) = \Q_p(x)$. In this case, 
we define the observed probability to be
% \vspace{-1.5mm}
\begin{align} \label{eq:indv_cali}
    p^{\text{obs}}_{indv}(p, x) := \mathbb{F}_{\textbf{Y}|x}(\hQ_p(x)),
    \hspace{2mm} \forall x \in \cx, \hspace{2mm} \forall p \in (0, 1).    
\end{align} 
In words, this requires that the probability of observing $y$ below the quantile prediction be equal to $p$, \textit{at each point x $\in \cx$, individually}.
% If the quantile predictions were perfect and exactly the true conditional quantile, $\hQ(x, p) = \Q(x, p)$, by definition, this will satisfy \textbf{individual calibration}:
% \begin{align}
%     \mathbb{F}_{\textbf{Y}|x}(\hQ(x, p)) = p, \forall x \in \cx, \forall p \in (0, 1)    
% \end{align}
If we can verify this property for all $x \in \cx$, then by definition, 
we will know the quantile output is correct and precisely the true conditional quantile. 
However, individual calibration is typically unverifiable with finite datasets in the assumption-less case \citep{zhao2020individual}. 
% This is because a dataset usually contains at most one $y$ value for any $x$ value \citep{zhao2020individual}.
% Furthermore, \cite{zhao2020individual} show that individual calibration is 
% impossible to verify with finite datasets and deterministic distributional predictions.

A relaxed condition is \textbf{average calibration}.
In this case, we define the observed probability to be
% \vspace{-1.5mm}
\begin{align} \label{eq:avg_cali}
    p^{\text{obs}}_{avg}(p) := \mathbb{E}_{x \sim \F_{\textbf{X}}}[\mathbb{F}_{\textbf{Y}|x}(\hQ_p(x))], \hspace{2mm} \forall p\in (0, 1),
\end{align}
i.e. the probability of observing the target below the quantile prediction, 
\textit{averaged over $\F_{\textbf{X}}$}, is equal to $p$. 
Average calibration is often referred to simply as ``calibration''
\citep{cui2020calibrated, kuleshov2018accurate}.
Given a dataset $D = \{(x_i, y_i)\}_{i=1}^{N}$, we can estimate $p^{\text{obs}}_{avg}(p)$ with
$\hat{p}^{\text{obs}}_{avg}(D, p) =
\frac{1}{N}\sum_{i=1}^{N} \mathbb{I}\{y_i \leq \hQ_p(x_i)\}$.
%
%
% \begin{align}
%     \mathbb{F}_{\textbf{Y,X}}(\hQ(x, p)) = p,  x \sim \F_{\textbf{X}}, \forall p \in (0, 1)    
% \end{align}
% \ysc{I need to check whether the above equation is correct}
% This is identical to requiring individual calibration \textit{on average} over the domain $\cx$.
% i.e. $\mathbb{E}_{x \sim \F_{\textbf{x}}}[\mathbb{F}_{\textbf{Y}|x}(\mathbb{Q}(x, p))] = p$, $\forall p \in (0, 1)$.
% Average calibration is often referred to simply as ``calibration'' \citep{cui2020calibrated, kuleshov2018accurate}, 
% and is a commonly used metric because it can be estimated with finite datasets.
% Given a dataset $D$ with $N$ points, $D = \{(x_i, y_i)\}_{i=1}^{N}$, we can estimate average
% calibration using $\hat{p}^{\text{obs}}_{avg}(D, p) = \frac{1}{N}\sum_{i=1}^{N} \mathbb{I}\{y_i \leq \hQ(x_i, p)\}$.
% \vspace{-1.5mm}
% \begin{align} \label{eq:finite_avg_cali}
%     \hat{p}^{\text{obs}}_{avg}(D, p) = \frac{1}{N}\sum_{i=1}^{N} \mathbb{I}\{y_i \leq \hQ(x_i, p)\}.
% \end{align}
Note that if our quantile estimate achieves average calibration then $\hat{p}^{\text{obs}}_{avg} \rightarrow p$ as $N\rightarrow\infty$, $\forall p \in (0, 1)$.
% and verify whether $\hat{p}^{\text{obs}}_{avg} \rightarrow p$ as $N\rightarrow\infty$.
%
%
%%%%% DEFINING ECE HERE
The degree of error in average calibration is commonly measured by \textit{expected calibration error} \cite{tran2020methods, cui2020calibrated, guo2017calibration},
$\text{ECE}(D, \hQ) = \frac{1}{m}\sum_{j=1}^{m} \left | \hat{p}^{\text{obs}}_{avg}\left(D, p_j\right) - p_j \right |$,
where $p_j \sim \text{Unif}(0, 1)$. %are sampled expected probabilities.
% are expected probabilities drawn uniformly between $(0, 1)$.
% where $p_j$ are expected probabilities drawn uniformly between $(0, 1)$.
%
% The degree of error in average calibration is commonly measured by \textit{expected calibration error} (ECE) \ysc{citations},
% which can be computed
%
% defined as $\text{ECE}(\hQ) = \int_0^1 \mid p^{\text{obs}}_{avg}(p) - p \mid dp,$.
% given a dataset $D = \{(x_i, y_i)\}_{i=1}^N$
% as
% $\text{ECE}(D, \hQ) = \frac{1}{m}\sum_{j=1}^{m} \left | \hat{p}^{\text{obs}}_{avg}\left(D, p_j\right) - p_j \right |$,
% \begin{align}
%     \label{eq:ece_est}
%     \widehat{\text{ECE}}(D, \hQ) = \frac{1}{m}\sum_{j=1}^{m} \left | \hat{p}^{\text{obs}}_{avg}\left(D, p_j\right) - p_j \right |,
% \end{align}
% where $p_j$ are a range of expected probabilities drawn uniformly between $(0, 1)$.


% i.e.
% $\text{ECE}(\hQ) = \int_0^1 \mid p^{\text{obs}}_{avg}(p) - p \mid dp,$
% % \vspace{-1.5mm}
% % \begin{align} \label{eq:ece}
% %     \text{ECE}(\hQ) = 
% %     &\int_0^1 \mid p^{\text{obs}}_{avg}(p) - p \mid dp,
% %     % \hspace{10pt} p_{obs}= \mathbb{F}_{\textbf{Y,X}}(\hQ (x, p))
% % \end{align}
%  which can be empirically estimated on any finite dataset $D = \{(x_i, y_i)\}_{i=1}^N$ by
% \begin{align} \label{eq:ece_est}
%     % \widehat{\text{ECE}}(D, \hQ) = \sum_{n=1}^{N-1} \left | \hat{p}^{\text{obs}}_{avg}\left(\frac{n}{N}\right) - \frac{n}{N} \right | 
%     \widehat{\text{ECE}}(D, \hQ) = \frac{1}{m}\sum_{j=1}^{m} \left | \hat{p}^{\text{obs}}_{avg}\left(D, p_j\right) - p_j \right |.
% \end{align}
% Here, $p_j$ are a range of expected probabilities drawn uniformly between $(0, 1)$.
% % Here $p$ is replaced with $n/N$ since $1/N, 2/N, \ldots, (N-1)/N$ are the only values of $p \in (0, 1)$ that can be observed.

% While an individually calibrated model is also average calibrated, it may be possible to have an uninformative, yet average calibrated model.
% For example, quantile predictions that match the true \textit{marginal} quantiles of $\F_{\textbf{Y}}$ 
% will be average calibrated, but will hardly be useful because 
% they do not consider the input $x$ at all.



% It may be possible to have an uninformative, yet average calibrated model. For example,
% quantile predictions that match the true \textit{marginal} quantiles of $\F_{\textbf{Y}}$ 
% will be average calibrated, but will hardly be useful since they do not depend on the input $x$.
% Therefore, the notion of \textbf{sharpness} is often considered together with average
% calibration. Sharpness quantifies the concentration of distributional predictions,
% and \textit{is a property of the distributional prediction only} \citep{gneiting2007probabilistic}. 
% For example, in non-parametric predictions, the width of a centered $95\%$ prediction interval is commonly used as a measure of sharpness.
% % For example, in predictions that parameterize a Gaussian, 
% % the variance of the predicted distribution is often taken as a measure of sharpness, while in
% % non-parametric predictions, the width of a centered $95\%$ prediction interval is commonly used.
% % \ysc{which we will use in this work.}
% There generally exists a tradeoff between average calibration and sharpness \citep{gneiting2007probabilistic, murphy1973new}.

It may be possible to have an uninformative, yet average calibrated model. For example,
quantile predictions that match the true \textit{marginal} quantiles of $\F_{\textbf{Y}}$ 
will be average calibrated, but will hardly be useful since they do not depend on the input $x$.
Therefore, the notion of \textbf{sharpness} is also considered, which quantifies the concentration of distributional predictions \citep{gneiting2007probabilistic}.
% (and \textit{is a property of the distributional prediction only} \citep{gneiting2007probabilistic}. 
% (and is a property of the distributional prediction only \citep{gneiting2007probabilistic}).
For example, for non-parametric predictions, the width of a centered $95\%$ prediction interval is often used as a measure of sharpness.
% For example, in predictions that parameterize a Gaussian, 
% the variance of the predicted distribution is often taken as a measure of sharpness, while in
% non-parametric predictions, the width of a centered $95\%$ prediction interval is commonly used.
% \ysc{which we will use in this work.}
There generally exists a tradeoff between average calibration and sharpness \citep{gneiting2007probabilistic, murphy1973new}.

Recent works have suggested a notion of calibration stronger than average calibration, called adversarial group calibration \citep{zhao2020individual}.
This stems from the notion of \textbf{group calibration} \citep{hebert2017calibration, kleinberg2016inherent}, which prescribes measurable subsets 
$\mathcal{S}_i \subset \cx$ s.t. $P_{x \sim \F_{\textbf{X}}}(x \in \mathcal{S}_i) > 0$, $i=1,\dots,k$, 
and requires the predictions to be average calibrated within each subset.
% $\mathcal{S}_1,\dots,\mathcal{S}_k$.
Adversarial group calibration then
% does not prescribe known subsets in advance, but
requires average calibration for \textit{any subset of $\cx$ with non-zero measure}.
Denote $\bx_{\mathcal{S}}$ as a random variable that is conditioned on being in the set $\mathcal{S}$.
For \textbf{adversarial group calibration}, the observed probability is
% \vspace{-1mm}
% \vspace{-1.5mm}
\begin{align} \label{eq:adversarial-group-calibration}
\begin{split}
    % &p^{\text{obs}}_{adv}(p) := \mathbb{E}_{x \sim \F_{\textbf{X}_{\mathcal{S}}}}[\mathbb{F}_{\textbf{Y}|x}(\hQ(x, p))], \forall p \in (0, 1),\\
    % &\hspace{20pt} \forall \mathcal{S} \subset \cx \text{  s.t.  } P_{x \sim \F_{\textbf{X}}} (x \in \mathcal{S}) > 0.
    %
    % p^{\text{obs}}_{adv}(p) := \hspace{2mm} &\mathbb{E}_{x \sim \F_{\textbf{X}_{\mathcal{S}}}}[\mathbb{F}_{\textbf{Y}|x}(\hQ(x, p))], \forall p \in (0, 1),\\
    % & \forall \mathcal{S} \subset \cx \text{  s.t.  } P_{x \sim \F_{\textbf{X}}} (x \in \mathcal{S}) > 0.
    %
    p^{\text{obs}}_{adv}(p) := \hspace{2mm} \mathbb{E}_{x \sim \F_{\textbf{X}_{\mathcal{S}}}}[\mathbb{F}_{\textbf{Y}|x}(\hQ_p(x))],
    \hspace{2mm} \forall p \in (0, 1),
    \hspace{2mm} \forall \mathcal{S} \subset \cx \text{  s.t.  } P_{x \sim \F_{\textbf{X}}} (x \in \mathcal{S}) > 0.
\end{split}
\end{align}
% \begin{align}
%     &\mathbb{F}_{\textbf{Y,X}_{\mathcal{S}}}(\hQ(x, p)) = p,  x \sim \F_{\textbf{X}_{\mathcal{S}}}, \forall p \in (0, 1),\\
%     &\hspace{20pt} \forall \mathcal{S} \subset \cx \text{  s.t.  } P_{x \sim \F_{\textbf{X}}} (x \in \mathcal{S}) > 0
% \end{align}
With a finite dataset, we can measure a proxy of adversarial group calibration by measuring the average calibration within all subsets of the dataset with sufficiently many points.
%
% The key difference among the three notions of calibration involves $\mathcal{X}$:
Intuitively, individual calibration inspects the discrepancy between $p^{\text{obs}}$ and $p$ for
individual inputs $x \in \cx$, adversarial group calibration relaxes this by
inspecting any subset of $\mathcal{X}$ with non-zero measure, and
average calibration relaxes this further by considering the full distribution of $\bX$.

% The key difference among the three notions of calibration involves the
% input space $\mathcal{X}$. 
% Individual calibration inspects the discrepancy between observed and expected probabilities for individual inputs $x \in \cx$, 
% while adversarial group calibration relaxes this by inspecting any subset of
% $\mathcal{X}$ with non-zero measure. Average calibration relaxes this
% further by considering the full distribution of $\bx$.
% % The key difference among the three notions of calibration is the distribution over input points. 
% % where any single point $x$ has probability measure 0. 
% % Adversarial group calibration relaxes this by similarly inspecting any subset of




\begin{figure}[t!]
    \centering
    \subfigure[Test Loss Curves]{\includegraphics[width=0.325\textwidth]{NeurIPS2021/figures/synth_test_loss.pdf}}
    % \subfigure[]{\includegraphics[width=0.35\textwidth]{NeurIPS2021/figures/synth_test_cal_sharp.pdf}}
    % \subfigure[]{\includegraphics[width=0.30\textwidth]{NeurIPS2021/figures/pareto.pdf}}
    \subfigure[Test Calibration]{\includegraphics[width=0.33\textwidth]{NeurIPS2021/figures/synth_test_cal.pdf}}
    \subfigure[Test Sharpness]{\includegraphics[width=0.33\textwidth]{NeurIPS2021/figures/synth_test_sharp.pdf}}
    \vspace{-3mm}
    \caption{\textbf{(a)} Test loss continues to decrease until the validated epoch. \textbf{(b-c)} At the validated epoch, \textit{SQR} (optimizes \textit{pinball loss}) is highly miscalibrated while sharper than the true sharpness level. \textit{Cali} (optimizes proposed \textit{calibration loss}) is better calibrated while less sharp than the true sharpness.}
    \label{fig:synth_example}
    \vspace{-2mm}
\end{figure}




One alternative family of evaluation metrics is \textbf{proper scoring rules} \citep{gneiting2007strictly}. 
Proper scoring rules are summary statistics of overall performance of a
distributional prediction and consider both calibration and sharpness
jointly \citep{gneiting2007probabilistic}. 
% A (possibly non-unique) optimum of a proper scoring rule is attained when the prediction matches the true underlying distribution. 
For example, negative log-likelihood (NLL) is a proper scoring rule
that is commonly used with density predictions \citep{detlefsen2019reliable, pearce2018uncertainty, lakshminarayanan2017simple}. 
For quantile predictions, one proper score is the \textbf{check score}, \textit{which is identical to the pinball loss}. 
Since proper scoring rules consider both calibration and sharpness together 
in a single value, they can serve as optimization objectives for UQ. 
% NLL is a widely used loss function for density outputs \cite{}. 
% Likewise, optimizing the pinball loss 
For example, optimizing the pinball loss 
is the traditional method in quantile regression \citep{koenker1978regression},
and many recent quantile-based UQ methods focus on optimizing this objective \citep{rodrigues2020beyond, tagasovska2019single, cannon2018non, xu2017composite}.

% In this work, however, we take note of the fact that
% the balance between calibration and sharpness that the pinball loss provides
% is arbitrary and dependent on the expressivity of the model class --
% with highly expressive models, this balance can be heavily skewed towards sharpness.

In this work, however, we note that the balance between calibration and
sharpness implied by the pinball loss
is arbitrary and depends on the expressivity of the model class---and with highly
expressive models, this balance can be heavily skewed towards sharpness.
In their seminal work on probabilistic forecasts, 
\citet{gneiting2007strictly} contend that the goal of probabilistic forecasting 
is to ``maximize the sharpness of the predictive distribution subject to calibration'',
i.e. calibration should be first achieved and then sharpness optimized.
We show that common machine learning methods that use 
the pinball loss objective may in fact lead to an arbitrary and miscalibrated UQ.
% i.e. calibration should be achieved and then sharpness optimized as much as possible.
% once calibration is first achieved, sharpness should then be optimized
% while maintaining calibration.
%
% Meanwhile, we can show that the standard machine learning procedure
% with the pinball loss objective (i.e. assume a flexible model, 
% optimize for the pinball loss on a finite training set, 
% and validating and testing on separate, held out, finite datasets) 
% may lead to an arbitrary UQ that is miscalibrated.

% We show that
% procedures in machine learning, which use the
% % optimize the pinball loss objective with flexible model classes, using the
% pinball loss objective (i.e. assume a flexible model, 
% optimize for the pinball loss on a finite training set, 
% and validating and testing on separate, held out, finite datasets) 
% may lead to an arbitrary and miscalibrated UQ.
















% {\bf Proposition 1.}  \label{prop:pinball}
% OLD PROP 1
% {\it Assume a model class $F$ with an infinite capacity, and pinball
% loss $\rho_{\tau}(y, \hat{y})$ as defined in Eq.~\ref{eq:pinball_loss}.
% Consider a model $f \in F$ that is empirically average calibrated, 
% i.e. $\widehat{\text{ECE}}(D, f) = 0.0$.
% Then, there always exists another solution $g \in F$
% s.t. $g$ has lower pinball loss than $f$ for any quantile level $\tau \in (0, 1)$,
% but worse empirical average calibration than $f$ on $D$.} [Proof: Appendix~\ref{}]


{\bf Proposition 1}. \label{prop:pinball}
{\it Consider a finite dataset $D$, the pinball loss $\rho_\tau$ (Eq.~\ref{eq:pinball_loss}) and a quantile model
$f: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$ that is average calibrated on $D$, i.e. $\text{ECE}(D, f) = 0$.
Then there always exists another quantile model $g: \mathcal{X} \times (0, 1) \rightarrow \mathcal{Y}$, such that, for any quantile level $\tau \in (0, 1)$, 
$g$ has lower pinball loss than $f$ on $D$, i.e. 
$\sum_{i=1}^{N}\rho_\tau(y_i, g_\tau(x_i)) < \sum_{i=1}^{N}\rho_\tau(y_i, f_\tau(x_i))$,
but worse average calibration than $f$, i.e. $\text{ECE}(D, g) > \text{ECE}(D, f)$.} 

\textbf{Proof:} The proof is given in Appendix~\ref{app:prop_1}.


% \williex{State here: [In some cases, could try to mitigate this with 
% regularization (or a constrained model class), but we still find that this
% adverse behavior holds (we show this explicitly in experiments in appendix
% XYZ), (and regularization can also warp results in other ways?)]}




% Based on the best validation loss, we examine the performance at training epoch 350 and 410, respectively for \textit{SQR} and \textit{Cali}.
%     \textit{SQR} learns a solution that is sharper than the true sharpness, while highly miscalibrated. 
%     \textit{Cali} learns a solution that is less sharp than the true sharpness, but more calibrated.

% \ysc{add a note about the ``empirical, practical'' setting where
% only empirical calibration is measureable?}

This proposition essentially states
how the pinball loss can become detached from
calibration, and we show its practical ramifications via a synthetic example in
Figure~\ref{fig:synth_example} (experiment details in Appendix~\ref{app:synth_example}).
% We further demonstrate this proposition empirically in Figure~\ref{fig:synth_example}.
We first note in Figure~\ref{fig:synth_example} (a) and (b) that
even while the pinball loss decreases on the test set,
test calibration worsens (while sharpness improves).
Further, at the best validation epoch, 
optimizing the pinball loss converges to a solution that is sharper than the true noise level. 
% This is especially egregious (\ysc{too strong?}), since
Note that a UQ that is sharper than the true noise level will \textit{never} be calibrated 
(meanwhile, a less sharp prediction \textit{can still be calibrated}, e.g. 
the marginal distribution $\F_{\textbf{Y}}$).
While this may seem like an issue that can simply be addressed with regularization, we demonstrate in Appendix~\ref{app:regularization_pinball} how that is not the case.
These pitfalls motivate our methods in Section~\ref{sec:methods}. 

% These pitfalls motivate our loss function in Section~\ref{sec:cali},
% which targets calibration and sharpness, and explicitly selects a trade-off between the two.

==> app_definition.tex <==
\section{Additional Definitions} \label{app:definition}

% \williex{Want an opening sentence before the bullets, such as:}\\
We give definitions for the two empirical quantities discussed in Section~\ref{sec:cali}.

The \textit{Empirical Calibration Objective}, $\mathcal{C}(D, \hQ_p, p)$,
is defined to be
\begin{align} %\label{eq:emp_cal_obj}
    \begin{split}
        \mathcal{C}(D, \hQ, p) 
        & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ_p(x_i)) \mathbb{I}\{y_i > \hQ_p(x_i)\} \right] \\ 
        % &\mathcal{C}(D, \hQ, p) = \\
        % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
        & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ_p(x_i) - y_i) \mathbb{I}\{\hQ_p(x_i) > y_i\} \right].
    \end{split}
\end{align}

The \textit{Empirical Sharpness Objective}, $\mathcal{P}(D, \hQ_p, p)$, is defined to be
\begin{align} %\label{eq:emp_sharp_obj}
    &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} 
        \begin{cases} 
            \hQ_{1-p}(x_i) - \hQ_p(x_i) \hspace{5pt} (p \leq 0.5)\\
            \hQ_p(x_i) - \hQ_{1-p}(x_i) \hspace{5pt} (p > 0.5).
        \end{cases}
\end{align}

% \begin{itemize}
% \item
% Empirical Calibration Objective, $\mathcal{C}(D, \hQ_p, p):$
% \begin{align} \label{eq:emp_cal_obj}
%     \begin{split}
%         \mathcal{C}(D, \hQ, p) 
%         & =\mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         % &\mathcal{C}(D, \hQ, p) = \\
%         % & \hspace{12pt} \mathbb{I}\{\hp^{\text{obs}}_{avg} < p\} \frac{1}{N}\sum_{i=1}^{N} \left[ (y_i - \hQ(x_i, p)) \mathbb{I}\{y_i > \hQ(x_i, p)\} \right] \\ 
%         & \hspace{10pt} +\mathbb{I}\{\hp^{\text{obs}}_{avg} > p\} * \frac{1}{N}\sum_{i=1}^{N} \left[ (\hQ(x_i, p) - y_i) \mathbb{I}\{\hQ(x_i, p) > y_i\} \right] \\
%     \end{split}
% \end{align}

% \item
% Empirical Sharpness Objective, $\mathcal{P}(D, \hQ_p, p):$
% \begin{align} \label{eq:emp_sharp_obj}
%     &\mathcal{P}(D, \hQ, p) = \frac{1}{N}\sum_{i=1}^{N} 
%         \begin{cases} 
%             \hQ(x_i, 1-p) - \hQ(x_i, p) \hspace{5pt} (p \leq 0.5)\\
%             \hQ(x_i, p) - \hQ(x_i, 1-p) \hspace{5pt} (p > 0.5)
%         \end{cases}
% \end{align}

% \end{itemize}
